DeltaGrad: Rapid retraining of machine learning models

Machine learning models are not static and may need to be retrained on slightly changed datasets, for instance, with the addition or deletion of a set of data points. This has many applications, including privacy, robustness, bias reduction, and uncertainty quantifcation. However, it is expensive to retrain models from scratch. To address this problem, we propose the DeltaGrad algorithm for rapid retraining machine learning models based on information cached during the training phase. We provide both theoretical and empirical support for the effectiveness of DeltaGrad, and show that it compares favorably to the state of the art.

==> Sections/online_SGD_analysis.tex <==
% !TEX root = ..\supplement.tex
\subsubsection{Convergence rate analysis for online stochastic gradient descent version of \Increm}


For stochastic gradient descent (SGD), at the $k_{th}$
deletion request, suppose that at the $t_{th}$ iteration, the minibatch is $\miniB_t$, the model parameters computed by using the \Basel\ and \Increm\ are denoted by $\usw_t(k)$ and $\isw_t(k)$ resp., where $\isw_t(0) = \usw_t(0) = \sw_t$. The Hessian matrix evaluated at this mini-batch between $\isw_t(k+1)$ and $\isw_t(k)$ at the $t_{th}$ iteration is denoted as $\sbHk{k}_t$, which equals to:
$$\sbHk{k}_t = \frac{1}{B-\Delta B_{t,k}}\sum_{i\not\in R_{k}, i \in \miniB_t}\int_{0}^1 \bH_i(\isw_t(k) + x(\isw_t(k+1)-\isw_t(k)))dx$$

for which, $$\sbHk{0}_t = \frac{1}{B}\sum_{i \in \miniB_t}\int_0^1\bH_i(\isw_t(0) + x(\isw_t(1)-\isw_t(0)))dx$$

in which $\Delta B_{t,k}$ represents the total number of samples removed from mini-batch $\miniB_t$ at the first $k$ deletion requests. Since the total number of the removed samples at the first $k$ deletion requests is no more than $k$, then $\Delta B_{t,k} \leq k$. We use $\sBk{k-1}_{j_m}$ to denote the approximated Hessian matrix at the $k_{th}$ deletion request at the ${j_m}_{th}$ iteration and the product $\sBk{k-1}_{j_m}(\isw_t(k) - \isw_t(k-1))$ approximates $$\frac{1}{B-\Delta B_{t,k-1}}\sum_{i\not\in R_{k-1}, i \in \miniB_t}\nabla F_i(\isw_t(k)) - \nabla F_i(\isw_t(k-1)).$$

The evaluation of \Increm\ at the $r_{th}$ depends on the following history information $\{\isw_{0}(r-1), \isw_{1}(r-1), \dots, \isw_{t}(r-1)\}$ and $$\{\ag \left(\isw_{0}(r-1)\right), \ag\left(\isw_{1}(r-1)\right), \dots, \ag\left(\isw_{t}(r-1)\right)\}$$ 
(instead of $\{\sw_{0}, \sw_{1}, \dots, \sw_{t}\}$ and $\{\ag \left(\sw_{0}\right), \ag\left(\sw_{1}\right), \dots, \ag\left(\sw_{t}\right)\}$ in the SGD version of \Increm). 

%Note that $\ag(\isw_t(k))$ ($k\leq r$) is not necessarily equal to $\nabla F$ due to the approximation brought by \Increm. 
Again, we know that due to the periodicity of \Increm, at iteration $0,1,\dots,j_0$ and iteration $j_0 + xT_0$ ($x=1,2,\dots,$), the gradients are explicitly evaluated:
$$\ag(\isw_t(k)) = \frac{1}{B-\Delta B_{t,k}}\sum_{i\not\in R_k, i \in \miniB_t} \nabla F_i(\isw_t(k))$$
in which $t = 0,1,\dots, j_0$ or $t = j_0 + xT_0$ ($x \geq 1$) and all $k \leq r$. 
Thus at those iterations, $\Dsg$ (We use $\Dsg(k)$ to denote the $\Dsg$ at the $k_{th}$ deletion request) is evaluated as below and used as the input of Algorithm \ref{alg: lbfgs_algorithm} later.
$$\Dsg_{j_q}(k) = \frac{1}{B-\Delta B_{t,k}}[\sum_{i\not\in R_k, i \in \miniB_t}\nabla F_i(\isw_{j_q}(k)) - \sum_{i \not\in R_k, i \in \miniB_t}\nabla F_i(\isw_{j_q}(k-1))]$$



%Also, due to the periodicity, the sequence $[\Dsg_{j_0}, \Dsg_{j_1},\dots, \Dsg_{j_{m-1}}]$ that is used in approximating the hessian matrix should always use the exact gradient information, which means that:
where $q=1,2,\dots,m-1$. So equation \eqref{sgdcond}, i.e. the bound on the eigenvalues of $\sBk{k}_{j_q}$ holds for all $k=1,2,\dots,r$. 

As the other input of Algorithm \ref{alg: lbfgs_algorithm}, $\Dsw$ (We use $\Dsw(k)$ to denote the $\Dsw$ at the $k_{th}$ deletion request) becomes:
$$\Dsw_{j_q}(k) = \isw_{j_q}(k) - \isw_{j_q}(k-1)$$
where $q=1,2,\dots,m-1$.

But for the iterations where the gradients are not explicitly evaluated, the calculation of $\ag(\isw_t(k))$ depends on the approximated Hessian matrix $\sBk{k-1}_{j_m}$ and the approximated gradients calculated at the $t_{th}$ iteration at the ${k-1}_{th}$ deletion request. But the update rule depends on whether the removed sample $i_k$ is in $\miniB_t$ or not:
% the derivation rule for $\ag(\isw_t(k))$ is:
\begin{align}\label{eq: sg_w_k_deriv}
    \begin{split}
        & \ag(\isw_t(k))\\
        & = \frac{1}{B-\Delta B_{t,k}}\{[B-\Delta B_{t,k-1})(\sBk{k-1}_{j_m}(\isw_t(k) - \isw_t(k-1))\\
        & + \ag(\isw_t(k-1))] - \mathbbm{1}(i_k \in \miniB_t)\cdot\nabla F_{i_k}(\isw_t(k))\}
    \end{split}
\end{align}

in which $\mathbbm{1}(i_k \in \miniB_t)$ is the indicator function that is 1 when the sample $i_k$ is in current mini-batch and 0 otherwise. If $i_k$ is in the mini-batch $\miniB_t$, then $\Delta B_{t,k} = \Delta B_{t,k-1} + 1$, otherwise $\Delta B_{t,k} = \Delta B_{t,k-1}$. So $\Delta B_{t,k} = \Delta B_{t,k-1} + \mathbbm{1}(i_k \in \miniB_t)$. 
Note that  $\ag(\isw_t(k))$ approximates $$\frac{1}{B-\Delta B_{t,k}}\sum_{i\not\in R_{k}, i\in \miniB_{t}}\nabla F_i(\isw_t(k))$$
and its evaluation requires $\ag(\isw_t(k-1))$ which approximates $$\frac{1}{B-\Delta B_{t,k-1}}\sum_{i\not\in R_{k-1}, i\in \miniB_{t}}\nabla F_i(\isw_t(k-1)).$$

Similarly, we use $d_{j_a,j_b}(k)$ 
% and $\xi_{j_a,j_b}(k)$ 
to denote the value of $d$
% and $\xi$ values 
at the $k_{th}$ deletion request and .
% $$\xi_{j_1,j_m}^S(k-1):= A d_{j_1,j_m + T_0 - 1}(k-1)
% + A \frac{1}{\frac{1}{2}-\frac{1}{n}}M_1\frac{1}{n}$$




So in this case, the update rule of $\isw_t(k)$ becomes:
\begin{align}\label{iw_u_online_sgd}
    \isw_{t+1}(k) = \begin{cases}
         &\isw_{t}(k)-\frac{\eta}{B-\Delta B_{t,k}} \sum_{i\not\in R_k, i \in \miniB_t}\nabla F_i(\isw_t(k)),\,\, (t - j_0) \mod T_0 = 0\ or\ t \leq j_0 \\[2pt]
         \begin{split}
        &\isw_{t}(k)\\
        & - \frac{\eta}{B-\Delta B_{i,k}}\{(B-\Delta B_{i,k-1})[\B_{j_m}^{k-1}(\isw_t(k) - \isw_t(k-1)) \\
        &+ \ag(\isw_{t}(k-1))] - \mathbbm{1}(i_k \in \miniB_t)\nabla F_{i_k}(\isw_t(k))\},\,\, else     
         \end{split}
        \end{cases}
\end{align}

% where we define $R_k = \{i_1,i_2,\dots, i_k\}$. Note that $\{i_1,i_2,\dots,i_{k-1}\}$ has been deleted in the first $k-1$ deletion requests while the sample $i_k$ is removed at the $k_{th}$ deletion request. Also we define $\isw_t(0) = \sw_t$.

% Recall that the gradients are explicitly evaluated 


\textbf{Proof preliminary}

%Note that at the $k_{th}$ deletion request, the sample $i_k$ is deleted from the remaining samples after the first $k-1$ deletion requests, which means that at the $t_{th}$ iteration at the $k_{th}$ deletion request, the mini-batch size before and after the $k_{th}$ deletion will be $B-\Delta B_{t,k-1}$ and $B-\Delta B_{t,k}$ respectively. According to equation \eqref{eq: sg_w_k_deriv}, we know that $\Delta B_{t,k} = \Delta B_{t, {k-1}} + \mathbbm{1}(i_k \in \miniB_t)$. 

%Note that for the first $k$ deletion requests, there are $k$ samples removed in total and we assume that the distribution of the removed samples is uniformly distributed. So equation \eqref{eq: delta_b_bound} still holds, which is rewritten as below by using current notations:
%with probability higher than $1-(t+1)\times 2\exp(-2\sqrt{B})$, 
%\begin{align}
%\frac{\Delta B_{t', k}}{B} \leq \frac{k}{n} + \frac{1}{B^{1/4}}
%\end{align}
%holds for all $t' \le t$



Lemma \ref{lemma: delta_t_zeta_bounds} can be rephrased as:

\begin{lemma}[Upper bound on $\delta_{t,S}$]\label{lemma: delta_t_zeta_bounds_multi_sgd}
Define $$\delta_{t,S}^k = \frac{1}{B-\Delta B_{t,{k-1}}}\sum_{i\in \miniB_t, i \not\in R_{k-1}} \nabla F_i(\usw_t(k-1)) - \frac{1}{B-\Delta B_{t,k}}\sum_{i\in \miniB_t, i \not\in R_{k}} \nabla F_i(\usw_t(k-1))$$.
Then $\|\delta_{t,S}^k\| \leq 2c_2 \frac{\Delta B_{t,k} - \Delta B_{t,k-1}}{B-\Delta B_{t,{k-1}}}$.
Plus, with probability higher than $1-t\times 2\exp(-2\sqrt{B-{k+1}})$, $\|\delta_{t',S}\| \leq 2c_2 \frac{\Delta B_{t', k} - \Delta B_{t', k-1}}{B-\Delta B_{t, k-1}} \leq 2c_2(\frac{1}{n} + \frac{1}{(B-k+1)^{1/4}})$ for all $t' \leq t$.
\label{updels_sgd}
\end{lemma}

\begin{proof}
Through the same derivation as the proof of Lemma \ref{lemma: delta_t_zeta_bounds}, we know that:
$$\|\delta_{t,S}^k\| \leq 2c_2 \frac{\Delta B_{t,k} - \Delta B_{t,k-1}}{B-\Delta B_{t,{k-1}}}$$

Then Hoeffding's inequality is used and thus the following inequality holds:
% \begin{align}
%     Pr(|\frac{\Delta B_t}{B} - \frac{r}{n}| \leq k \sqrt{\frac{r}{Bn}(1-\frac{r}{n})}) \leq \frac{1}{k^2}
% \end{align}

\begin{align*}
 Pr(|\frac{\Delta B_{t',k} - \Delta B_{t',k-1}}{B-\Delta B_{t',k-1}} - \frac{1}{n}| \leq \epsilon) \geq 1-2\exp(-2\epsilon^2(B-\Delta B_{t',k-1}))
\end{align*}

in which $\Delta B_{t',k} - \Delta B_{t',k-1}$ represents the number of the newly removed samples at the $k_{th}$ deletion request at the $t'_{th}$ iteration, which may be 0 or 1.

Then by setting $\epsilon = \frac{1}{(B-\Delta B_{t',k-1})^{1/4}}$
% $k=\frac{1}{\sqrt{\frac{r}{n}(1-\frac{r}{n})}}$, 
the formula above can be written as:
\begin{align*}
    Pr(|\frac{\Delta B_{t',k} - \Delta B_{t',k-1}}{B-\Delta B_{t',k-1}} - \frac{1}{n}| \geq \frac{1}{(B-\Delta B_{t',k-1})^{1/4}}) \leq 2\exp(-2\sqrt{B-\Delta B_{t',k-1}})
\end{align*}

Then by taking the union for all the iterations before $t$, we have: with probability higher than $1-(t+1)\times 2\exp(-2\sqrt{B-\Delta B_{t',k-1}})$, $$|\frac{\Delta B_{t'}-\Delta B_{t',k-1}}{B-\Delta B_{t',k-1}} - \frac{1}{n}| \leq \frac{1}{(B-\Delta B_{t',k-1})^{1/4}}$$ and thus $$\frac{\Delta B_{t'}-\Delta B_{t',k-1}}{B-\Delta B_{t',k-1}} \leq \frac{1}{n} + \frac{1}{(B-\Delta B_{t',k-1})^{1/4}}$$ for all $t' \le t$

Note that since there are $k-1$ samples removed in total across all the mini-batches, then $B-\Delta B_{t',k-1} \geq B - k + 1$

So $$\frac{\Delta B_{t'}-\Delta B_{t',k-1}}{B-\Delta B_{t',k-1}} \leq \frac{1}{n} + \frac{1}{(B-\Delta B_{t',k-1})^{1/4}} \leq \frac{1}{n} + \frac{1}{(B-k+1)^{1/4}}$$ with probability higher than $1-t\times 2\exp(-2\sqrt{B-k+1})$. In what follows, we use $\Psi_1(k)$ to represent $\wuprobk{k}$, for which we know that $\Psi_1(k) \leq \Psi_1(r)$ for any $k \leq r$.

\end{proof}

Similarly, we get the following bound on the average Hessian in a mini-batch at the $k_{th}$ deletion request at the iteration $t$ by using the same derivation as the proof of Theorem \ref{theorem: stochastic_hessian_bound} (except that $B$, $\frac{1}{B}\sum_{i \in \miniB_t}\bH_i(\sw_t))$, $\bH(\sw_t)$ are replaced by $B-\Delta B_{t,k-1}$, $\left(\frac{1}{B-\Delta B_{t,k-1}}\sum_{i \in \miniB_{t}, i\not\in R_{k-1}} \bH_i(\isw_{t}(k-1))\right)$, 
$\frac{1}{n-{k-1}}\sum_{i \not\in R_{k-1}} \bH_i(\isw_{t}(k-1))$ resp.).
\begin{theorem}[Hessian matrix bound in SGD (online deletion)]\label{theorem: stochastic_hessian_bound_multi}
For a given iteration $t$, with probability higher than $$1-\probk{k},$$ $$\|\left(\frac{1}{B-\Delta B_{t,k-1}}\sum_{i \in \miniB_{t}, i\not\in R_{k-1}} \bH_i(\isw_{t}(k-1))\right) - \frac{1}{n-{k-1}}\sum_{i \not\in R_{k-1}} \bH_i(\isw_{t}(k-1))\|$$
$$\leq \rhboundk{\Delta B_{t,k-1}} \leq \rhboundk{(k-1)}$$ where $p$ represents the number of model parameters.
% $\bH(\w) = \left(\frac{1}{n}\sum_{i =1}^n \bH_i(\w)\right)$ for any model parameter $\w$.
\end{theorem}

In the remaining of this document, we use $\Psi_2(k)$ to represent the probability $\probk{k}$. Similar to $\Psi_1(k)$, $\Psi_2(k)$ also decreases with increasing $k$.

Also, we know that equation \eqref{eq: miniB_gradient_full_gradient_diff} also holds at the $k_{th}$ deletion request in which the mini-batch size becomes $B-\Delta B_{t,k}$, the gradients are evaluated with model parameter $\isw_t(k)$ and the full gradients becomes $\frac{1}{n-k}\sum_{i \not\in R_k} \nabla F_{i}(\isw_t(k))$:
\begin{align*}
    \begin{split}
        & Pr(\|\frac{1}{B-\Delta B_{t,k}}\sum_{i \in \miniB_t, i\not\in R_k}\nabla F_{i}(\isw_t(k)) - \frac{1}{n-k}\sum_{i \not\in R_k} \nabla F_{i}(\isw_t(k))\| \geq c_2 \left(\frac{\log(p+1)}{B-\Delta B_{t,k}}^2\right)^{1/4}) \\
        & \leq  (p+1)\exp\left({-\frac{\log(p+1)\sqrt{B-\Delta B_{t,k}}}{4 + \frac{2}{3}\left(\frac{\log(p+1)}{B-\Delta B_{t,k}}^2\right)^{1/4}}}\right)
    \end{split}
\end{align*}

We can further get the relaxation of the above formula  by using the fact that $\Delta B_{t,k} \leq k$:
\begin{align}\label{eq: miniB_gradient_full_gradient_diff_multi0}
    \begin{split}
        & Pr(\|\frac{1}{B-\Delta B_{t,k}}\sum_{i \in \miniB_t, i\not\in R_k}\nabla F_{i}(\isw_t(k)) - \frac{1}{n-k}\sum_{i \not\in R_k} \nabla F_{i}(\isw_t(k))\| \geq c_2 \left(\frac{\log(p+1)}{B-k}^2\right)^{1/4}) \\
        & \leq \probwk{k} 
%        (p+1)\exp\left({-\frac{\log(p+1)\sqrt{B-k}}{4 + \frac{2}{3}\left(\frac{\log(p+1)}{B-k}^2\right)^{1/4}}}\right)
    \end{split}
\end{align}

Similarly, we use $\Psi_3(k)$ to denote the probability, $\probwk{k}$. Similar to $\Psi_1(k), \Psi_2(k)$, $\Psi_3(k)$ also decreases with increasing $k$.

Note that for \Basel\ to deal with each deletion request, the model parameters will always be retrained from scratch over the remaining samples, which means that Theorem \ref{wu_sgd} also holds if we replace $\usw_t$, $\sw_t$ and $r$ with $\usw_t(k)$, $\usw_t(k-1)$ and 1 respectively:

\begin{theorem}
[Bound between iterates on full and the leave-1-out dataset for $r$ times]\label{wu_sgd_multi} We have
$$\|\usw_{t'+1}(k) - \usw_{t'+1}(k-1)\| \leq (1-\mu\eta) \|\sw_{t'}(k) - \usw_{t'}(k-1)\| + 2c_2\eta \frac{\Delta B_{t',k}- \Delta B_{t',k-1}}{B - \Delta B_{t',k-1}}$$

when $$\frac{\Delta B_{t',k}-\Delta B_{t',k-1}}{B-\Delta B_{t',k-1}} \leq \frac{1}{n} + \frac{1}{(B-k+1)^{1/4}}$$ holds for all $t' \leq t$ and a given $k$, $$\|\usw_{t'+1}(k) - \usw_{t'+1}(k-1)\| \leq \frac{2c_2}{\mu}(\frac{1}{n} + \frac{1}{(B-k+1)^{1/4}}).$$
Since with probability higher than $1-t\times \Psi_1(k)$, $$\frac{\Delta B_{t'}-\Delta B_{t',k-1}}{B-\Delta B_{t',k-1}} \leq \frac{1}{n} + \frac{1}{(B-k+1)^{1/4}}$$ holds for all $t' \leq t$. Then with the same probability, $\|\usw_{t'+1}(k) - \usw_{t'+1}(k-1)\| \leq \frac{2c_2}{\mu}(\frac{1}{n} + \frac{1}{(B-k+1)^{1/4}})$ for $t'\leq t$, where $M_1:=\frac{2c_2}{\mu}$.

% and with probability higher than $1-T\times \wuprob$, $\|\sw_{t} - \usw_{t}\| \leq \frac{2c_2}{\mu}(\frac{1}{n} + \frac{1}{B^{1/4}})$ for all iterations $t$, where $M_1:=\frac{2c_2}{\mu}$.
% [Bound between iterates on full and the leave-1-out dataset for $r$ times]\label{wu_SGD_multi}
% $\|\usw_{t}(r) - \usw_{t}(r-1)\| \leq M_1 \frac{1}{n}$ where $M_1=\frac{2}{\mu }c_2$ is some positive constant that does not depend on $t$.
\end{theorem}

By induction, we know that the following inequalities hold with probability higher than $1-rt\times \Psi_1(r)$:
\begin{align}\label{eq: w_u_w_gap_sgd_single_deletion}
\begin{split}
    & \|\usw_{t'+1}(k) - \usw_{t'+1}(k-1)\|\leq M_1 r (\frac{1}{n} + \frac{1}{(B-r+1)^{1/4}})
\end{split}
\end{align}
for all $k \leq r, t' \leq t$ and
\begin{align}\label{eq: w_u_w_gap_sgd}
\begin{split}
    & \|\usw_{t'+1}(r) - \usw_{t'+1}(0)\|\\
    &= \|\usw_{t'+1}(r) - \sw_{t'+1}\| \leq M_1 r (\frac{1}{n} + \frac{1}{(B-r+1)^{1/4}})
\end{split}
\end{align}
for all $t' \leq t$.



% Also the history information for \Increm\ used at the $k_{th}$ request will become $\{\sw_{0}(k-1), \sw_{1}(k-1), \dots, \sw_{t}(k-1)\}$ and $$\{\ag \left(\sw_{0}(k-1)\right), \ag\left(\sw_{1}(k-1)\right), \dots, \ag\left(\sw_{t}(k-1)\right)\}$$ (note that $\ag$ is not necessarily equal to $\nabla F$ due to the approximation brought by \Increm). Similarly, we use $d_{j_a,j_b}(k)$ 
% % and $\xi_{j_a,j_b}(k)$ 
% to denote the value of $d$ and
% % and $\xi$ values 
% in the $k_{th}$ deletion request and use $\bH_t^{k}$ and $\B_t^{j_m}$ to denote the Hessian matrix and approximated Hessian matrix in the $k_{th}$ deletion request.
% $$\xi_{j_1,j_m}^S(k-1):= A d_{j_1,j_m + T_0 - 1}(k-1)
% + A \frac{1}{\frac{1}{2}-\frac{1}{n}}M_1\frac{1}{n}$$




% So in this case, the update rule for $\isw_t(k)$ becomes:
% \begin{align}\label{iw_u_online}
%     \isw_{t+1}(k) = \begin{cases}
%          &\isw_{t}(k)-\frac{\eta}{B-\Delta B_{t, k}} \sum_{i\not\in R_k}\nabla F(\isw_t(k)),\,\, (t - j_0) \mod T_0 = 0\ or\ t \leq j_0 \\[2pt]
%          \begin{split}
%         &\isw_{t}(k) - \frac{\eta}{B-\Delta B_{t, k}}[(B-\Delta B_{t, k}+1)(\B_{j_m}(\isw_t(k) - \isw_t(k-1)) \\
%         &+ \ag(\isw_{t}(k-1))) - \nabla F_{i_k}(\isw_t(k))],\,\, else     
%          \end{split}
%         \end{cases}
% \end{align}

% where we define $R_k = \{i_1,i_2,\dots, i_k\}$. Note that $\{i_1,i_2,\dots,i_{k-1}\}$ has been deleted in the first $k-1$ deletion requests while the sample $i_k$ is removed at the $k_{th}$ deletion request. Also we define $\isw_t(0) = \sw_t$.

% Recall that the gradients are explicitly evaluated at iteration $0,1,\dots,j_0$ and iteration $j_0 + xT_0$ ($x=1,2,\dots,$), which is true for all $k=1,2,\dots,r$. It indicates that the sequence $[\Delta g_{j_0}, \Delta g_{j_1},\dots, \Delta g_{j_{m-1}}]$ that is used in approximating the hessian matrix should always use the exact gradient information, i.e. $\Delta g_{j_q} = \frac{1}{B-\Delta B_{t, k}}[\sum_{i\not\in R_k}\nabla F_i(\isw_{j_q}(k)) - \sum_{i \not\in R_k}\nabla F_i(\isw_{j_q}(k-1))]$ ($q=1,2,\dots,m-1$). So Lemma \ref{assp: B_K_product_bound}, i.e. the bound of the eigenvalues of $B_{j_q}$ holds for all $k=1,2,\dots,r$. 


Then let us do some analysis on $d_{j_a,j_b}(k)$. 


\begin{lemma}\label{lemma: bound_d_j_multi_sgd}
Suppose that there are $T$ iterations in total at each deletion request, then if we define $$d_{a, b}(k) = \max(\|\isw_y(k) - \isw_z(k)\|)_{a < y < z < b},$$ and the following conditions hold:
\begin{enumerate}
\item $$\|\isw_{t'}(k) - \isw_{t'}(k-1)\| \leq \swikbound{k}$$ $$\leq \frac{2M_1(\frac{1}{n}+\frac{1}{(B-k+1)^{1/4}})}{1-\frac{1}{n} - \frac{1}{(B-r+1)^{1/4}}-2(r-1)(\frac{1}{n} + \frac{1}{(B-r+1)^{1/4}})(\frac{2L+\mu}{\mu})} := \sswikbound{k}$$ holds for all $k < r, t' \leq T$ and $k=r, t'\leq t$
\item $$d_{a, b}(0) \leq (1-\eta\mu)^{a}d_{0,b-a}(0) + 2c_2 \left(\frac{(\log(p+1))^2}{B}\right)^{1/4}$$ holds for all $a < b \leq T$
\end{enumerate}
then 
\begin{align*}
\begin{split}
& d_{a,b}(r) \leq d_{a,b}(0) + 2r\cdot \sswikbound{r} \\&\leq (1-\eta\mu)^{a}d_{0,b-a}(0) + 2c_2 \left(\frac{(\log(p+1))^2}{B}\right)^{1/4}\\
& + 2r\cdot \sswikbound{r}
\end{split}
\end{align*}
 
% and thus $$\xi_{j_a,j_b}(r) \leq A d_{j_a,j_b + T_0 - 1}(0)
% + A \frac{2r + 1}{\frac{1}{2}-\frac{1}{n}}M_1\frac{1}{n}$$ 
where $M_1$ is defined in Theorem \ref{wu_sgd_multi} and $M_1^S$ is a constant which does not depend on $t$ or $k$.
\end{lemma}

\begin{proof}
%Recall that $d_{a, b}(k) = \max(\|\isw_y(k) - \isw_z(k)\|)_{a < y < z < b}$.
For arbitrary $y, z$ such that ${a < y < z < b}$, let us bound $\|\isw_y(k) - \isw_z(k)\|$ as below:
\begin{align*}
    \begin{split}
        & \|\isw_y(k) - \isw_z(k)\|\\
        & = \|\isw_y(k) - \isw_z(k) + \isw_y(k-1) - \isw_z(k-1) + \isw_z(k-1) - \isw_y(k-1)\|\\
        & \leq \|\isw_y(k) - \isw_y(k-1)\| + \|\isw_z(k) - \isw_z(k-1)\| + \|\isw_z(k-1) - \isw_y(k-1)\|
    \end{split}
\end{align*}

Then by using the bound on $\|\isw_t(k) - \isw_t(k-1)\|$, the above formula can be bounded as:
\begin{align}\label{eq: w_is_k_pair_bound_deriv1}
    \begin{split}
        & \leq 2\cdot \sswikbound{k}
        + \|\isw_z(k-1) - \isw_y(k-1)\|
    \end{split}
\end{align}

By using the fact that $$\sswikbound{k}
\leq \sswikbound{r}$$ and applying equation \eqref{eq: w_is_k_pair_bound_deriv1} recursively, we have:
\begin{align*}
    \begin{split}
        &\|\isw_y(r) - \isw_z(r)\|\leq \|\isw_z(0) - \isw_y(0)\| \\
        & + 2r\cdot \sswikbound{r}
    \end{split}
\end{align*}

Then by using the definition of $d_{a,b}(k)$ and the bound on $d_{a,b}(0)$, we get:
\begin{align*}
\begin{split}
    d_{a,b}(r)
   & \leq d_{a,b}(0)
+ 2r\cdot \sswikbound{r}\\
& \leq (1-\eta\mu)^{a}d_{0,b-a}(0) + 2c_2 \left(\frac{(\log(p+1))^2}{B}\right)^{1/4}
 + 2r\cdot \sswikbound{r}
\end{split}
\end{align*}
% \begin{equation}
%     \xi_{j_a,j_b}(r) \leq A d_{j_a,j_b + T_0 - 1}(0)
% + A \frac{2Cr+1}{\frac{1}{2}-\frac{1}{n}}M_1\frac{1}{n}
% \end{equation}

\end{proof}

Also note that according to Lemma \ref{Lemma: bound_d_j_sgd}, $d_{a, b}(0) \leq (1-\eta\mu)^{a}d_{0,b-a} + 2c_2 \left(\frac{\log(p+1)}{B}^2\right)^{1/4}$ holds with probability higher than $1- (t+1)\Psi_3(1) $ for any $a < b \leq t$



%Suppose $\|\sw_{t'} - \isw_{t'}\| \leq \frac{1}{\frac{1}{2}-\frac{r}{n} - \frac{1}{B^{1/4}}}M_1 (\frac{r}{n} + \frac{1}{B^{1/4}})$ and 
%$$\|\left(\frac{1}{B}\sum_{i \in \miniB_{t'}} \bH_i(\sw_{t'})\right) - \bH(\sw_{t'})\| \leq \rhbound$$ hold for any $t' \leq t$.
%%and $\|\bH_{t'}^S - \sB_{j_m}\| \leq \xi_{j_1,j_m}^S^S$ for any $t' < t$  where $k<t$, 
%$M_1$ is provided in Theorem \ref{wu}, i.e. $M_1 = \frac{2c_2}{\mu}$. Then for any $t'$ and $j_m$ such that $ j_m \le t' \leq j_m + T_0 - 1$ and $t' \leq t$, 
%%with probability higher than $$1 - \prob,$$ 
%the following inequality holds:

\begin{theorem}\label{theorem: delta_model_para_bound_multi_sgd}
Suppose that at the $k_{th}$ deletion request, $\|\isw_{t'}(k) - \isw_{t'}(k-1)\| \leq \sswikbound{k} $ and 
$$\|\frac{\sum_{i \in \miniB_{t'}, i \not\in R_{k-1}} \bH_i(\isw_{t'}(k-1))}{B-\Delta B_{t',k-1}}
-
\frac{\sum_{i \not\in R_{k-1}}\bH_i(\isw_{t'}(k-1))}{n-{k-1}} \|
 \leq \rhboundk{(k-1)}$$ hold for any $t' \leq t$ where $M_1 = \frac{2c_2}{\mu}$. Let $a = \frac{L(L+1) + K_2 L}{\mu  K_1}$ for the upper and lower bounds $K_1,K_2$ on the eigenvalues of the quasi-Hessian from equation \eqref{sgdcond}, and for the Lipshitz constant $c_0$ of the Hessian. 
Then for any $t_1,t_2, t, j_m$ such that $1 \leq t_1 < t_2 \leq t$, 
% with probability higher than $1- \prob)$, 
we have:
$$\|\sbHk{(k-1)}_{t_1} - \sbHk{k-1}_{t_2}\| \leq 2\rhboundk{k-1} + c_0 d_{t_1, t_2}(k-1)$$
$$ + 3c_0 \sswikbound{k}$$
%$$ c_0 M_1\frac{1}{\frac{1}{2}-\frac{r}{n} - \frac{1}{B^{1/4}}}(\frac{r}{n} + \frac{1}{B^{1/4}})$$
%, then for $1 \leq z+1 \leq y \leq m$ we have,
%$$\|\sbHk{k-1}_{j_z} - \sbHk{k-1}_{j_y}\| \leq c_0 d_{j_z, j_y}(k-1) + c_0 \sswikbound{k}$$
 and for any $j_1,j_2,\dots,j_m$ and the corresponding $[\Dsg_{j_1}, \Dsg_{j_2},\dots,\Dsg_{j_m}]$, $[\Dsw_{j_1}, \Dsw_{j_2},\dots,\Dsw_{j_m}]$ such that $j_m \leq t' \leq j_m +T_0 - 1$ and $t' \leq t$
$$\|\Dsg_{j_z} - \sBk{k-1}_{j_y}\Dsw_{j_z}\| \leq \left[(1+a)^{j_y-j_z-1} - 1\right]\cdot c_0[\frac{2}{c_0}\rhboundk{(k-1)}$$
$$+ d_{j_z, j_y}(k-1) + 3\times\sswikbound{k}]s_{j_1,j_m}(k-1)$$
 where $s_{j_1,j_m}(k-1) = \max\left(\|\Dsw_{a}(k-1)\|\right)_{a=j_1,j_{2},\dots,j_m}$, 
 and $d_{j_z,j_y}(k-1)$ is defined in Lemma \ref{lemma: bound_d_j_multi_sgd}
%  as the maximum gap between the steps of the algorithm over the iterations from $j_z$ to $j_y$:
%\beq\label{d0_sgd_multi}
%d_{j_z,j_y}(k-1) = \max\left(\|\isw_{a}(k-1) - \isw_{b}(k-1)\|\right)_{j_z \leq a \leq b \leq j_y}.
%\eeq
\end{theorem}
%\begin{proof}
%Let us bound the difference between the averaged Hessians $\|\sbHk{k-1}_{j_z} - \sbHk{k-1}_{j_y}\|$, where $1 \leq z < y \leq m$, using their definition, as well as using Assumption \ref{assp: hessian_continuous} on the Lipshitzness of the Hessian:
%%k->y, q->z
%\begin{align}\label{eq: hessian_diff_bound01}
%    \begin{split}
%      & \|\bH_{j_y}^{k-1} - \bH_{j_z}^{k-1}\|\\
%      & = \|\int_0^1 [\bH(\isw_{j_y}(k-1) + x (\isw_{j_y}(k) - \isw_{j_y}(k-1)))]dx\\
%      & - \int_0^1 [\bH(\isw_{j_z}(k-1) + x (\isw_{j_z}(k) - \isw_{j_z}(k-1)))]dx\|\\
%      & = \| \int_0^1 [\bH(\isw_{j_y}(k-1) + x (\isw_{j_y}(k) - \isw_{j_y}(k-1)))\\
%      & -\bH(\isw_{j_z}(k-1) + x (\isw_{j_z}(k) - \isw_{j_z}(k-1)))]dx \|\\
%      & \leq c_0 \int_0^1 \|\isw_{j_y}(k-1) + x (\isw_{j_y}(k) - \isw_{j_y}(k-1))\\
%      & - [\isw_{j_z}(k-1) + x (\isw_{j_z}(k) - \isw_{j_z}(k-1))]\| dx \\
%      & \leq c_0\| \isw_{j_y}(k-1) - \isw_{j_z}(k-1)\|\\
%      & + \frac{c_0}{2}\|\isw_{j_y}(k) - \isw_{j_y}(k-1) - (\isw_{j_z}(k) - \isw_{j_z}(k-1))\| \\
%      & \leq c_0 \|\isw_{j_y}(k-1) - \isw_{j_z}(k-1)\|\\
%      & + \frac{c_0}{2}\|\isw_{j_z}(k)- \isw_{j_z}(k-1)\| + \frac{c_0}{2}\|\isw_{j_y}(k) - \isw_{j_y}(k-1)\|\\
%      & \leq c_0 d_{j_y, j_z}(k-1) + c_0\sswikbound{k}\\
%      & \leq c_0 d_{j_1, j_m +T_0 - 1}(k-1) + c_0\sswikbound{k}
%    \end{split}
%\end{align}
%On the last line, we have used the definition of $d_{j_z, j_y}$, and the assumption on the boundedness of $\|\isw_{j_z}(k) - \isw_{j_z}(k-1)\|$.
%
%Then by following the rest of the proof of Theorem \ref{theorem: delta_model_para_bound}, we know that the following inequality holds: $$\|\Dg_{j_z} - \B_{j_y}\Dw_{j_z}\| \leq \left[(1+a)^{y-z-1} - 1\right]\cdot c_0 (d_{j_z,j_y}(k-1) + \sswikbound{k}) \cdot s_{j_1,j_m}$$
%
%\end{proof}

Similarly the online version of Corollary \ref{corollary: approx_hessian_real_hessian_bound_sgd} also holds by following the same derivation as the proof of Corollary \ref{corollary: approx_hessian_real_hessian_bound_sgd} (except that $r$, $\xi_{j_1, j_m}^S$ and $d_{j_1, j_m + T_0 -1}$ is replaced by 1, $\xi_{j_1, j_m}^S(k-1)$ and $d_{j_1, j_m + T_0 -1}(k-1)$ respectively), i.e.:

\begin{corollary}[Approximation accuracy of quasi-Hessian to mean Hessian]\label{lemma: corollary: approx_hessian_real_hessian_bound_multi_sgd}
%Suppose at the $k_{th}$ deletion request, $\|\isw_{j_s}(k) - \isw_{j_s}(k-1)\| \leq \sswikbound{k} $ where $s = 1,2,\dots, m$. 
Suppose that at the $k_{th}$ deletion request, $$\|\isw_{t'}(k) - \isw_{t'}(k-1)\| \leq \sswikbound{k}$$ and 
$$\|\frac{\sum_{i \in \miniB_{t'}, i \not\in R_{k-1}} \bH_i(\isw_{t'}(k-1))}{B-\Delta B_{t',k-1}}
-
\frac{\sum_{i \not\in R_{k-1}}\bH_i(\isw_{t'}(k-1))}{n-{k-1}} \|
 \leq \rhboundk{(k-1)}$$ 
hold for any $t' \leq t$
Then for $ j_m \le t' \leq j_m + T_0 - 1$
\begin{align*}%\label{xi_multi_20_sgd}
% \|\bH_{t} - \B_{j_m}\| \leq \xi_{j_1,j_m}^S:= c_0 d_{j_1,j_m + T_0 - 1}\left(1+ \frac{\sqrt{m}[(1+a)^{m}-1]}{c_1}\right) 
% + c_0 M_2\frac{r}{n},
&\|\sbHk{k-1}_{t'} - \sBk{k-1}_{j_m}\| \leq \xi_{j_1,j_m}^S(k-1)\\
&:= A d_{j_1,j_m + T_0 - 1}(k-1)
+ A\frac{2}{c_0}\rhboundk{(k-1)} + 3A \sswikbound{k},
\end{align*}
where recall again that $c_0$ is the Lipschitz constant of the Hessian, $A = \frac{c_0\sqrt{m}[(1+a)^{m}-1]}{c_1} + c_0$, $d_{j_1,j_m + T_0 - 1}(k-1)$ is defined in Lemma \ref{lemma: bound_d_j_multi_sgd},
% the maximal gap between the iterates of the SGD algorithm on the full data from $j_1$ to $j_m+T_0-1$ (see equation \eqref{d}), which goes to zero as $t\to\infty$),
  $a$ is a problem dependent constant defined in Theorem \ref{theorem: delta_model_para_bound_multi_sgd}, $c_1$ is the "strong independence" constant from Assumption \eqref{assp: singular_lower_bound}.%, 
\end{corollary}


Based on this, let us derive the bound on $\|\nabla F_i(\isw_t(r))\|$, $\|\ag(\isw_{t}(r)) - \frac{1}{B-\Delta B_{t, r}}\sum_{i\not\in R_r}\nabla F_i(\isw_{t}(r))\|$ and $\|\ag(\isw_{t}(r))\|$

% Note that Lemma \ref{Lemma \ref{Lemma: bound_d_j}} still holds for $d_{j_1, j_m +T_0-1}(r-1)$

\begin{lemma}\label{lemma: gradient_multi_bound_sgd}
If at a given iteration $t$, for all $k < r$, the following inequality holds:
 $$\|\isw_{t}(k) - \isw_{t}(k-1)\| \leq \sswikbound{k},$$ then for all $i=1,2,\dots,n$, the following inequality holds:
$$\|\nabla F_i(\isw_t(r-1))\| \leq \sswikbound{r} Lr + c_2$$
\end{lemma}
\begin{proof}

First of all by using the fact that $$\sswikbound{k} \leq \sswikbound{r}$$ and thus $$\|\isw_{t}(k) - \isw_{t}(k-1)\| \leq \sswikbound{k}\leq \sswikbound{r}.$$

Then by adding and subtracting $\nabla F_i(\isw_t(r-2))$ inside $\|\nabla F_i(\isw_t(r-1))\|$, we get:
% This inequality is derived by induction:
\begin{align*}
    \begin{split}
        & \|\nabla F_i(\isw_t(r-1))\|
         = \|\nabla F_i(\isw_t(r-1)) - \nabla F_i(\isw_t(r-2)) + \nabla F_i(\isw_t(r-2))\|\\
        & \leq \|\nabla F_i(\isw_t(r-1)) - \nabla F_i(\isw_t(r-2))\| + \|\nabla F_i(\isw_t(r-2))\|\\
    \end{split}
\end{align*}

The last inequality uses the triangle inequality. Then by using the Cauchy mean-value theorem, the upper bound on the eigenvalue of the Hessian matrix (i.e. Assumption \ref{assp: strong_convex smooth}) and the bound on $\|\isw_{t}(k) - \isw_{t}(k-1)\|$, the formula above can bounded as:
\begin{align*}
    & = \|\bH_i(\isw_t(r-1) + x(\isw_t(r-2)-\isw_t(r-1)))\cdot (\isw_t(r-1) - \isw_t(r-2))\| + \|\nabla F_i(\isw_t(r-2))\|\\
    & \leq L \sswikbound{r} + \|\nabla F_i(\isw_t(r-2))\|
\end{align*}

Then by applying it recursively, the formula above becomes:
\begin{align*}
    & \leq \sum_{k=1}^{r-1} \sswikbound{r} L + \|\nabla F_i(\isw_t(0))\|\leq \sswikbound{r} Lr + c_2
    % & = \sum_{k=1}^{r} \sswikbound{k} L + c_2 \\
%    & 
\end{align*}

\end{proof}



\begin{lemma}\label{lemma: approximate_vs_real_gradient_bound_sgd_multi}
If at a given iteration $t$ such that $j_m \leq t \leq j_m +T_0 -1$, for all $k < r$, the following inequalities hold:
\begin{enumerate}
\item \label{approximate_vs_real_gradient_bound_sgd_multi_cond1}
\begin{align*}
\|\isw_{t}(k) - \isw_{t}(k-1)\|\leq \sswikbound{k}
\end{align*}
\item \label{approximate_vs_real_gradient_bound_sgd_multi_cond2}
\begin{align*}
\|\sbHk{k-1}_t-\sBk{k-1}_{j_m}\| \leq \xi_{j_1,j_m}^S(k-1)
\end{align*}
\item \label{approximate_vs_real_gradient_bound_sgd_multi_cond3}
\begin{align*}
&\xi_{j_1,j_m}^S(k-1) = \xi_{j_0+xT_0,j_0 + (x+m-1)T_0}(k-1)\\
%& = A d_{j_0+xT_0,j_0 + (x+m)T_0-1}(k-1)
%+ A\frac{2}{c_0}\rhboundk{(k-1)}\\
%&+ 3A \sswikbound{k} \\
&\leq (1-\eta\mu)^{j_0+xT_0}Ad_{0,mT_0-1}(0) + 2Ac_2 \left(\frac{(\log(p+1))^2}{B}\right)^{1/4}+ A\frac{2}{c_0}\rhboundk{(k-1)}\\
& + (2Ak+A)\cdot \sswikbound{k}
%& + 3A \sswikbound{k} \leq \frac{\mu}{2}
\end{align*}
\item \label{approximate_vs_real_gradient_bound_sgd_multi_cond4}
\begin{align*}
& Ad_{0,mT_0-1}(0) + 2Ac_2 \left(\frac{(\log(p+1))^2}{B}\right)^{1/4}+ A\frac{2}{c_0}\rhboundk{(k-1)}\\
& + (2Ak+A)\cdot \sswikbound{k} \leq \frac{\mu}{2}
\end{align*}
\end{enumerate}


then the following inequalities hold:
\begin{align*}
    \begin{split}
        &\|\frac{1}{B-\Delta B_{t, r-1}}\sum_{i\not\in R_{r-1}, i\in \miniB_{t}}\nabla F_i(\isw_t(r-1))-\ag(\isw_t(r-1))\|
         \leq \sswikbound{r}r\mu 
        % & \leq \sum_{k=0}^{r-1}\frac{B-\Delta B_{t, k}}{B-\Delta B_{t, r}}\frac{\mu}{2} (\frac{2n}{n-7k-8}M_1\frac{1}{n} ) := \Delta_r
        % &\leq \sum_{k=1}^r (1+\frac{k}{B-\Delta B_{t, r}})[A d_{j_1,j_m + T_0 - 1}(0)\\
        % & + A (\sum_{l=1}^k (C_{l-1}M_1\frac{1}{n} + D_{l-1}))](\sum_{l=1}^k (C_{l-1}M_1\frac{1}{n} + D_{l-1})):= \Delta_r
    \end{split}
\end{align*}
and 
\begin{align*}
&\|\ag(\isw_t(r-1))\| \leq \sswikbound{r}(r\mu + lr)+ c_2
\end{align*}
\end{lemma}
\begin{proof}
First of all, we rewrite $\frac{1}{B-\Delta B_{t, r-1}}\sum_{i\not\in R_{r-1}, i \in \miniB_t}\nabla F_i(\isw_t(r-1))$ by using the Cauchy mean value theorem as below:
\begin{align*}
\begin{split}
& \frac{1}{B-\Delta B_{t, r-1}}\sum_{i\not\in R_{r-1}, i \in \miniB_t}\nabla F_i(\isw_t(r-1))\\
& = \frac{1}{B-\Delta B_{t, r-1}}[\sum_{i\not\in R_{r-2}, i \in \miniB_t}\nabla F_i(\isw_t(r-1)) - \mathbbm{1}(i_{r-1} \in \miniB_t)\cdot\nabla F_{i_{r-1}}(\isw_t(r-1))]\\
& = \frac{1}{B-\Delta B_{t, r-1}}\{[(B-\Delta B_{t, r-2})(\sbHk{r-2}_{t}\times (\isw_t(r-1) - \isw_t(r-2))]\\
& + \sum_{i\not\in R_{r-2}, i \in \miniB_t}\nabla F_i(\isw_t(r-2))) - \mathbbm{1}(i_{r-1} \in \miniB_t)\cdot\nabla F_{i_{r-1}}(\isw_t(r-1))\}    
\end{split}
\end{align*}



%First of all, let us compute the difference 
%$\frac{1}{B-\Delta B_{t, r-1}}\sum_{i\not\in R_{r-1}}\nabla F_i(\isw_t(r-1))-\ag(\isw_t(r-1))$. For the  use the fact that 

    
Then by computing the norm of the difference between the formula above and equation \eqref{eq: sg_w_k_deriv},
% , i.e. $$\ag(\isw_t(r)) = \frac{1}{B-\Delta B_{t, r}}[(B-\Delta B_{t, r}+1)(\B_{j_m}(\isw_t(r) - \isw_t(r-1)) + \ag(\isw_t(r-1))) - \nabla F_{i_r}(\isw_t(r))]$$
% \ag(\isw_t(r-1)) + \B_{j_m}\times (\isw_t(r) - \isw_t(r-1)),$$ 
we get:
\begin{align*}
\begin{split}
    & \|\frac{1}{B-\Delta B_{t, r-1}}\sum_{i\not\in R_{r-1}, i\in \miniB_t}\nabla F_i(\isw_t(r-1)) - \ag(\isw_t(r-1))\| \\
    & = \frac{1}{B-\Delta B_{t, r-1}}\|(B-\Delta B_{t, r-2})(\sbHk{r-2}_t-\sBk{r-2}_{j_m})\cdot (\isw_t(r-1) - \isw_t(r-2))\\
    & + \sum_{i\not\in R_{r-2}, i\in \miniB_t}\nabla F_i(\isw_t(r-2))- (B-\Delta B_{t, r-2})\ag(\isw_t(r-2)) \|\\
\end{split}
\end{align*}

Then by using the triangle inequality and the fact that $$\|\sbHk{k-1}_t-\sBk{k-1}_{j_m}\| \leq \xi_{j_1,j_m}^S(k-1),$$ the formula above can be bounded as:
\begin{align}\label{eq: real_approx_gradient_gap_deriv1_sgd}
    \begin{split}
        & \leq \frac{B-\Delta B_{t, r-2}}{B-\Delta B_{t, r-1}}\|\sbHk{r-2}_t - \sBk{r-2}_{j_m}\|\|\isw_t(r-1) - \isw_t(r-2)\|\\
        & + \frac{1}{B-\Delta B_{t, r-1}} \|\sum_{i\not\in R_{r-2},i \in \miniB_t}\nabla F_i(\isw_t(r-2)) - (B-\Delta B_{t, r-2})\ag(\isw_t(r-2))\| \\
        & \leq \frac{B-\Delta B_{t, r-2}}{B-\Delta B_{t, r-1}}\xi_{j_1,j_m}^S(r-2) \sswikbound{r}\\
        & + \frac{B-\Delta B_{t, r-2}}{B-\Delta B_{t, r-1}}\|\frac{1}{B-\Delta B_{t, r-2}}\sum_{i\not\in R_{r-2},i \in \miniB_t}\nabla F_i(\isw_t(r-2)) - \ag(\isw_t(r-2))\|
    \end{split}
\end{align}

The combination of Condition \ref{approximate_vs_real_gradient_bound_sgd_multi_cond3} and \ref{approximate_vs_real_gradient_bound_sgd_multi_cond4} tell us that $\xi_{j_1,j_m}^S(r-2) \leq \frac{\mu}{2}$. So the formula above can be bounded as:
\begin{align*}
    & \leq \frac{B-\Delta B_{t, r-2}}{B-\Delta B_{t, r-1}}\frac{\mu}{2} (\sswikbound{r} )\\
        & + \frac{B-\Delta B_{t, r-2}}{B-\Delta B_{t, r-1}}\|\frac{1}{B-\Delta B_{t, r-2}}\sum_{i\not\in R_{r-2},i \in \miniB_t}\nabla F_i(\isw_t(r-2)) - \ag(\isw_t(r-2))\|
\end{align*}

By applying it recursively (Note that $\nabla F(\isw_t(0)) = \ag(\isw_t(0))$). In the end, we get the following inequality:
\begin{align*}
    \begin{split}
        & \leq \sum_{k=1}^{r-1}\frac{B-\Delta B_{t, k}}{B-\Delta B_{t, r}}\frac{\mu}{2} (\sswikbound{k})\\
        & \leq \sswikbound{r}\frac{\mu}{2} \sum_{k=1}^{r-1}\frac{B-\Delta B_{t, k}}{B-\Delta B_{t, r}}
        % ((1+\frac{r}{B-\Delta B_{t, r}})\frac{\mu}{2} + (1+\frac{r-1}{B-\Delta B_{t, r}})\xi_{j_1,j_m}^S(1) + \dots +(1+\frac{1}{B-\Delta B_{t, r}})\xi_{j_1,j_m}^S(r-1)) \\
        % &\cdot (\frac{2n}{n-7k-1}M_1\frac{1}{n} )
    \end{split}
\end{align*}

Also since $\Delta B_{t, r} \ll B$, then $\frac{B-\Delta B_{t, k}}{B-\Delta B_{t, r}} \leq 2$. So the formula above can be bounded as:
\begin{align*}
    \begin{split}
        & \leq \sswikbound{r}r\mu 
    \end{split}
\end{align*}

Based on Lemma \ref{lemma: gradient_multi_bound_sgd}, we know that when condition \ref{approximate_vs_real_gradient_bound_sgd_multi_cond1} holds, the following inequality holds:
$$\|\nabla F_i(\isw_t(r-1))\| \leq \sswikbound{r} Lr + c_2.$$

Then the bound on $\|\ag(\isw_t(r))\|$ can be derived by adding and subtracting $\frac{1}{B-\Delta B_{t, r-1}}\sum_{i\not\in R_{r-1}}\nabla F_i(\isw_t(r-1))$, using triangle inequality and using the bounds on $\|\nabla F_i(\isw_t(r-1))\|$ and $\frac{1}{B-\Delta B_{t, r-1}}\sum_{i\not\in R_{r-1}, i\in \miniB_{t}}\nabla F_i(\isw_t(r-1))-\ag(\isw_t(r-1))$:
%and the bound on $\|\nabla F_i(\isw_t(r-1))\|$ and $\ag(\isw_t(r-1)) - \frac{1}{B-\Delta B_{t, r-1}}\sum_{i\not\in R_{r-1}}\nabla F_i(\isw_t(r-1))$:
\begin{align}\label{eq: approximate_gradient_bound_sgd}
\begin{split}
    \|\ag(\isw_t(r-1))\|
    & = \|\ag(\isw_t(r-1)) - \frac{1}{B-\Delta B_{t, r-1}}\sum_{i\not\in R_{r-1}}\nabla F_i(\isw_t(r-1))\\
    & + \frac{1}{B-\Delta B_{t, r-1}}\sum_{i\not\in R_{r-1}}\nabla F_i(\isw_t(r-1))\|\\
    & \leq \|\ag(\isw_t(r-1)) - \frac{1}{B-\Delta B_{t, r-1}}\sum_{i\not\in R_{r-1}}\nabla F_i(\isw_t(r-1))\|\\
    & + \|\frac{1}{B-\Delta B_{t, r-1}}\sum_{i\not\in R_{r-1}}\nabla F_i(\isw_t(r-1))\|\\
    % & \leq\Delta_r + \sum_{k=0}^{r-1} (\frac{2n}{n-7k-8}M_1\frac{1}{n} ) L + c_2\\
    & = \sswikbound{r}(r\mu + lr) +c_2
%    & + \sswikbound{r} Lr + c_2
\end{split}
\end{align}

% Then based on Lemma \ref{lemma: bound_d_j_multi_sgd}, $$\xi_{j_1,j_m}^S(k) = A d_{j_1,j_m + T_0 - 1}(k)
% + A (\frac{2n}{n-7k-1}M_1\frac{1}{n} )$$
% % $$Ad_{j_a,j_b + T_0 - 1}(0)
% % + A\frac{2Ck}{\frac{1}{2}-\frac{1}{n}}M_1\frac{1}{n}$$
% $$\leq A d_{j_1,j_m + T_0 - 1}(0)
% + A \sum_{l=1}^k (C_{l-1}M_1\frac{1}{n} + D_{l-1}),$$ the formula above can be further bounded as:
% \begin{align}
%     \begin{split}
%         & \leq 
%         \sum_{k=1}^r (1+\frac{k}{B-\Delta B_{t, r}})[A d_{j_1,j_m + T_0 - 1}(0) + (A \sum_{l=1}^k (C_{l-1}M_1\frac{1}{n} + D_{l-1}))]\\
%         & \cdot (\frac{2n}{n-7k-1}M_1\frac{1}{n} ):= \Delta_r\\
%         % & = [(\frac{nr}{B-\Delta B_{t, r}}-\frac{r(r-1)}{2(B-\Delta B_{t, r})})Ad_{j_1,j_m +T_0 - 1}(0)\\
%         % & + (\frac{r(r+1)(2r+1)}{3(B-\Delta B_{t, r})} + r^2 - \frac{r(r+1)}{2(B-\Delta B_{t, r})})A\frac{M_1}{\frac{1}{2}-\frac{1}{n}}\frac{C}{n}]\frac{M_1}{\frac{1}{2}-\frac{1}{n}}\frac{C}{n} 
%     \end{split}
% \end{align}

\end{proof}

Note that for $\|\frac{1}{B-\Delta B_{t, r-1}}\sum_{i\not\in R_{r-1},i \in \miniB_t}\nabla F_i(\isw_t(r-1))-\ag(\isw_t(r-1))\|$, we get a tighter bound when $t\rightarrow \infty$ by using equation \eqref{eq: real_approx_gradient_gap_deriv1_sgd}, Lemma \ref{lemma: bound_d_j_multi_sgd} (i.e. $d_{a,b}(r) \leq d_{a,b}(0) + 2r\cdot \sswikbound{r} \leq (1-\eta\mu)^{a}d_{0,b-a}(0) + 2c_2 \left(\frac{(\log(p+1))^2}{B}\right)^{1/4}+ 2r\cdot \sswikbound{r}$) without using $\xi_{j_1,j_m}^S(r-1) \leq \frac{\mu}{2}$, which ends up with condition \ref{approximate_vs_real_gradient_bound_sgd_multi_cond3} in Lemma \ref{lemma: approximate_vs_real_gradient_bound_sgd_multi}:
%starts by bounding $\xi_{j_1,j_m}^S(k-1)$ where $k \leq r$, $j_1 = j_0 + xT_0$ and $j_m = j_0 + (x+m-1)T_0$:

\begin{align}\label{eq: xi_bound_multi_sgd}
    \begin{split}
    & \xi_{j_1,j_m}^S(k-1) = \xi_{j_0 + xT_0,j_0 + (x+m-1)T_0}^S(k-1)\\
%     = A d_{j_0+xT_0,j_0 + (x+m)T_0-1}(k-1) + A\frac{2}{c_0}\rhboundk{(k-1)}\\
%& + 3A \sswikbound{k}\\
%& \leq A d_{j_0+xT_0,j_0 + (x+m)T_0-1}(0)+ A\frac{2}{c_0}\rhboundk{(k-1)}\\
%& + 2(k-1)A \cdot \sswikbound{k}\\
%& + 3A \sswikbound{k}\\
& \leq A (1-\mu\eta)^{j_0 + xT_0}d_{0,mT_0-1}(0)+ A\frac{2}{c_0}\rhboundk{(k-1)}\\
& + (2Ak + A)\sswikbound{k}\\
%& + 3A \sswikbound{k}\\
    \end{split}
\end{align}

Note that the inequality in Lemma \ref{lemma: bound_d_j_multi_sgd} holds with the probability higher than $1- (t+1)\Psi_3(1)$ for any $a < b \leq t$ when the bound on $\|\isw_{t'}(k)-\isw_{t'}(k-1)\|$ holds. Then with the same probability and the same bounds on $\|\isw_{t'}(k)-\isw_{t'}(k-1)\|$, the formula above holds for any $t' \leq t$ and $j_m \leq t' \leq j_m + T_0 - 1$.

Then by plugging equation \eqref{eq: xi_bound_multi_sgd} into equation \eqref{eq: real_approx_gradient_gap_deriv1_sgd} and using the same derivation as equation \eqref{eq: real_approx_gradient_gap_tight}, we get:
\begin{align}\label{eq: real_approx_gradient_gap_tight_sgd}
    \begin{split}
        & \|\frac{1}{B-\Delta B_{t, r-1}}\sum_{i\not\in R_{r-1}, i \in \miniB_t}\nabla F_i(\isw_t(r-1))-\ag(\isw_t(r-1))\| \\
%        & \leq \frac{B-\Delta B_{t, r-2}}{B-\Delta B_{t, r-1}}\xi_{j_1,j_m}^S(r-2) \sswikbound{r}\\
%        & + \frac{B-\Delta B_{t, r-2}}{B-\Delta B_{t, r-1}}\|\frac{1}{B-\Delta B_{t, r-2}}\sum_{i\not\in R_{r-2}}\nabla F_i(\isw_t(r-2)) - \ag(\isw_t(r-2))\|\\
%        & \leq \sum_{k=1}^{r-1} \xi_{j_1,j_m}^S(k-1)\sswikbound{k}\\
%        & \leq \sum_{k=1}^{r-1}(A (1-\mu\eta)^{j_0 + xT_0}d_{0,mT_0-1}(0) + A(2k-1)\sswikbound{k}\\
%& + 3A \sswikbound{k} + A\frac{2}{c_0}\rhboundk{(k-1)})\\
%        & \cdot\sswikbound{k}\\
        & \leq [A (1-\mu\eta)^{j_0 + xT_0}d_{0,mT_0-1}(0)r+ Ar\frac{2}{c_0}]
         \cdot \sswikbound{r}\\
        & + A (r^2 + r)(\sswikbound{r})^2\\
%        &  + 3Ar (\sswikbound{r})^2
%        & \rhboundk{(r-1)}\sswikbound{r}
    \end{split}
\end{align}

%The last step uses the fact that $\sswikbound{k} \leq \sswikbound{r}$, $\sum_{k=1}^{r-1} (2k-1) < \sum_{k=1}^r (2k-1) = r^2$ and $\rhboundk{(k-1)} \leq \rhboundk{(r-1)}$. 
So when $t\rightarrow \infty$ and thus $x \rightarrow \infty$, $\|\frac{1}{B-\Delta B_{t, r}}\sum_{i\not\in R_r}\nabla F_i(\isw_t(r))-\ag(\isw_t(r))\| = o(\frac{r}{n} +\frac{r}{(B-r+1)^{\frac{1}{4}}})$

%Based on Lemma \ref{lemma: gradient_multi_bound_sgd} and \ref{lemma: approximate_vs_real_gradient_bound_sgd_multi}, the bound on $\|\ag(\isw_t(r))\|$ is:
%\begin{align}\label{eq: approximate_gradient_bound_sgd}
%\begin{split}
%    & \|\ag(\isw_t(r-1))\|\\
%    & = \|\ag(\isw_t(r-1)) - \frac{1}{B-\Delta B_{t, r-1}}\sum_{i\not\in R_{r-1}}\nabla F_i(\isw_t(r-1))\\
%    & + \frac{1}{B-\Delta B_{t, r-1}}\sum_{i\not\in R_{r-1}}\nabla F_i(\isw_t(r-1))\|\\
%    & \leq \|\ag(\isw_t(r-1)) - \frac{1}{B-\Delta B_{t, r-1}}\sum_{i\not\in R_{r-1}}\nabla F_i(\isw_t(r-1))\|\\
%    & + \|\frac{1}{B-\Delta B_{t, r-1}}\sum_{i\not\in R_{r-1}}\nabla F_i(\isw_t(r-1))\|\\
%    % & \leq\Delta_r + \sum_{k=0}^{r-1} (\frac{2n}{n-7k-8}M_1\frac{1}{n} ) L + c_2\\
%    & = \sswikbound{r}r\mu \\
%    & + \sswikbound{r} Lr + c_2
%\end{split}
%\end{align}

\textbf{Main results}

\begin{theorem}[Bound between iterates on full data and incrementally updated ones]\label{bfi_multi_sgd}
% Suppose that for some given $t$ we have the bounds $\|\bH_{t'} - \B_{j_m}\| \leq \xi_{j_1,j_m}^S$, and $\xi_{j_1,j_m}^S \leq (1-r/n)\mu - \beta$  for all possible values of $t'\le t$ and the  $j_1,\ldots,j_m$ corresponding to $t'$ (i.e., not just for the current values at $t$), for some positive $\beta>0$
% Then 
% $$\|\isw_{t+1} - \sw_{t+1} \| \leq M_2 \frac{r}{n}$$ 
% where $M_2=\max(2c_2/\beta,M_1)$ is some positive constant, and recall that $M_1$ is defined in Theorem \ref{wu}. Neither depends on $t$.
Suppose that there are $T$ iterations in total at each deletion request to update the model parameters and the following conditions hold at the $t_{th}$ iteration at the $r_{th}$ deletion request:
 
%\begin{enumerate}
%\item \label{bfi_multi_sgd_cond1}
%\begin{align*}
%\|\isw_{t'}(k) - \isw_{t'}(k-1)\|\leq \sswikbound{k}
%\end{align*}
%\item \label{bfi_multi_sgd_cond2}
%\begin{align*}
%\|\sbHk{k-1}_{t'}-\sBk{k-1}_{j_m}\| \leq \xi_{j_1,j_m}^S(k-1)
%\end{align*}
%\item \label{bfi_multi_sgd_cond3}
%\begin{align*}
%&\xi_{j_1,j_m}^S(k-1) = \xi_{j_0+xT_0,j_0 + (x+m-1)T_0}(k-1)\\
%%& = A d_{j_0+xT_0,j_0 + (x+m)T_0-1}(k-1)
%%+ A\frac{2}{c_0}\rhboundk{(k-1)}\\
%%&+ 3A \sswikbound{k} \\
%&\leq (1-\eta\mu)^{j_0+xT_0}Ad_{0,mT_0-1}(0) + 2Ac_2 \left(\frac{(\log(p+1))^2}{B}\right)^{1/4}+ A\frac{2}{c_0}\rhboundk{(k-1)}\\
%& + (2Ak+A)\cdot \sswikbound{k}
%%& + 3A \sswikbound{k} \leq \frac{\mu}{2}
%\end{align*}
%\item \label{bfi_multi_sgd_cond4}
%\begin{align*}
%& Ad_{0,mT_0-1}(0) + 2Ac_2 \left(\frac{(\log(p+1))^2}{B}\right)^{1/4}+ A\frac{2}{c_0}\rhboundk{(k-1)}\\
%& + (2Ak+A)\cdot \sswikbound{k} \leq \frac{\mu}{2}
%\end{align*}
%
%
%
%\item \label{bfi_multi_sgd_cond5} 
%$$\frac{\Delta B_{t'}-\Delta B_{t',r-1}}{B-\Delta B_{t',r-1}} \leq \frac{1}{n} + \frac{1}{(B-r+1)^{1/4}}$$
%\end{enumerate} 
 
\begin{enumerate}
\item \label{bfi_multi_sgd_cond1} $\|\isw_{t'}(k) - \isw_{t'}(k-1)\| \leq \sswikbound{k}$ holds for all $k < r$, $t' \leq T$;
\item \label{bfi_multi_sgd_cond2} $\|\sbHk{k-1}_{t'} - \sBk{k-1}_{j_m}\| \leq \xi_{j_1,j_m}^S(k-1)$ holds for all $t' \leq T$ for all $k < r$ and for all $t' \leq t$ for $k = r$;
\item \label{bfi_multi_sgd_cond3}
\begin{align*}
&\xi_{j_1,j_m}^S(k-1) = \xi_{j_0+xT_0,j_0 + (x+m-1)T_0}(k-1)\\
%& = A d_{j_0+xT_0,j_0 + (x+m)T_0-1}(k-1)
%+ A\frac{2}{c_0}\rhboundk{(k-1)}\\
%&+ 3A \sswikbound{k} \\
&\leq (1-\eta\mu)^{j_0+xT_0}Ad_{0,mT_0-1}(0) + 2Ac_2 \left(\frac{(\log(p+1))^2}{B}\right)^{1/4}+ A\frac{2}{c_0}\rhboundk{(k-1)}\\
& + (2Ak+A)\cdot \sswikbound{k}
%& + 3A \sswikbound{k} \leq \frac{\mu}{2}
\end{align*}
holds for all $t' \leq T$ such that $j_m \leq t' \leq j_m +T_0 - 1$ for all $k < r$ and for all $t' \leq t$ such that $j_m \leq t' \leq j_m +T_0 - 1$ for $k = r$;
\item \label{bfi_multi_sgd_cond4} for all $k \leq r$,
\begin{align*}
& Ad_{0,mT_0-1}(0) + 2Ac_2 \left(\frac{(\log(p+1))^2}{B}\right)^{1/4}+ A\frac{2}{c_0}\rhboundk{(k-1)}\\
& + (2Ak+A)\cdot \sswikbound{k} \leq \frac{\mu}{2}
\end{align*}
\item \label{bfi_multi_sgd_cond5} $$\frac{\Delta B_{t'}-\Delta B_{t',k-1}}{B-\Delta B_{t',k-1}} \leq \frac{1}{n} + \frac{1}{(B-k+1)^{1/4}}$$holds for all $t' \leq T$ for all $k < r$ and for all $t' \leq t$ for $k = r$;
\end{enumerate} 

%and at the $r_{th}$ deletion request, the following inequalities holds for all $t' \leq t$ and $j_m \leq t' \leq t'+T_0-1$:
%$$\|\sbHk{r-1}_{t'} - \sBk{r-1}_{j_m}\| \leq \xi_{j_1,j_m}^S(r-1)$$
 
%
% $$= A d_{j_0+xT_0,j_0 + (x+m)T_0-1}(r-1) + A\frac{2}{c_0}\rhboundk{(r-1)}$$
%$$+ 3A \sswikbound{r} $$ (where we recalled the definition of $\xi^S$)  and
%\begin{align*}
%    \begin{split}
%       &\xi_{j_1,j_m}^S(k-1) = \xi_{j_0+xT_0,j_0 + (x+m-1)T_0}^S(k-1)\\
%&= A d_{j_0+xT_0,j_0 + (x+m)T_0-1}(k-1)
%+ A\frac{2}{c_0}\rhboundk{(k-1)}\\
%& + 3A \sswikbound{k}\\
%&\leq Ad_{0,mT_0-1}(0)+ A\frac{2}{c_0}\rhboundk{(k-1)}+ 2Ac_2 \left(\frac{(\log(p+1))^2}{B}\right)^{1/4}\\
%&+ 2Ar\cdot \sswikbound{r}\\
%& + 3A \sswikbound{k} \leq \frac{\mu}{2}
%    \end{split}
%\end{align*}
%% for all iterations $x$
%and 

%for all $t' \leq t$
% and the  $j_1,\ldots,j_m$ corresponding to $t'$ (i.e., not just for the current values at $t$). % \ed{Need to double check that this is the right condition}. 
Then %for all $t$  $j_m \leq t \leq j_m + T_0$, 
$$\|\isw_{t'+1}(r) - \isw_{t'+1}(r-1) \| \leq
% \frac{2 c_2/n}{(1-1/n)\mu - \xi_{j_0,j_0+(m-1)T_0}(k-1)} \leq 
\sswikbound{r}.$$ 
% $$\|\isw_{t+1} - \sw_{t+1} \| \leq \frac{2r c_2/n}{(1-r/n)\mu - \xi_{j_1,j_m}^S}$$
% where $M_2=M_1 +  $ is some positive constant, and
Recall that $c_0$ is the Lipshitz constant of the Hessian, $M_1$ and $A$ are defined in Theorem \ref{wu_sgd_multi} and Corollary \ref{lemma: corollary: approx_hessian_real_hessian_bound_multi_sgd} respectively, and do not depend on $t$, 
\end{theorem}


Then by using the same proof techniques as Theorem \ref{bfi2_sgd}, we get the following results at the $r_{th}$ deletion request.

%\begin{theorem}[Bound between iterates on full data and incrementally updated ones (all iterations, online deletion)]\label{bfi2_multi_sgd}
%At deletion request $r$, suppose that there are $T$ iterations in total, if for all $k<r$ and $t<T$, $\|\isw_t(k)-\isw_t(k-1)\| \leq \sswikbound{k}$ holds, then for any $j_m \leq t \leq j_m +T_0 - 1$, with probability higher than $$1-T\times (\Psi_2(r) + $$
%$$\Psi_3(r) + \Psi_1(r)),$$ the following inequalities hold:
% $$\|\isw_t(r)-\isw_t(r-1)\| \leq \sswikbound{r}$$ and $$\|\sbHk{r-1}_{t} - \sBk{r-1}_{j_m}\| \leq \xi_{j_1,j_m}^S(r-1)$$
%$$:= A d_{j_1,j_m + T_0 - 1}(r-1)
%+ A \sswikbound{r}$$ 
%and $$\|\frac{1}{B-\Delta B_{t, r-1}}\sum_{i\not\in R_{r-1}}\nabla F_i(\isw_t(r-1))-\ag(\isw_t(r-1))\|\leq$$
%$$ \sswikbound{r}r\mu $$
%hold
%% the result $\isw_t$ of Algorithm \ref{alg: update_algorithm} approximates the correct iteration values $\usw_t$ at the rate 
%% $\|\isw_t - \sw_t\| \leq \frac{1}{\frac{1}{2}-\frac{r}{n}}M_1\frac{r}{n}$ and $\|\bH_{t} - \B_{j_m}\| \leq \xi_{j_1,j_m}^S$. 
%% Recall that $j_1,\ldots,j_m$ depend on $t$,  $\xi_{j_1,j_m}^S$ is defined in \eqref{xi} and $M_3$ is the constant from Theorem \ref{main10}.
%\end{theorem}

%The proof is very similar to that of Theorem \ref{bfi2_sgd}.
%
%
%Then by induction (the base case is similar to Theorem \ref{bfi2_sgd}), we should know that the following theorem holds:
\begin{theorem}[Bound between iterates on full data and incrementally updated ones (all iterations, all deletion requests, online deletion SGD)]\label{bfi2_multi_all_sgd}
Suppose that there are $T$ iterations in total at each deletion request, then for any $k \leq r$, $t<T$ and $j_m < t < j_m +T_0 - 1$, with probability higher than $1-T \times\Psi_3(1) - rT(\Psi_2(r) + \Psi_1(r))$, the following inequalities hold:
$$\|\isw_t(k)-\isw_t(k-1)\| \leq \sswikbound{k}$$ and $$\|\sbHk{k-1}_{t} - \sBk{k-1}_{j_m}\| \leq \xi_{j_1,j_m}^S(k-1)$$
and 
$$\|\frac{\sum_{i\not\in R_{k-1}}\nabla F_i(\isw_t(k-1))-\ag(\isw_t(k-1))}{B-\Delta B_{t, k-1}}\| 
\leq 
\sswikbound{k}r\mu $$
hold
% the result $\isw_t$ of Algorithm \ref{alg: update_algorithm} approximates the correct iteration values $\usw_t$ at the rate 
% $\|\isw_t - \sw_t\| \leq \frac{1}{\frac{1}{2}-\frac{r}{n}}M_1\frac{r}{n}$ and $\|\bH_{t} - \B_{j_m}\| \leq \xi_{j_1,j_m}^S$. 
% Recall that $j_1,\ldots,j_m$ depend on $t$,  $\xi_{j_1,j_m}^S$ is defined in \eqref{xi} and $M_3$ is the constant from Theorem \ref{main10}.
\end{theorem}

By induction, the following inequality holds:
\begin{align*}
\begin{split}
   & \|\isw_t(k)-\isw_t(0)\| = \|\isw_t(k)-\sw_t\|
   \leq k \cdot \sswikbound{k}
\end{split}    
\end{align*}

Then by using equation \eqref{eq: w_u_w_gap_sgd}, the following inequality holds:
\begin{align}\label{eq: w_u_w_i_prev_bound_sgd}
    \begin{split}
    &\|\usw_t(k) - \isw_t(k-1)\| = \|\usw_t(k) - \sw_t + \sw_t - \isw_t(k-1)\|\\
    & \leq \|\usw_t(k) - \sw_t\| + \|\sw_t - \isw_t(k-1)\| \\
    & \leq M_1 (\frac{k}{n} + \frac{k}{(B-k+1)^{1/4}}) + (k-1)\cdot \sswikbound{k}\\
    & = M_1 (\frac{k}{n} + \frac{k}{(B-k+1)^{1/4}}) + \frac{k-1}{k}\cdot (\frac{k}{n} + \frac{k}{(B-k+1)^{1/4}})\\
    & \leq M_1 (\frac{k}{n} + \frac{k}{(B-k+1)^{1/4}}) + (\frac{k}{n} + \frac{k}{(B-k+1)^{1/4}})\\
    & := M_2 (\frac{k}{n} + \frac{k}{(B-k+1)^{1/4}})
    \end{split}
\end{align}

where $M_2$ is a constant which does not depend on $t$.

In the end, we get a similar results for the bound on $\|\isw_t(k) - \usw_t(k)\|$:
\begin{theorem}
[Convergence rate of \Increm\ (online deletion)]\label{main10_multi_sgd}
% Suppose 
% $\xi_{j_0,j_0+(m-1)T_0} \leq \min\{\frac{\mu}{2}, (1-\frac{r}{n})\mu - \frac{c_0M_1 r(B-\Delta B_{t, r})}{2n^2}\}$ (recall $\xi$ was defined in \eqref{xi}) for all $t$ 
Suppose that there are $T$ iterations in total at each deletion request, then for all deletion requests $k \leq r$, all iterations $t<T$, the result $\isw_t(k)$ approximates the correct iteration values $\usw_t$ at the rate
$$\|\usw_t(k) - \isw_t(k)\| = o(\frac{k}{n} + \frac{k}{(B-k+1)^{1/4}})$$ with probability higher than $1-T \times\Psi_3(1) - rT(\Psi_2(r) + \Psi_1(r))$
$$\|\usw_t(k) - \isw_t(k)\| = o(\frac{k}{n} + \frac{k}{(B-k+1)^{1/4}}).$$
So $\|\usw_t(k) - \isw_t(k)\|$ is of a lower order than $\frac{k}{n} + \frac{k}{(B-k+1)^{1/4}}$.
% Here $M_3$ is a problem dependent constant that does not depend on $t$.
\end{theorem}



\textbf{The proof of Theorem \ref{bfi_multi_sgd}}
\begin{proof}

Note that the approximated update rules for $\isw_{t}$ at the $r_{th}$ and the $(r-1)_{th}$ deletion request are:
\begin{align}\label{eq: update_rule_w_it_curr_sgd}
\begin{split}
    & \isw_{t+1}(r) = \isw_t(r) - \frac{\eta}{B-\Delta B_{t, r}}[(B-\Delta B_{t, r-1})(\B_{j_m}^{r-1}(\isw_t(r) - \isw_t(r-1))\\
    & + \ag(\isw_{t}(r-1))) - \mathbbm{1}(i_{r} \in \miniB_t)\cdot\nabla F_{i_r}(\isw_t(r))]
\end{split}
\end{align}

and 
\begin{align}\label{eq: update_rule_w_it_prev0_sgd}
\begin{split}
     \isw_{t+1}(r-1) = \isw_{t}(r-1)
    & - \frac{\eta}{B-\Delta B_{t, r-1}}\{(B-\Delta B_{t, r-2})[\sBk{r-2}_{j_m}(\isw_t(r-1) - \isw_t(r-2))\\
    & + \ag(\isw_{t}(r-2))] - \mathbbm{1}(i_{r-1} \in \miniB_t)\cdot\nabla F_{i_{r-1}}(\isw_t(r-1))\}
\end{split}
\end{align}

Note that since $$\ag(\isw_t(r-1)) = \frac{1}{B-\Delta B_{t, r-1}}[(B-\Delta B_{t, r-2})(\sBk{r-2}_{j_m}(\isw_t(r-1) - \isw_t(r-2))$$
$$+ \ag(\isw_t(r-2))) - \mathbbm{1}(i_{r-1} \in \miniB_t)\cdot\nabla F_{i_{r-1}}(\isw_t(r-1))]$$
Then equation \eqref{eq: update_rule_w_it_prev0_sgd} can be rewritten as:
\begin{align}\label{eq: update_rule_w_it_prev_sgd}
    \begin{split}
     \isw_{t+1}(r-1) = \isw_{t}(r-1)
    & - \frac{\eta}{B-\Delta B_{t, r-1}}[(B-\Delta B_{t, r-2})(\sBk{r-2}_{j_m}(\isw_t(r-1) - \isw_t(r-2))\\
    & + \ag(\isw_{t}(r-2))) - \mathbbm{1}(i_{r-1} \in \miniB_t)\cdot\nabla F_{i_{r-1}}(\isw_t(r-1))]\\
    & = \isw_{t}(r-1) - \eta \ag(\isw_t(r-1))
\end{split}
\end{align}

Then we subtract equation \eqref{eq: update_rule_w_it_prev0_sgd} from equation \eqref{eq: update_rule_w_it_prev_sgd}, the result will be:

\begin{align*}
\begin{split}
     \isw_{t+1}(r) - \isw_{t+1}(r-1) 
    & = (\isw_{t}(r) - \isw_{t}(r-1)) - \\
    & \frac{\eta}{B-\Delta B_{t, r}}[(B-\Delta B_{t, r-1})(\B_{j_m}^{r-1}(\isw_t(r) - \isw_t(r-1))\\
    & + \ag(\isw_{t}(r-1))) - \mathbbm{1}(i_{r} \in \miniB_t)\cdot\nabla F_{i_r}(\isw_t(r))] + \eta \ag(\isw_t(r-1))
\end{split}
\end{align*}

Then by adding and subtracting $\sbHk{r-1}_t$ and $\frac{1}{B-\Delta B_{t, r-1}}\sum_{i\not\in R_{r-1}}\nabla F(\isw_t(r-1))$ in the formula above and rearranging the result properly, it becomes:
\begin{align}\label{eq: w_i_t_prev_curr_gap_1_sgd}
\begin{split}
    & \isw_{t+1}(r) - \isw_{t+1}(r-1) \\
    & = (\textbf{I} - \eta\frac{B-\Delta B_{t, r-1}}{B-\Delta B_{t, r}}(\B_{j_m}^{r-1} - \sbHk{r-1}_t))(\isw_{t}(r) - \isw_{t}(r-1))\\
    & - \frac{\eta}{B-\Delta B_{t, r}}[(B-\Delta B_{t, r-1})(\sbHk{r-1}_t(\isw_t(r) - \isw_t(r-1))\\
    & + \frac{1}{B-\Delta B_{t, r-1}}\sum_{i\not\in R_{r-1}, i \in \miniB_t}\nabla F(\isw_t(r-1)) - \frac{1}{B-\Delta B_{t, r-1}}\sum_{i\not\in R_{r-1}, i \in \miniB_t}\nabla F(\isw_t(r-1)) \\
    & + \ag(\isw_{t}(r-1))) - \mathbbm{1}(i_{r} \in \miniB_t)\cdot\nabla F_{i_r}(\isw_t(r))] + \eta \ag(\isw_t(r-1))\\
\end{split}
\end{align}


Then by using the fact that 
\begin{align*}
    & \sbHk{r-1}_t(\isw_t(r) - \isw_t(r-1)) + \frac{1}{B-\Delta B_{t, r-1}}\sum_{i\not\in R_{r-1}, i \in \miniB_t}\nabla F(\isw_t(r-1))\\
    & = \frac{1}{B-\Delta B_{t, r-1}}\sum_{i\not\in R_{r-1}, i \in \miniB_t}\nabla F(\isw_t(r))
\end{align*}

and $$\sum_{i\not\in R_{r-1}, i \in \miniB_t}\nabla F(\isw_t(r))) - \mathbbm{1}(i_r \in \miniB_t)\cdot\nabla F_{i_r}(\isw_t(r)
= 
\sum_{i\not\in R_{r}, i \in \miniB_t}\nabla F(\isw_t(r))$$

equation \eqref{eq: w_i_t_prev_curr_gap_1_sgd} becomes:
\begin{align}\label{eq: w_i_t_prev_curr_gap_2_sgd}
\begin{split}
     \isw_{t+1}(r) - \isw_{t+1}(r-1) 
    & = (\textbf{I} - \eta\frac{B-\Delta B_{t, r-1}}{B-\Delta B_{t, r}}(\B_{j_m}^{r-1} - \sbHk{r-1}_t))(\isw_{t}(r) - \isw_{t}(r-1))\\
    & - \frac{\eta}{B-\Delta B_{t, r}}[\sum_{i\not\in R_{r}}\nabla F(\isw_t(r)) - \sum_{i\not\in R_{r-1}}\nabla F(\isw_t(r-1)) \\
    & + (B-\Delta B_{t, r-1})\ag(\isw_{t}(r-1))] + \eta \ag(\isw_t(r-1))\\
\end{split}
\end{align}

Also note that 
\begin{align*}
    \begin{split}
        & \sum_{i\not\in R_{r}, i \in \miniB_t}\nabla F_i(\isw_t(r)) - \sum_{i\not\in R_{r-1}, i \in \miniB_t}\nabla F_i(\isw_t(r-1)) \\
        & = \sum_{i\not\in R_{r}, i \in \miniB_t}\nabla F_i(\isw_t(r)) - \sum_{i\not\in R_{r}, i \in \miniB_t}\nabla F_i(\isw_t(r-1)) - \mathbbm{1}(i_r \in \miniB_t)\cdot\nabla F_{i_r}(\isw_t(r-1)) \\
        & = [\sum_{i \not\in R_r, i \in \miniB_t} \int_0^1 \bH_i(\isw_{t}(r-1) + x (\isw_{t}(r) - \isw_{t}(r-1)))dx](\isw_t(r)-\isw_t(r-1))\\
        & - \mathbbm{1}(i_r \in \miniB_t)\cdot\nabla F_{i_r}(\isw_t(r-1))
    \end{split}
\end{align*}

which can be plugged into equation \eqref{eq: w_i_t_prev_curr_gap_2_sgd}, i.e.:
\begin{align}\label{eq: w_i_t_prev_curr_gap_3_sgd}
\begin{split}
    & \isw_{t+1}(r) - \isw_{t+1}(r-1) \\
    & = (\textbf{I} - \eta\frac{B-\Delta B_{t, r-1}}{B-\Delta B_{t, r}}(\B_{j_m}^{r-1} - \sbHk{r-1}_t))(\isw_{t}(r) - \isw_{t}(r-1))\\
    & - \frac{\eta}{B-\Delta B_{t, r}}\{[\sum_{i \not\in R_r, i \in \miniB_t} \int_0^1 \bH_i(\isw_{t}(r-1) + x (\isw_{t}(r) - \isw_{t}(r-1)))dx]\\
    & \cdot (\isw_{t}(r) - \isw_{t}(r-1)) - \mathbbm{1}(i_r \in \miniB_t)\cdot\nabla F_{i_r}(\isw_t(r-1))\\
    & + (B-\Delta B_{t, r-1})\ag(\isw_{t}(r-1))\} + \eta \ag(\isw_t(r-1))\\
\end{split}
\end{align}

which can be rearranged as:
\begin{align}\label{eq: w_i_t_prev_curr_gap_4_sgd}
\begin{split}
    & \isw_{t+1}(r) - \isw_{t+1}(r-1) \\
    & = (\textbf{I} - \eta\frac{B-\Delta B_{t, r-1}}{B-\Delta B_{t, r}}(\B_{j_m}^{r-1} - \sbHk{r-1}_t))(\isw_{t}(r) - \isw_{t}(r-1))\\
    & - \frac{\eta}{B-\Delta B_{t, r}}\{[\sum_{i \not\in R_r, i \in \miniB_t} \int_0^1 \bH_i(\isw_{t}(r-1) + x (\isw_{t}(r) - \isw_{t}(r-1)))dx]\\
    & \cdot (\isw_{t}(r) - \isw_{t}(r-1)) - \mathbbm{1}(i_r \in \miniB_t)\cdot\nabla F_{i_r}(\isw_t(r-1))\}\\
    & - \frac{\eta(\Delta B_{t, r} - \Delta B_{t, r-1})}{B-\Delta B_{t, r}}\ag(\isw_t(r-1))\\
\end{split}
\end{align}

Then by taking the matrix norm on both sides of the equation in equation \eqref{eq: w_i_t_prev_curr_gap_4_sgd} and using the fact that $\|\bH_i(\isw_{t}(r-1) + x (\isw_{t}(r) - \isw_{t}(r-1)))\| \geq \mu$ and $\|\B_{j_m}^{r-1} - \sbHk{r-1}_t\| \leq \xi_{j_1,j_m}^S(r-1)$, equation \eqref{eq: w_i_t_prev_curr_gap_4_sgd} can be bounded as:
\begin{align*}
    \begin{split}
        \|\isw_{t+1}(r) - \isw_{t+1}(r-1)\|
        & \leq (1-\eta\mu)\|\isw_{t}(r) - \isw_{t}(r-1)\| \\
        & + \frac{(B-\Delta B_{t, r-1})\eta}{B-\Delta B_{t, r}}\xi_{j_1,j_m}^S(r-1)\|\isw_{t}(r) - \isw_{t}(r-1)\|\\
        & + \frac{\eta}{B-\Delta B_{t, r}}\|\mathbbm{1}(i_r \in \miniB_t)\cdot\nabla F_{i_r}(\isw_t(r-1))\|\\
        & + \|\frac{\eta(\Delta B_{t,r} - \Delta B_{t,r-1})}{B-\Delta B_{t, r}}\ag(\isw_t(r-1))\|\\
    \end{split}
\end{align*}

Then by using condition \ref{bfi_multi_sgd_cond5}, i.e.: $$\frac{\Delta B_{t', k}-\Delta B_{t',k-1}}{B-\Delta B_{t',k-1}} = \frac{\mathbbm{1}(i_{k} \in \miniB_{t'})}{B-\Delta B_{t',k-1}} \leq \frac{1}{n} + \frac{1}{(B-k+1)^{1/4}} \leq \frac{1}{n} + \frac{1}{(B-r+1)^{1/4}}$$ for all $t' \leq t$, the formula above can be bounded as:
\begin{align*}
    \begin{split}
         \|\isw_{t+1}(r) - \isw_{t+1}(r-1)\|
        & \leq (1-\eta\mu)\|\isw_{t}(r) - \isw_{t}(r-1)\| \\
        & + \eta(1 + \frac{1}{n} + \frac{1}{(B-r+1)^{1/4}})\xi_{j_1,j_m}^S(r-1)\|\isw_{t}(r) - \isw_{t}(r-1)\|\\
        & + \eta(\frac{1}{n} + \frac{1}{(B-r+1)^{1/4}})\|\nabla F_{i_r}(\isw_t(r-1))\|\\
        & + \eta(\frac{1}{n} + \frac{1}{(B-r+1)^{1/4}})\|\ag(\isw_t(r-1))\|\\
    \end{split}
\end{align*}

Also note that when condition \ref{bfi_multi_sgd_cond1}-\ref{bfi_multi_sgd_cond4} hold,  Lemma \ref{lemma: gradient_multi_bound_sgd} and Lemma \ref{lemma: approximate_vs_real_gradient_bound_sgd_multi} hold. 
Then by using the bound on $\|\nabla F_{i_r}(\isw_t(r-1))\|$ and $\|\ag(\isw_t(r-1))\|$ from the two lemmas, the formula above is bounded as:
\begin{align*}
    & \leq (1-\eta\mu + \eta(1 + \frac{1}{n} + \frac{1}{(B-r+1)^{1/4}})\xi_{j_1,j_m}^S(r))\|\isw_{t}(r) - \isw_{t}(r-1)\|\\
        & + \eta(\frac{1}{n} + \frac{1}{(B-r+1)^{1/4}})[\sswikbound{r} L(r-1) + c_2]\\
        & + \eta(\frac{1}{n} + \frac{1}{(B-r+1)^{1/4}})[\sswikbound{r}(r-1)(\mu+L) + c_2]
\end{align*}

%Then by using the fact that $$\frac{\Delta B_{t', k}-\Delta B_{t',k-1}}{B-\Delta B_{t',k-1}} \leq \frac{1}{n} + \frac{1}{(B-k+1)^{1/4}}$$ and $B-\Delta B_{t',k} \leq B-r$ for all $t' \leq t$, the formula above can be bounded as:
%
%\begin{align*}
%    & \leq (1-\eta\mu + \eta(1+\frac{1}{n} + \frac{1}{(B-r+1)^{1/4}})\xi_{j_1,j_m}^S(r))\|\isw_{t}(r) - \isw_{t}(r-1)\|\\
%        & + \frac{\eta}{B-r}(\sswikbound{r} L(r-1) + c_2)\\
%        & + \frac{\eta}{B-r}(\sswikbound{r}(r-1)\mu + \sswikbound{r} L(r-1) + c_2)
%\end{align*}

Also when condition \ref{bfi_multi_sgd_cond4} and \ref{bfi_multi_sgd_cond5} hold, we know that $\xi_{j_1,j_m}^S(r) \leq \frac{\mu}{2}$ for all $j_m \leq t' \leq j_m +T_0 - 1$. Then by using the bound for $\xi_{j_1,j_m}^S(r)$ and applying the above formula recursively across all the iterations, the formula above becomes:
\begin{align*}
    \begin{split}
    & \leq \frac{1}{\eta\mu - \eta(1+\frac{1}{n} + \frac{1}{(B-r+1)^{1/4}})\frac{\mu}{2}}(\eta(\frac{1}{n} + \frac{1}{(B-r+1)^{1/4}})\\
    & \cdot(\sswikbound{r} (2L+\mu)(r-1) + c_2)\\
%    & + \eta(\frac{1}{n} + \frac{1}{(B-r+1)^{1/4}})(\sswikbound{r} L(r-1)\\
%    & + \sswikbound{r} \mu (r-1) + c_2)\\
    & = \frac{(\frac{1}{n} + \frac{1}{(B-r+1)^{1/4}})}{\mu(\frac{1}{2} - \frac{1}{2n} -\frac{1}{2(B-r+1)^{1/4}})}
    \cdot((\sswikbound{r} (2L(r-1) + (r-1)\mu) + 2c_2)
    \end{split}
\end{align*}

Then by using the fact that $M_1 = \frac{2c_2}{\mu}$ and $\sswikbound{r} = \swikbound{r}$, the formula above can be rewritten as:
\begin{align*}
    & = \sswikbound{r}
\end{align*}

This finishes the proof.

\end{proof}

\textbf{The proof of Theorem \ref{bfi2_multi_all_sgd}}
\begin{proof}
Similar to the proof of Theorem \ref{bfi2_sgd}, we define the following events:
$$\Omega_0(k, t) = \{\|\usw_t(k-1) - \usw_t(k)\| \leq M_1(\frac{r}{n} + \frac{1}{(B-k)^{1/4}})\}$$
$$\Omega_1(k, t) = \{\|\isw_t(k-1) - \isw_t(k)\| \leq \sswikbound{k}\}$$
%$$\omega_1(t) = \{\|\sw_{t} - \isw_{t}\| \leq \frac{1}{\frac{1}{2}-\frac{r}{n}-\frac{1}{B^{1/4}}}M_1(\frac{r}{n} + \frac{1}{B^{1/4}})\}$$
$$\Omega_2(k, t) = \{\|\sbHk{k-1}_t - \sBk{k-1}_{j_m}\| \leq \xi_{j_1,j_m}^S(k-1)\}$$
%$$\Omega_3(k) = \{\|\frac{1}{B}\sum_{i\in\miniB_k}\nabla F_i(\sw_k) - \frac{1}{n}\sum_{i=1}^n\nabla F_i(\sw_k)\| \leq c_2 \left(\frac{(\log(p+1))^2}{B}\right)^{1/4}\}$$
$$\Omega_3(k, t) = \{\|\left(\frac{1}{B-\Delta B_{t,k-1}}\sum_{\substack{i \in \miniB_{t}\\ i \not\in R_{k-1}}} \bH_i(\isw_{t}(k-1))\right)$$
$$ - \frac{1}{n-{(k-1)}}\sum_{i \not\in R_{k-1}} \bH_i(\isw_{t}(k-1))\|\leq \rhboundk{k-1}\}$$
$$\Omega_4(k,t) = \{\xi_{j_1,j_m}^S(k-1) = \xi_{j_0+xT_0,j_0 + (x+m-1)T_0}(k-1)\leq A(1-\eta\mu)^{j_0+xT_0}d_{0,mT_0-1}(0) + 2Ac_2 \left(\frac{(\log(p+1))^2}{B}\right)^{1/4}$$
$$+ A\frac{2}{c_0}\rhboundk{(k-1)}+ (2Ak+A)\cdot \sswikbound{k}\}$$
%$$ + 3A \sswikbound{k}\}$$
$$\Omega_5(k,t) = \{\frac{\Delta B_{t,k}-\Delta B_{t,k-1}}{B-\Delta B_{t,k}} \leq \frac{1}{n} + \frac{1}{(B-k+1)^{1/4}}\}$$

From Theorem \ref{theorem: stochastic_hessian_bound_multi}, equation \eqref{eq: xi_bound_multi_sgd}, Lemma \eqref{Lemma: bound_d_j_sgd} and Lemma \ref{lemma: delta_t_zeta_bounds_multi_sgd}, we know that the following inequalities or equations hold:
\begin{align}
%&Pr(\bigcap_{\tau=1}^t\Omega_0(k,\tau) \Bigr|\bigcap_{\tau=1}^t \Omega_5(k-1,\tau))=1 \label{eq: prob_omega0}\\
&Pr(\Omega_3(k, t)) \geq 1-\Psi_2(k)\label{eq: prob_omega3}\\
\begin{split}
& Pr(\bigcap_{k'=1}^k\bigcap_{\tau=1}^t\Omega_4(k',\tau) \Bigr| \bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^t\Omega_1(k',\tau), \bigcap_{\tau=1}^t\Omega_4(0,\tau)) = 1
\end{split}\label{eq: prob_omega4}\\
& Pr(\bigcap_{\tau=1}^t\Omega_4(0,\tau)) \geq 1-t \times\Psi_3(1)\\
&Pr(\bigcap_{\tau=1}^t \Omega_5(k,\tau))\geq 1- t\times\Psi_1(k)\label{eq: prob_omega5}
\end{align}


Also from Theorem \ref{wu_sgd_multi}, Corollary \ref{lemma: corollary: approx_hessian_real_hessian_bound_multi_sgd} and Theorem \ref{bfi_multi_sgd},  
we know that the following conditional probabilities hold:
\begin{align}
&Pr(\bigcap_{\tau=1}^t\Omega_0(k, \tau)\Bigr|\bigcap_{\tau=1}^t\Omega_5(k, \tau)) = 1\\
&Pr(\bigcap_{\tau=1}^t\Omega_2(k, \tau) \Bigr| \bigcap_{\tau=1}^t\Omega_1(k,\tau), \bigcap_{\tau=1}^t\Omega_3(k,\tau)) = 1\label{eq: condition_prob_omega2}\\
\begin{split}
& Pr(\bigcap_{\tau=1}^{t+1} \Omega_1(k,\tau) \Bigr| \bigcap_{\tau=1}^t\Omega_4(k,\tau), \bigcap_{\tau=1}^t \Omega_2(k, \tau),\bigcap_{\tau=1}^t \Omega_5(k, \tau)\\&\bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_4(k',\tau),
 \bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T \Omega_2(k', \tau), \bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_1(k',\tau),\bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_5(k',\tau))=1
\end{split}
\label{eq: condition_prob_omega1}
\end{align}

According to equation \eqref{eq: condition_prob_omega2}, we know that the following equation also holds:
\begin{align}\label{eq: prob_omega2_full}
\begin{split}
&Pr(\bigcap_{\tau=1}^t\Omega_2(k, \tau), \bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_2(k', \tau) \Bigr| \bigcap_{\tau=1}^t\Omega_1(k,\tau), \bigcap_{\tau=1}^t\Omega_3(k,\tau)\\
&, \bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_1(k',\tau), \bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_3(k',\tau)) = 1
\end{split}
\end{align}
which is then multiplied by equation \eqref{eq: condition_prob_omega1}. Then the result becomes:
\begin{align*}
\begin{split}
& Pr(\bigcap_{\tau=1}^{t+1} \Omega_1(k,\tau), \bigcap_{\tau=1}^t\Omega_2(k, \tau), \bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_2(k', \tau) \Bigr|\\
&\bigcap_{\tau=1}^t\Omega_4(k,\tau),\bigcap_{\tau=1}^t\Omega_1(k,\tau),\bigcap_{\tau=1}^t \Omega_5(k, \tau), \\
&\bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_4(k',\tau),
 \bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_1(k',\tau),\bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_5(k',\tau))=1
\end{split}
\end{align*}
which is then multiplied by equation \eqref{eq: condition_prob_omega1} with $t \rightarrow t-1$. The result is:
\begin{align*}
\begin{split}
& Pr(\bigcap_{\tau=1}^{t+1} \Omega_1(k,\tau), \bigcap_{\tau=1}^t\Omega_2(k, \tau), \bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_2(k', \tau) \Bigr|\\
&\bigcap_{\tau=1}^t\Omega_4(k,\tau),\bigcap_{\tau=1}^{t-1}\Omega_2(k,\tau),\bigcap_{\tau=1}^t \Omega_5(k, \tau),\bigcap_{\tau=1}^t \Omega_3(k, \tau), \\
&\bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_4(k',\tau),\bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_3(k',\tau),
 \bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_1(k',\tau),\bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_5(k',\tau))=1
\end{split}
\end{align*}

This can proceed recursively in the similar way to the proof of  Theorem \ref{bfi2_sgd}. In the end, the following inequality holds:
\begin{align*}
\begin{split}
& Pr(\bigcap_{\tau=1}^{T} \Omega_1(k,\tau), \bigcap_{\tau=1}^T\Omega_2(k, \tau), \bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_2(k', \tau) \Bigr|\\&\bigcap_{\tau=1}^T\Omega_4(k,\tau),\bigcap_{\tau=1}^T \Omega_5(k, \tau), \bigcap_{\tau=1}^T \Omega_3(k, \tau),\bigcap_{\tau=1}^{j_0} \Omega_0(k,\tau), \\
&\bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_3(k',\tau),\bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_4(k',\tau),
 \bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_1(k',\tau),\bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_5(k',\tau))=1
\end{split}
\end{align*}

By using the equation $Pr(\bigcap_{\tau=1}^t\Omega_0(k, \tau)\Bigr|\bigcap_{\tau=1}^t\Omega_5(k, \tau)) = 1$ at the ${j_0}_{th}$ iteration, the equation above becomes:
\begin{align*}
\begin{split}
& Pr(\bigcap_{\tau=1}^{T} \Omega_1(k,\tau), \bigcap_{\tau=1}^T\Omega_2(k, \tau), \bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_2(k', \tau) \Bigr|\\&\bigcap_{\tau=1}^T\Omega_4(k,\tau),\bigcap_{\tau=1}^T \Omega_5(k, \tau), \bigcap_{\tau=1}^T \Omega_3(k, \tau), \\
&\bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_3(k',\tau),\bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_4(k',\tau),
 \bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_1(k',\tau),\bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_5(k',\tau))=1
\end{split}
\end{align*}

which can be rewritten as:
\begin{align}\label{eq: full_prob_k}
\begin{split}
& Pr(\bigcap_{k'=1}^{k}\bigcap_{\tau=1}^{T} \Omega_1(k',\tau), \bigcap_{k'=1}^{k}\bigcap_{\tau=1}^T\Omega_2(k', \tau)\Bigr|\\
&\bigcap_{k'=1}^{k}\bigcap_{\tau=1}^T\Omega_3(k',\tau),\bigcap_{k'=1}^{k}\bigcap_{\tau=1}^T\Omega_4(k',\tau),
 \bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_1(k',\tau),\bigcap_{k'=1}^{k}\bigcap_{\tau=1}^T\Omega_5(k',\tau))=1
\end{split}
\end{align}

Since the above formula holds for any $k$, the following equation thus also holds:
\begin{align}\label{eq: full_prob_k_1}
\begin{split}
& Pr(\bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^{T} \Omega_1(k',\tau), \bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_2(k', \tau)\Bigr|\\
&\bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_3(k',\tau),\bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_4(k',\tau),
 \bigcap_{k'=1}^{k-2}\bigcap_{\tau=1}^T\Omega_1(k',\tau),\bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_5(k',\tau))=1
\end{split}
\end{align}

Then by multiplying equation \eqref{eq: full_prob_k} by equation \eqref{eq: full_prob_k_1}, we get:
\begin{align*}
\begin{split}
& Pr(\bigcap_{k'=1}^{k}\bigcap_{\tau=1}^{T} \Omega_1(k',\tau), \bigcap_{k'=1}^{k}\bigcap_{\tau=1}^T\Omega_2(k', \tau)\Bigr|\bigcap_{k'=1}^{k}\bigcap_{\tau=1}^T\Omega_3(k',\tau),\bigcap_{k'=1}^{k}\bigcap_{\tau=1}^T\Omega_4(k',\tau),\\
&\bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_2(k',\tau),\bigcap_{k'=1}^{k-2}\bigcap_{\tau=1}^T\Omega_1(k',\tau),\bigcap_{k'=1}^{k}\bigcap_{\tau=1}^T\Omega_5(k',\tau))=1
\end{split}
\end{align*}

Then by multiplying the formula by equation \eqref{eq: prob_omega3}, we get:
\begin{align*}
\begin{split}
& Pr(\bigcap_{k'=1}^{k}\bigcap_{\tau=1}^{T} \Omega_1(k',\tau), \bigcap_{k'=1}^{k}\bigcap_{\tau=1}^T\Omega_2(k', \tau), \bigcap_{k'=1}^{k}\bigcap_{\tau=1}^T\Omega_4(k',\tau) \Bigr|\bigcap_{k'=1}^{k}\bigcap_{\tau=1}^T\Omega_3(k',\tau),\\&\bigcap_{\tau=1}^T\Omega_4(0,\tau),
\bigcap_{k'=1}^{k-1}\bigcap_{\tau=1}^T\Omega_2(k',\tau),\bigcap_{k'=1}^{k-2}\bigcap_{\tau=1}^T\Omega_1(k',\tau),\bigcap_{k'=1}^{k}\bigcap_{\tau=1}^T\Omega_5(k',\tau))=1
\end{split}
\end{align*}


Then by replacing $k$ with $k-1$ in equation \eqref{eq: prob_omega2_full} and multiplying the resulting formula by the formula above, the result becomes:
\begin{align*}
\begin{split}
& Pr(\bigcap_{k'=1}^{k}\bigcap_{\tau=1}^{T} \Omega_1(k',\tau), \bigcap_{k'=1}^{k}\bigcap_{\tau=1}^T\Omega_2(k', \tau), \bigcap_{k'=1}^{k}\bigcap_{\tau=1}^T\Omega_4(k',\tau)\Bigr|\bigcap_{k'=1}^{k}\bigcap_{\tau=1}^T\Omega_3(k',\tau),\bigcap_{\tau=1}^T\Omega_4(0,\tau),\\
&\bigcap_{k'=1}^{k-2}\bigcap_{\tau=1}^T\Omega_1(k',\tau),\bigcap_{k'=1}^{k}\bigcap_{\tau=1}^T\Omega_5(k',\tau))=1
\end{split}
\end{align*}

This can proceed recursively (similar to the proof of Theorem \ref{bfi2_sgd}), in the end, the following equation holds:
\begin{align*}
\begin{split}
& Pr(\bigcap_{k'=1}^{k}\bigcap_{\tau=1}^{T} \Omega_1(k',\tau), \bigcap_{k'=1}^{k}\bigcap_{\tau=1}^T\Omega_2(k', \tau), \bigcap_{k'=1}^{k}\bigcap_{\tau=1}^T\Omega_4(k',\tau)\Bigr|\bigcap_{k'=1}^{k}\bigcap_{\tau=1}^T\Omega_3(k',\tau),\\
&\bigcap_{\tau=1}^T\Omega_4(0,\tau),\bigcap_{k'=1}^{k}\bigcap_{\tau=1}^T\Omega_5(k',\tau))=1
\end{split}
\end{align*}

By using the probability provided in equation \eqref{eq: prob_omega3}-\eqref{eq: prob_omega5} and using the same derivation as the proof of Theorem \ref{bfi2_sgd}, the following inequality holds:
\begin{align*}
\begin{split}
& Pr(\bigcap_{k'=1}^{k}\bigcap_{\tau=1}^{T} \Omega_1(k',\tau), \bigcap_{k'=1}^{k}\bigcap_{\tau=1}^T\Omega_2(k', \tau), \bigcap_{k'=1}^{k}\bigcap_{\tau=1}^T\Omega_4(k',\tau))\\
& \geq 1-T \times\Psi_3(1)\\
& - kT(\Psi_2(k) + \Psi_1(k))
\end{split}
\end{align*}

It indicates that with probability higher than $1-T \times\Psi_3(1)- rT(\Psi_2(r) + \Psi_1(r))$, the events $\bigcap_{k'=1}^{r}\bigcap_{\tau=1}^{T} \Omega_1(k',\tau)$, $\bigcap_{k'=1}^{r}\bigcap_{\tau=1}^T\Omega_2(k', \tau)$, $\bigcap_{k'=1}^{r}\bigcap_{\tau=1}^T\Omega_4(k',\tau)$ are true.

Then according to Lemma \ref{lemma: approximate_vs_real_gradient_bound_sgd_multi}, with the same probability, the following inequality holds for any $k \leq r$ and $t \leq T$:
\begin{align*}
    \begin{split}
        &\|\frac{1}{B-\Delta B_{t, k-1}}\sum_{i\not\in R_{k-1}, i\in \miniB_{t}}\nabla F_i(\isw_t(k-1))-\ag(\isw_t(k-1))\|
         \leq \sswikbound{k}k\mu
    \end{split}
\end{align*}

This finishes the proofs.

\end{proof}

\textbf{The proof of Theorem \ref{main10_multi_sgd}}
\begin{proof}
According to Theorem \ref{bfi2_multi_all_sgd}, we know that with probability higher than $1-T \times\Psi_3(1) - rT(\Psi_2(r) + \Psi_1(r))$, the following inequalities hold for all $k\leq r$, $t \leq T$:
\begin{align*}
& \|\isw_t(k)-\isw_t(k-1)\| \leq \sswikbound{k}\\
& \|\sbHk{k-1}_{t} - \sBk{k-1}_{j_m}\| \leq \xi_{j_1,j_m}^S(k-1)\\
\begin{split}
&\|\frac{1}{B-\Delta B_{t, k-1}}\sum_{i\not\in R_{k-1}}\nabla F_i(\isw_t(k-1))-\ag(\isw_t(k-1))\| \\
&\leq \sswikbound{k}r\mu
\end{split}\\
\begin{split}
& \xi_{j_1,j_m}^S(k-1) = \xi_{j_0+xT_0,j_0 + (x+m-1)T_0}(k-1)\\
& \leq A(1-\eta\mu)^{j_0+xT_0}d_{0,mT_0-1}(0) + 2Ac_2 \left(\frac{(\log(p+1))^2}{B}\right)^{1/4}+ A\frac{2}{c_0}\rhboundk{(k-1)}\\
& + (2Ak+A)\cdot \sswikbound{k}
\end{split}
\end{align*}

Then by using the same derivation as the proof of Theorem 
\ref{main10_sgd} at each deletion request, we know that with the same probability, $$\|\usw_t(k) - \isw_t(k)\| = o(\frac{k}{n} + \frac{k}{(B-k+1)^{1/4}})$$ holds for every $k \leq r$.

\end{proof}


%\textbf{The proof of Theorem \ref{main10_multi_sgd}}
%\begin{proof}
%Recall that the update rule for $\usw_t(r)$ is:
%$$\usw_{t+1}(r) = \usw_t(r) - \eta\frac{1}{B-\Delta B_{t, r}}\sum_{i\not\in R_r}\nabla F(\usw_t(r))$$ and the update rule for $\isw_t(r)$ is (where the gradients are explicitly evaluated):
%$$\isw_{t+1}(r) = \isw_{t}(r) - \frac{\eta}{B-\Delta B_{t, r}}[(B-\Delta B_{t, r-1})(\B_{j_m}^{r-1}(\isw_t(r) - \isw_t(r-1)) + \ag(\isw_{t}(r-1))) - \nabla F_{i_r}(\isw_t(r))]$$
%Then by subtracting $\isw_{t+1}(r)$ by $\usw_{t+1}(r)$, we get:
%\begin{align*}
%    \begin{split}
%        & \|\isw_{t+1}(r) - \usw_{t+1}(r)\|\\
%        & = \|\isw_{t}(r) - \usw_{t}(r) - \frac{\eta}{B-\Delta B_{t, r}}[(B-\Delta B_{t, r-1})(\B_{j_m}^{r-1}(\isw_t(r) - \isw_t(r-1)) \\
%        & + \ag(\isw_{t}(r-1))) - \nabla F_{i_r}(\isw_t(r))] + \frac{\eta}{B-\Delta B_{t, r}}\sum_{i \not\in R_r}\nabla F(\usw_t(r))\|\\
%    \end{split}
%\end{align*}
%
%Then by bringing in $\sbHk{r-1}_t$ and $\frac{1}{B-\Delta B_{t, r-1}}\sum_{i\in R_{r-1}}\nabla F(\isw_t(r-1))$ into the formula above, we get:
%\begin{align*}
%    \begin{split}
%        & = \|\isw_{t}(r) - \usw_{t}(r) - \frac{(B-\Delta B_{t, r-1})\eta}{B-\Delta B_{t, r}}\left[\left(\B_{j_m}^{r-1} - \bH_{t}^{r-1}\right)(\isw_{t}(r) - \isw_{t}(r-1))\right.\\
%        & + \bH_{t}^{r-1}\mmop(\isw_{t}(r) - \isw_{t}(r-1)) + \ag(\isw_{t}(r-1))\\
%        &\left. - \frac{1}{B-\Delta B_{t, r-1}}\sum_{i\in R_{r-1}}\nabla F(\isw_t(r-1)) + \frac{1}{B-\Delta B_{t, r-1}}\sum_{i\in R_{r-1}}\nabla F(\isw_t(r-1))\right]\\
%     & + \frac{\eta}{B-\Delta B_{t, r}}(\nabla F_{i_r}(\isw_{t}(r)) - \nabla F_{i_r}(\isw_{t}(r-1)) + \nabla F_{i_r}(\isw_{t}(r-1)))\\
%     & + \frac{\eta}{B-\Delta B_{t, r}}\sum_{\substack{i \not\in R_r}} \nabla F_i(\usw_{t}(r))\|
%    \end{split}
%\end{align*}
%
%Then by using triangle inequality and the result from equation \eqref{eq: real_approx_gradient_gap_tight_sgd}, the formula above can be bounded as:
%\begin{align*}
%    \begin{split}
%        & \leq \|\isw_{t}(r) - \usw_{t}(r) - \frac{(B-\Delta B_{t, r-1})\eta}{B-\Delta B_{t, r}}\left[\left(\B_{j_m}^{r-1} - \bH_{t}^{r-1}\right)(\isw_{t}(r) - \isw_{t}(r-1))\right.\\
%        & + \left.\bH_{t}^{r-1}\mmop(\isw_{t}(r) - \isw_{t}(r-1)) + \frac{1}{B-\Delta B_{t, r-1}}\sum_{i\in R_{r-1}}\nabla F_i(\isw_t(r-1))\right]\\
%     & + \frac{\eta}{B-\Delta B_{t, r}}(\nabla F_{i_r}(\isw_{t}(r)) - \nabla F_{i_r}(\isw_{t}(r-1)) + \nabla F_{i_r}(\isw_{t}(r-1)))\\
%     & + \frac{\eta}{B-\Delta B_{t, r}}\sum_{\substack{i \not\in R_r}} \nabla F_i(\usw_{t}(r))\| + A (1-\mu\eta)^{j_0 + xT_0}d_{0,(m-1)T_0}(0)r\sswikbound{r}\\
%        & + A(r\sswikbound{r})^2
%    \end{split}
%\end{align*}
%
%Note that the first matrix norm in this formula is the same as equation \eqref{eq: w_i_w_u_gap_deriv1} by replacing $n$, $r$, $\isw_t$, $\usw_t$, $\sw_t$, $\B_{j_m}$, $\bH_t$ and $\nabla F(\sw_t)$ with $B-\Delta B_{t, r-1}$, $1$, $\isw_t(r)$, $\usw_t(r)$, $\isw_t(r-1)$, $\B_{j_m}^{r-1}$, $\sbHk{r-1}_t$ and $\frac{1}{B-\Delta B_{t, r-1}}\sum_{i\not\in R_{r-1}}\nabla F_i(\isw_t(r-1))$ reps.. So by following the same derivations, the formula above can be bounded as:
%\begin{align}
%\begin{split}
%& \leq \|(\textbf{I} - \frac{\eta}{B-\Delta B_{t, r}}\sum_{\substack{i \not\in R_r}}\bH_{t,i}^{r-1})(\isw_{t}(r)-\usw_{t}(r))\|\\
%& + \|\frac{(B-\Delta B_{t, r-1})\eta}{B-\Delta B_{t, r}}\left[\left(\B_{j_m}^{r-1} - \bH_{t}^{r-1}\right)(\isw_{t}(r) - \usw_{t}(r))\right]\|\\
%& + \|\frac{\eta}{B-\Delta B_{t, r}}[\sum_{i\not\in R_r}\int_0^1 \bH_i(\isw_t(r-1) + x(\usw_t(r)-\isw_t(r-1)))dx \\
%& - \int_0^1 \bH_i(\isw_t(r-1) + x(\isw_t(r)-\isw_t(r-1)))dx](\usw_{t}(r)-\isw_t(r-1))\|\\
%& + \|\frac{(B-\Delta B_{t, r-1})\eta}{B-\Delta B_{t, r}}\left[\left(\B_{j_m}^{r-1} - \bH_{t}^{r-1}\right)(\usw_{t}(r) - \isw_{t}(r-1))\right]\|\\
%& + A (1-\mu\eta)^{j_0 + xT_0}d_{0,(m-1)T_0}(0)r\sswikbound{r}\\
%        & + A(r\sswikbound{r})^2
%\end{split}
%\end{align}
%
%Then we use the following facts 
%\benum 
%\item $\|\textbf{I} - \eta \bH_{t,i}^{r-1}\| \le 1 - \eta \mu$ 
%\item from Theorem \ref{bfi2_multi_all} on the approximation accuracy of the quasi-Hessian to mean Hessian, we have the error bound $\|\sbHk{r-1}_t - \B_{j_m}^{r-1}\|\le\xi_{j_1,j_m}^S(r-1)$,
%\item we bound the difference of integrated Hessians using the strategy from equation \eqref{eq: hessian_diff_bound0}
%\item from equation \eqref{eq: w_u_w_i_prev_bound}, we have the error bound $\|\usw_{t}(r)-\isw_t(r-1)\|\le M_2 \frac{r}{n}$ (and this requires no additional assumptions)
%\eenum
%The expression can be bounded as follows. 
%
%\begin{align}
%    \begin{split}
%        & \leq (1-\eta\mu + \frac{(B-\Delta B_{t, r-1})\eta}{B-\Delta B_{t, r}}\xi_{j_0,j_0+(m-1)T_0}(r-1)+\frac{c_0M_2r\eta}{2n})\|\isw_t - \usw_t\|\\
%        & + \frac{M_2(B-\Delta B_{t, r-1})r\eta}{n(B-\Delta B_{t, r})} \xi_{j_1,j_m}^S(r-1) + A (1-\mu\eta)^{j_0 + xT_0}d_{0,(m-1)T_0}(0)r\sswikbound{r}\\
%        & + A(r\sswikbound{r})^2
%    \end{split}
%\end{align}
%
%
%
%% By using the result from equation \eqref{eq: xi_bound_multi}, the formula above can be bounded as:
%% \begin{align}
%%     \begin{split}
%%         & \leq (1-\eta\mu + \frac{n\eta}{B-\Delta B_{t, r}}\xi_{j_0,j_0+(m-1)T_0}(r-1)+\frac{c_0M_2r\eta}{2n})\|\isw_t - \usw_t\|\\
%%         & + \frac{M_2r\eta}{B-\Delta B_{t, r}} (A (1-\mu\eta)^{j_0 + xT_0}d_{0,mT_0-1}(0) + A(2r-1)\sswikbound{r})\\
%%         & + A (1-\mu\eta)^{j_0 + xT_0}d_{0,mT_0-1}(0)r\sswikbound{r}\\
%%         & + A(r\sswikbound{r})^2
%%     \end{split}
%% \end{align}
%
%which is very similar to equation \eqref{eq: w_u_w_i_gap_deriv_2} (except the difference in the coefficient). So by following the derivation after equation \eqref{eq: w_u_w_i_gap_deriv_2}, we know that:
%\begin{align}
%    \|\isw_t(r)-\usw_t(r)\| = o(\frac{r}{n})
%\end{align}
%
%when $t\rightarrow \infty$.
%
%\end{proof}
%


==> Sections/other_alg_backup.tex <==
% !TEX root = supplement.tex

\section{Supplementary algorithm details}

In Section \ref{sec: alg}, we only provided the details of \Increm\ for deterministic gradient descent for the strongly convex and smooth objective functions in batch deletion/addition scenarios. In this section, we will provide more details on how to extend \Increm\ to handle stochastic gradient descent, online deletion/addition scenarios and non-strongly convex, non-smooth objective functions.

\subsection{Extension of \Increm\ for stochastic gradient descent}
By using the notations from equations \eqref{eq: sw_update}-\eqref{eq: isw_update}, we need to approximately or explicitly compute 
$\sgrad$, 
i.e. the average gradient for a mini-batch in the SGD version of \Increm, instead of 
$\nabla F$
, which is the average gradient for all samples. So by replacing $\w_t$, $\uw_t$, $\iw_t$, $\nabla F$, $\B$ and $\bH$ with $\sw_t$, $\usw_t$, $\isw_t$, $\sgrad$, $\sB$ and $\sbH$ in Algorithm \ref{alg: update_algorithm}, we get the SGD version of \Increm.

\subsection{Extension of \Increm\ for online deletion/addition}

In the online deletion/addition scenario, whenever the model parameters are updated after the deletion or addition of one sample, the history information should be also updated to reflect the changes. By assuming that only one sample is deleted or added each time, the online deletion/addition version of \Increm\ is provided in Algorithm \ref{alg: update_algorithm_online} and the differences relative to Algorithm \ref{alg: update_algorithm} are highlighted.

Since the history information needs to be updated every time when new deletion or addition requests arrive, we need to do some more analysis on the error bound, which is still pretty close to the analysis in Section \ref{sec: math}. %This will be done in future work. 

In what follows, the analysis will be conducted on gradient descent with online deletion, which should be pretty similar to other scenarios, e.g. stochastic gradient descent with online addition.

\begin{algorithm}[t] 
\small
% \footnotesize
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{The full training set $\left(\textbf{X}, \textbf{Y}\right)$, model parameters cached during the training phase for the full training samples $\{\w_{0}, \w_{1}, \dots, \w_{t}\}$ and corresponding gradients $\{\nabla F\left(\w_{0}\right), \nabla F\left(\w_{1}\right), \dots, \nabla F\left(\w_{t}\right)\}$, the index of the removed training sample or the added training sample $i_r$, period $T_0$, total iteration number $T$, history size $m$, warmup iteration number $j_0$, learning rate $\eta$}
\Output{Updated model parameter $\iw_{t}$}
Initialize $\iw_{0} \leftarrow \w_{0}$

Initialize an array $\Delta G = \left[\right]$

Initialize an array $\Delta W = \left[\right]$

\For{$t=0;t<T; t++$}{

\eIf{$[((t - j_0) \mod T_0) == 0]$ or $t \leq j_0$}
{
    compute $\nabla F\left(\iw_{t}\right)$ exactly
    
    compute $\nabla F\left(\iw_{t}\right) - \nabla F\left(\w_{t}\right)$ based on the cached gradient $\nabla F\left(\w_{t}\right)$
    
    set $\Delta G\left[k\right] = \nabla F\left(\iw_{t}\right) - \nabla F\left(\w_{t}\right)$
    
    set $\Delta W\left[k\right] = \iw_{t} - \w_{t}$, based on the cached parameters $\w_{t}$
    
    $k\leftarrow k+1$
    
    compute $\iw_{t+1}$ by using exact GD update (equation \eqref{eq: update_rule_naive})
    \hl{$\w_t \leftarrow \iw_t$}
    
    \hl{$\nabla F(\w_t) \leftarrow \nabla F(\iw_t)$}
}
{
    Pass $\Delta W\left[-m:\right]$, $\Delta G\left[-m:\right]$, the last $m$ elements in $\Delta W$ and $\Delta G$, which are from the $j_1^{th}, j_2^{th},\dots, j_m^{th}$ iterations where $j_1 < j_2< \dots < j_m$ depend on $t$, $\textbf{v} = \iw_{t} - \w_{t}$, and the history size $m$, to the L-BFGFS Algorithm (See Supplement) to get the approximation of $\bH(\w_{t})\textbf{v}$, i.e., $\B_{j_m}\textbf{v}$
    
    Approximate $\nabla F\left(\iw_{t}\right) = \nabla F\left(\w_{t}\right) + \B_{j_m}\left(\iw_{t} - \w_{t}\right)$
    
    Compute $\iw_{t+1}$ by using the "leave-$1$-out" gradient formula, based on the approximated $\nabla F(\iw_{t})$ 
    
    \hl{$\w_t \leftarrow \iw_t$}
    
    \hl{$\nabla F(\w_t) \leftarrow \frac{\eta}{n-1}[n(\B_{j_m}(\iw_t - \w_t) + \nabla F(\w_{t})) - \nabla F_{i_r}(\w_t)]$}
}
}

\Return $\iw_{t}$
\caption{DeltaGrad (online deletion/addition)}
\label{alg: update_algorithm_online}
\end{algorithm}


\subsubsection{Convergence rate for online gradient descent version of \Increm}

\textbf{Additional notes on setup, preliminaries}

Let us still denote the model parameters for the original dataset at the $t_{th}$ iteration by $\w_t$. During the model update phase for the $k_{th}$ deletion request at the $t_{th}$ iteration, the model parameters updated by \Basel\ and \Increm\ are denoted by $\uw_t(k)$ and $\iw_t(k)$ respectively where $\uw_t(0) = \iw_t(0) = \w_t$. We also assume that the total number of removed samples in all deletion requests, $r$, is still far smaller than the total number of samples, $n$. 

Also suppose that the indices of the removed samples are $\{i_1,i_2,\dots, i_{r}\}$, which are removed at the $1_{st}$, $2_{nd}$, $3_{rd},\dots,$, ${r}_{th}$ deletion request. This also means that the cumulative number of samples up to the $k_{th}$ deletion request ($k\leq r$) is $n-k$ for all $1 \leq k \leq r$ and thus the objective function at the $k_{th}$ iteration will be:
\begin{align}
    F^k(\w) = \frac{1}{n-k}\sum_{i \not\in R_{k}} F_i(\w)
\end{align}

where $R_k = \{i_1,i_2,\dots,i_k\}$. Plus, at the $k_{th}$
deletion request, we denote by $\bH^{k}_t$ the average Hessian matrix of  $F^k(\w)$ evaluated between $\iw_t(k+1)$ and $\iw_t(k)$:
$$\bH^{k}_t = \frac{1}{n-k}\sum_{i\not\in R_{k}} \int_{0}^1\bH_i(\iw_t(k) + x(\iw_t(k+1)-\iw_t(k)))dx$$

Specifically, $$\bH^{0}_t = \frac{1}{n}\sum_{i=1}^n \int_0^1\bH_i(\iw_t(0) + x(\iw_t(1)-\iw_t(0)))dx.$$

Also the model parameters and the gradients evaluated by using \Increm\ at each iteration at the ${r-1}_{st}$ deletion request are used  at the $r_{th}$ request, and are denoted by: $$\{\iw_{0}(r-1), \iw_{1}(r-1), \dots, \iw_{t}(r-1)\}$$ and $$\{\ag \left(\iw_{0}(r-1)\right), \ag\left(\iw_{1}(r-1)\right), \dots, \ag\left(\iw_{t}(r-1)\right)\}$$ 

Note that $\ag(\iw_t(k))$ ($k\leq r$) is not necessarily equal to $\nabla F$ due to the approximation brought by \Increm. But due to the periodicity of \Increm, at iteration $0,1,\dots,j_0$ and iteration $j_0 + xT_0$ ($x=1,2,\dots,$), the gradients are explicitly evaluated, i.e.:
$$\ag(\iw_t(k)) = \frac{1}{n-k}\sum_{i\not\in R_k} \nabla F_i(\iw_t(k))$$
for $t = 0,1,\dots, j_0$ or $t = j_0 + xT_0$ ($x \geq 1$) and all $k \leq r$. 

Also, due to the periodicity, the sequence $[\Delta g_{j_0}, \Delta g_{j_1},\dots, \Delta g_{j_{m-1}}]$ used in approximating the Hessian matrix always uses the exact gradient information, which means that:
$$\Delta g_{j_q} = \frac{1}{n-k}[\sum_{i\not\in R_k}\nabla F_i(\iw_{j_q}(k)) - \sum_{i \not\in R_k}\nabla F_i(\iw_{j_q}(k-1))]$$

where $q=1,2,\dots,m-1$. So Lemma \ref{assp: B_K_product_bound} on the bound on the eigenvalues of $B_{j_q}$ holds for all $k=1,2,\dots,r$. 



But for the iterations where the gradients are not explicitly evaluated, the calculation of $\ag(\iw_t(k))$ depends on the approximated Hessian matrix $\B_{j_m}^{k-1}$ and the approximated gradients calculated at the $t_{th}$ iteration at the $(k-e$ deletion request. So the update rule for $\ag(\iw_t(k))$ is:
\begin{align}\label{eq: g_w_k_deriv}
    \begin{split}
        & \ag(\iw_t(k)) = \frac{1}{n-k}[(n-k+1)(\B_{j_m}^{k-1}(\iw_t(k) - \iw_t(k-1))\\
        & + \ag(\iw_t(k-1))) - \nabla F_{i_k}(\iw_t(k))]
    \end{split}
\end{align}

in which the product $\B_{j_m}^{k-1}(\iw_t(k) - \iw_t(k-1))$ approximates $$\frac{1}{n-k+1}\sum_{i\not\in R_{k-1}}\nabla F_i(\iw_t(k)) - \nabla F_i(\iw_t(k-1))$$
and $\ag(\iw_t(k-1))$ approximates $\frac{1}{n-k+1}\sum_{i\not\in R_{k-1}}\nabla F_i(\iw_t(k-1))$.


Similarly, the online version of $\Dw$ (at the $k_{th}$ iteration) becomes:
$$\Dw_{j_q}(k) = \iw_{j_q}(k) - \iw_{j_q}(k-1)$$
where $q=1,2,\dots,m-1$.




Similarly, we use $d_{j_a,j_b}(k)$ 
% and $\xi_{j_a,j_b}(k)$ 
to denote the value of $d$
% and $\xi$ values 
at the $k_{th}$ deletion request and use $\B_{j_m}^{k-1}$ to denote the approximated Hessian matrix in the $k_{th}$ deletion request, which approximated the Hessian matrix $\bH_t^{k-1}$.
% $$\xi_{j_1,j_m}(k-1):= A d_{j_1,j_m + T_0 - 1}(k-1)
% + A \frac{1}{\frac{1}{2}-\frac{1}{n}}M_1\frac{1}{n}$$




So in this case, the update rule for $\iw_t(k)$ becomes:
\begin{align}\label{iw_u_online}
    \iw_{t+1}(k) = \begin{cases}
         &\iw_{t}(k)-\frac{\eta}{n-k} \sum_{i\not\in R_k}\nabla F_i(\iw_t(k)),\,\, (t - j_0) \mod T_0 = 0\ or\ t \leq j_0 \\[2pt]
         \begin{split}
        &\iw_{t}(k) - \frac{\eta}{n-k}[(n-k+1)(\B_{j_m}^{k-1}(\iw_t(k) - \iw_t(k-1)) \\
        &+ \ag(\iw_{t}(k-1))) - \nabla F_{i_k}(\iw_t(k))],\,\, else     
         \end{split}
        \end{cases}
\end{align}

% where we define $R_k = \{i_1,i_2,\dots, i_k\}$. Note that $\{i_1,i_2,\dots,i_{k-1}\}$ has been deleted in the first $k-1$ deletion requests while the sample $i_k$ is removed at the $k_{th}$ deletion request. Also we define $\iw_t(0) = \w_t$.

% Recall that the gradients are explicitly evaluated 


\textbf{Proof preliminary}

Note that for \Basel\ to deal with each deletion request, the model parameters will always be retrained from scratch on the remaining samples, which means that Theorem \ref{wu} also holds if we replace $\uw_t$, $\w_t$ and $r$ with $\uw_t(k)$, $\uw_t(k-1)$ and 1 respectively:

\begin{theorem}[Bound between iterates deleting one datapoint]\label{wu_multi}
$\|\uw_{t}(r) - \uw_{t}(r-1)\| \leq M_1 \frac{1}{n}$ where $M_1=\frac{2}{\mu }c_2$ is some positive constant that does not depend on $t$. Here $\mu$ is the strong convexity constant, and $c_2$ is the bound on the individual gradients. 
\end{theorem}

By induction, we also know that the following inequality holds:
\begin{align}\label{eq: w_u_w_gap}
    \|\uw_{t}(r) - \uw_{t}(0)\| = \|\uw_{t}(r) - \w_{t}\| \leq M_1 \frac{r}{n}
\end{align}



% Also the history information for \Increm\ used at the $k_{th}$ request will become $\{\w_{0}(k-1), \w_{1}(k-1), \dots, \w_{t}(k-1)\}$ and $$\{\ag \left(\w_{0}(k-1)\right), \ag\left(\w_{1}(k-1)\right), \dots, \ag\left(\w_{t}(k-1)\right)\}$$ (note that $\ag$ is not necessarily equal to $\nabla F$ due to the approximation brought by \Increm). Similarly, we use $d_{j_a,j_b}(k)$ 
% % and $\xi_{j_a,j_b}(k)$ 
% to denote the value of $d$ and
% % and $\xi$ values 
% in the $k_{th}$ deletion request and use $\bH_t^{k}$ and $\B_t^{j_m}$ to denote the Hessian matrix and approximated Hessian matrix in the $k_{th}$ deletion request.
% $$\xi_{j_1,j_m}(k-1):= A d_{j_1,j_m + T_0 - 1}(k-1)
% + A \frac{1}{\frac{1}{2}-\frac{1}{n}}M_1\frac{1}{n}$$




% So in this case, the update rule for $\iw_t(k)$ becomes:
% \begin{align}\label{iw_u_online}
%     \iw_{t+1}(k) = \begin{cases}
%          &\iw_{t}(k)-\frac{\eta}{n-k} \sum_{i\not\in R_k}\nabla F(\iw_t(k)),\,\, (t - j_0) \mod T_0 = 0\ or\ t \leq j_0 \\[2pt]
%          \begin{split}
%         &\iw_{t}(k) - \frac{\eta}{n-k}[(n-k+1)(\B_{j_m}(\iw_t(k) - \iw_t(k-1)) \\
%         &+ \ag(\iw_{t}(k-1))) - \nabla F_{i_k}(\iw_t(k))],\,\, else     
%          \end{split}
%         \end{cases}
% \end{align}

% where we define $R_k = \{i_1,i_2,\dots, i_k\}$. Note that $\{i_1,i_2,\dots,i_{k-1}\}$ has been deleted in the first $k-1$ deletion requests while the sample $i_k$ is removed at the $k_{th}$ deletion request. Also we define $\iw_t(0) = \w_t$.

% Recall that the gradients are explicitly evaluated at iteration $0,1,\dots,j_0$ and iteration $j_0 + xT_0$ ($x=1,2,\dots,$), which is true for all $k=1,2,\dots,r$. It indicates that the sequence $[\Delta g_{j_0}, \Delta g_{j_1},\dots, \Delta g_{j_{m-1}}]$ that is used in approximating the Hessian matrix should always use the exact gradient information, i.e. $\Delta g_{j_q} = \frac{1}{n-k}[\sum_{i\not\in R_k}\nabla F_i(\iw_{j_q}(k)) - \sum_{i \not\in R_k}\nabla F_i(\iw_{j_q}(k-1))]$ ($q=1,2,\dots,m-1$). So Lemma \ref{assp: B_K_product_bound}, i.e. the bound of the eigenvalues of $B_{j_q}$ holds for all $k=1,2,\dots,r$. 


Then let us do some analysis on $d_{j_a,j_b}(k)$. 


\begin{lemma}\label{lemma: bound_d_j_multi}
If $\|\iw_t(k) - \iw_t(k-1)\| \leq \wikbound{k}$  for all $k \leq r$, then $d_{j_a,j_b}(r) \leq d_{j_a,j_b}(0) + 2r\cdot \wikbounds$ 
% and thus $$\xi_{j_a,j_b}(r) \leq A d_{j_a,j_b + T_0 - 1}(0)
% + A \frac{2r + 1}{\frac{1}{2}-\frac{1}{n}}M_1\frac{1}{n}$$ 
where $M_1$ is defined in Theorem \ref{wu_multi}.
\end{lemma}

\begin{proof}
Recall that $d_{j_a, j_b}(k) = \max(\|\iw_y(k) - \iw_z(k)\|)_{j_a < y < z < j_b}$.
Then for two arbitrary iterations $y, z$, let us bound $\|\iw_y(k) - \iw_z(k)\|$ as below:
\begin{align}
    \begin{split}
        & \|\iw_y(k) - \iw_z(k)\|\\
        & = \|\iw_y(k) - \iw_z(k) + \iw_y(k-1) - \iw_z(k-1) + \iw_z(k-1) - \iw_y(k-1)\|\\
        & \leq \|\iw_y(k) - \iw_y(k-1)\| + \|\iw_z(k) - \iw_z(k-1)\| + \|\iw_z(k-1) - \iw_y(k-1)\|
    \end{split}
\end{align}

Then by using the bound on $\|\iw_t(k) - \iw_t(k-1)\|$, the above formula leads to:
\begin{align}
    \begin{split}
        & \leq 2\cdot \wikbound{k}+ \|\iw_z(k-1) - \iw_y(k-1)\|
    \end{split}
\end{align}

By using  that $\wikbound{k} \leq \wikbound{r}$ and applying it recursively for $k=1,2,\dots,r$, we have:
\begin{align}
    \begin{split}
        &\|\iw_y(r) - \iw_z(r)\|
         \leq 2r\cdot \wikbound{r} + \|\iw_z(0) - \iw_y(0)\|
    \end{split}
\end{align}

Then by using the definition of $d_{j_a,j_b}(k)$, the following inequality holds:
\begin{equation}
    d_{j_a,j_b}(r) \leq d_{j_a,j_b + T_0 - 1}(0)
+ 2r\cdot \wikbound{r}
\end{equation}
% \begin{equation}
%     \xi_{j_a,j_b}(r) \leq A d_{j_a,j_b + T_0 - 1}(0)
% + A \frac{2Cr+1}{\frac{1}{2}-\frac{1}{n}}M_1\frac{1}{n}
% \end{equation}
Note that since $\wikbound{k} \leq \wikbound{r}$, then the assumption of the above result also implies that $\|\iw_t(k) - \iw_t(k-1)\| \leq \wikbound{r}$ for any $k \leq r$. In the rest of the document, we use $\wikbounds$ to represent $\wikbound{r}$ where $M_1^{r}$ is a constant which does not depend on $k$.

\end{proof}



\begin{theorem}\label{theorem: delta_model_para_bound_multi}
Suppose that at the $k_{th}$ deletion request, $\|\iw_{j_q}(k) - \iw_{j_q}(k-1)\| \leq \wikbounds $, where $q=1,2,\dots,m$ and $M_1 = \frac{2c_2}{\mu}$. Let $a = \frac{L(L+1) + K_2 L}{\mu  K_1}$ for the upper and lower bounds $K_1,K_2$ on the eigenvalues of the quasi-Hessian from Lemma \ref{assp: B_K_product_bound}, and for the Lipshitz constant $c_0$ of the Hessian. For $1 \leq z+1 \leq y \leq m$ we have,
$$\|\bH_{j_z}^{k-1} - \bH_{j_y}^{k-1}\| \leq c_0 d_{j_z, j_y}(k-1) + c_0 \wikbounds$$ and 
$$\|\Dg_{j_z} - \B_{j_y}^{k-1}\Dw_{j_z}\| \leq \left[(1+a)^{y-z-1} - 1\right]\cdot c_0 (d_{j_z,j_y} + \wikbounds) \cdot s_{j_1,j_m}(k-1)$$
 where $s_{j_1,j_m}(k-1) = \max\left(\|\Dw_{a}(k-1)\|\right)_{a=j_1,j_{2},\dots,j_m} = \max\left(\|\isw_{a}(k-1)-\isw_{a}(k-2)\|\right)_{a=j_1,j_{2},\dots,j_m}$, 
 and recall that $d$ is defined as the maximum gap between the steps of the algorithm for the iterations from $j_z$ to $j_y$:
\beq\label{d0}
d_{j_z,j_y}(k-1) = \max\left(\|\iw_{a}(k-1) - \iw_{b}(k-1)\|\right)_{j_z \leq a \leq b \leq j_y}.
\eeq
\end{theorem}
\begin{proof}
Let us bound the difference between the averaged Hessians $\|\bH_{j_z}^{k-1} - \bH_{j_y}^{k-1}\|$, where $1 \leq z < y \leq m$, using their definition, as well as using Assumption \ref{assp: hessian_continuous} on the Lipshitzness of the Hessian:
%k->y, q->z
\begin{align}\label{eq: hessian_diff_bound01}
    \begin{split}
      & \|\bH_{j_y}^{k-1} - \bH_{j_z}^{k-1}\|\\
      & = \|\int_0^1 [\bH(\iw_{j_y}(k-1) + x (\iw_{j_y}(k) - \iw_{j_y}(k-1)))]dx\\
      & - \int_0^1 [\bH(\iw_{j_z}(k-1) + x (\iw_{j_z}(k) - \iw_{j_z}(k-1)))]dx\|\\
      & = \| \int_0^1 [\bH(\iw_{j_y}(k-1) + x (\iw_{j_y}(k) - \iw_{j_y}(k-1)))\\
      & -\bH(\iw_{j_z}(k-1) + x (\iw_{j_z}(k) - \iw_{j_z}(k-1)))]dx \|\\
      & \leq c_0 \int_0^1 \|\iw_{j_y}(k-1) + x (\iw_{j_y}(k) - \iw_{j_y}(k-1))\\
      & - [\iw_{j_z}(k-1) + x (\iw_{j_z}(k) - \iw_{j_z}(k-1))]\| dx \\
      & \leq c_0\| \iw_{j_y}(k-1) - \iw_{j_z}(k-1)\|\\
      & + \frac{c_0}{2}\|\iw_{j_y}(k) - \iw_{j_y}(k-1) - (\iw_{j_z}(k) - \iw_{j_z}(k-1))\| \\
      & \leq c_0 \|\iw_{j_y}(k-1) - \iw_{j_z}(k-1)\|\\
      & + \frac{c_0}{2}\|\iw_{j_z}(k)- \iw_{j_z}(k-1)\| + \frac{c_0}{2}\|\iw_{j_y}(k) - \iw_{j_y}(k-1)\|\\
      & \leq c_0 d_{j_y, j_z}(k-1) + c_0\wikbounds\\
      & \leq c_0 d_{j_1, j_m +T_0 - 1}(k-1) + c_0\wikbounds
    \end{split}
\end{align}
On the last line, we have used the definition of $d_{j_z, j_y}$, and the assumption on the boundedness of $\|\iw_{j_z}(k) - \iw_{j_z}(k-1)\|$.

Then by following the rest of the proof of Theorem \ref{theorem: delta_model_para_bound}, we know that the following inequality holds: $$\|\Dg_{j_z} - \B_{j_y}\Dw_{j_z}\| \leq \left[(1+a)^{y-z-1} - 1\right]\cdot c_0 (d_{j_z,j_y}(k-1) + \wikbounds) \cdot s_{j_1,j_m}(k-1)$$

\end{proof}

Similarly the online version of Corollary \ref{corollary: approx_hessian_real_hessian_bound} also holds by following the same derivation as the proof of Corollary \ref{corollary: approx_hessian_real_hessian_bound} (except that $r$, $\xi_{j_1, j_m}$ and $d_{j_1, j_m + T_0 -1}$ is replaced by 1, $\xi_{j_1, j_m}(k-1)$ and $d_{j_1, j_m + T_0 -1}(k-1)$ respectively), i.e.:

\begin{corollary}[Approximation accuracy of quasi-Hessian to mean Hessian (online deletion)]\label{corollary: approx_hessian_real_hessian_bound_multi}
Suppose that at the $k_{th}$ deletion request, $\|\iw_{j_s}(k) - \iw_{j_s}(k-1)\| \leq \wikbounds $ and $\|\iw_{t}(k) - \iw_{t}(k-1)\| \leq \wikbounds$ where $s = 1,2,\dots, m$. Then for $ j_m \le t \leq j_m + T_0 - 1$
\beq\label{xi_multi_20}
% \|\bH_{t} - \B_{j_m}\| \leq \xi_{j_1,j_m}:= c_0 d_{j_1,j_m + T_0 - 1}\left(1+ \frac{\sqrt{m}[(1+a)^{m}-1]}{c_1}\right) 
% + c_0 M_2\frac{r}{n},
\|\bH_{t}^{k-1} - \B_{j_m}^{k-1}\| \leq \xi_{j_1,j_m}(k-1):= A d_{j_1,j_m + T_0 - 1}(k-1)
+ A \wikbounds,
\eeq 
where recall again that $c_0$ is the Lipschitz constant of the Hessian, $A = \frac{c_0\sqrt{m}[(1+a)^{m}-1]}{c_1} + c_0$, $d_{j_1,j_m + T_0 - 1}$ is the maximal gap between the iterates of the GD algorithm on the full data from $j_1$ to $j_m+T_0-1$ (see equation \eqref{d}), which goes to zero as $t\to\infty$), $a$ is a problem dependent constant defined in Theorem \ref{theorem: delta_model_para_bound}, $c_1$ is the "strong independence" constant from \eqref{assp: singular_lower_bound}.%, 
\end{corollary}


Based on this, let us derive the bound on $\|\nabla F_i(\iw_t(r))\|$, $\|\ag(\iw_{t}(r)) - \frac{1}{n-r}\sum_{i\not\in R_r}\nabla F_i(\iw_{t}(r))\|$ and $\|\ag(\iw_{t}(r))\|$

% Note that Lemma \ref{Lemma \ref{Lemma: bound_d_j}} still holds for $d_{j_1, j_m +T_0-1}(r-1)$

\begin{lemma}\label{lemma: gradient_multi_bound}
If at a given iteration $t$ such that $j_m \leq t \leq j_m +T_0 -1$, for all $k < r$, the following inequality holds:
$$\|\iw_{t}(k) - \iw_{t}(k-1)\| \leq \wikbounds$$
then for all $i=1,2,\dots,n$, the following inequality holds:
$$\|\nabla F_i(\iw_t(r-1))\| \leq \wikbounds Lr + c_2$$
\end{lemma}
\begin{proof}

First of all by using  that $\wikbounds \leq \wikbounds$, the following inequality holds:
$$\|\iw_{t}(k) - \iw_{t}(k-1)\| \leq \wikbounds \leq \wikbounds$$.

Then by adding and subtracting $\nabla F_i(\iw_t(r-2))$ inside $\|\nabla F_i(\iw_t(r-1))\|$, we get:
% This inequality is derived by induction:
\begin{align}
    \begin{split}
        & \|\nabla F_i(\iw_t(r-1))\|\\
        & = \|\nabla F_i(\iw_t(r-1)) - \nabla F_i(\iw_t(r-2)) + \nabla F_i(\iw_t(r-2))\|\\
        & \leq \|\nabla F_i(\iw_t(r-1)) - \nabla F_i(\iw_t(r-2))\| + \|\nabla F_i(\iw_t(r-2))\|\\
    \end{split}
\end{align}

The last inequality uses the triangle inequality. Then by using the Cauchy mean theorem, the upper bound on the eigenvalue of the Hessian matrix (i.e. Assumption \ref{assp: strong_convex smooth}) and the bound on $\|\iw_{t}(k) - \iw_{t}(k-1)\|$, the formula above is bounded as:
\begin{align*}
    & = \|\bH_i(\iw_t(r-1) + x(\iw_t(r-2)-\iw_t(r-1)))\cdot (\iw_t(r-1) - \iw_t(r-2))\|\\
    & + \|\nabla F_i(\iw_t(r-2))\|\\
    & \leq L \wikbounds + \|\nabla F_i(\iw_t(r-2))\|
\end{align*}

Then by using it recursively, the formula above becomes:
\begin{align*}
    & \leq \sum_{k=1}^{r-1} \wikbounds L + \|\nabla F_i(\iw_t(0))\|\\
    % & = \sum_{k=1}^{r} \wikbounds L + c_2 \\
    & \leq \wikbounds Lr + c_2
\end{align*}

\end{proof}



\begin{lemma}\label{lemma: approximate_vs_real_gradient_bound}
If at a given iteration $t$ such that $j_m \leq t \leq j_m +T_0 -1$, for all $k < r$, the following inequality holds:
$$\|\iw_{t}(k) - \iw_{t}(k-1)\| \leq \wikbounds$$ and $$\xi_{j_1,j_m}(k-1) \leq \frac{\mu}{2}$$, then the following inequality holds:
\begin{align*}
    \begin{split}
        &\|\frac{1}{n-r+1}\sum_{i\not\in R_{r-1}}\nabla F_i(\iw_t(r-1))-\ag(\iw_t(r-1))\|\\
        & \leq r\wikbounds \mu 
        % & \leq \sum_{k=0}^{r-1}\frac{n-k}{n-r}\frac{\mu}{2} (\frac{2n}{n-7k-8}M_1\frac{1}{n} ) := \Delta_r
        % &\leq \sum_{k=1}^r (1+\frac{k}{n-r})[A d_{j_1,j_m + T_0 - 1}(0)\\
        % & + A (\sum_{l=1}^k (C_{l-1}M_1\frac{1}{n} + D_{l-1}))](\sum_{l=1}^k (C_{l-1}M_1\frac{1}{n} + D_{l-1})):= \Delta_r
    \end{split}
\end{align*}
\end{lemma}
\begin{proof}
%Let us compute the difference 
%$\frac{1}{n-r+1}\sum_{i\not\in R_{r-1}}\nabla F_i(\iw_t(r-1))-\ag(\iw_t(r-1))$ and 
%use  that 
First of all, $\frac{1}{n-r+1}\sum_{i\not\in R_{r-1}}\nabla F_i(\iw_t(r-1))$ can be rewritten as below by using the Cauchy mean-value theorem:
\begin{align*}
\begin{split}
& \frac{1}{n-r+1}\sum_{i\not\in R_{r-1}}\nabla F_i(\iw_t(r-1))\\
& = \frac{1}{n-r+1}[\sum_{i\not\in R_{r-2}}\nabla F_i(\iw_t(r-1)) - \nabla F_{i_{r-1}}(\iw_t(r-1))]\\
& = \frac{1}{n-r+1}\{(n-r+2)[\bH_{t}^{r-2}\times (\iw_t(r-1) - \iw_t(r-2)]\\
& + \sum_{i\not\in R_{r-2}}\nabla F_i(\iw_t(r-2)) - \nabla F_{i_{r-1}}(\iw_t(r-1))\}
\end{split}
\end{align*}
    
By subtracting the above formula from Formula \eqref{eq: g_w_k_deriv},
% , i.e. $$\ag(\iw_t(r)) = \frac{1}{n-r}[(n-r+1)(\B_{j_m}(\iw_t(r) - \iw_t(r-1)) + \ag(\iw_t(r-1))) - \nabla F_{i_r}(\iw_t(r))]$$
% \ag(\iw_t(r-1)) + \B_{j_m}\times (\iw_t(r) - \iw_t(r-1))$$, 
we get:
\begin{align}
\begin{split}
    & \|\frac{1}{n-r+1}\sum_{i\not\in R_{r-1}}\nabla F_i(\iw_t(r-1)) - \ag(\iw_t(r-1))\| \\
    & = \frac{1}{n-r+1}\|(n-r+2)(\bH_t^{r-2}-\B_{j_m}^{r-2})\times (\iw_t(r-1) - \iw_t(r-2))\\
    & + \sum_{i\not\in R_{r-2}}\nabla F_i(\iw_t(r-2))- (n-r+2)\ag(\iw_t(r-2)) \|\\
\end{split}
\end{align}

Then by using the triangle inequality, Corollary \ref{corollary: approx_hessian_real_hessian_bound_multi} and the bound on $\|\iw_t(r-1)-\iw_t(r-2)\|$, the formula above is bounded as:
\begin{align}\label{eq: real_approx_gradient_gap_deriv1}
    \begin{split}
        & \leq \frac{n-r+2}{n-r+1}\|\bH_t^{r-2} - \B_{j_m}^{r-2}\|\|\iw_t(r-1) - \iw_t(r-2)\|\\
        & + \frac{1}{n-r+1} \|\sum_{i\not\in R_{r-2}}\nabla F_i(\iw_t(r-2)) - (n-r+2)\ag(\iw_t(r-2))\| \\
        & \leq \frac{n-r+2}{n-r+1}\xi_{j_1,j_m}(r-2) \wikbounds\\
        & + \frac{n-r+2}{n-r+1}\|\frac{1}{n-r+2}\sum_{i\not\in R_{r-2}}\nabla F_i(\iw_t(r-2)) - \ag(\iw_t(r-2))\|
    \end{split}
\end{align}

By using  that $\xi_{j_1,j_m}(r-2) \leq \frac{\mu}{2}$, the formula above is bounded as:
\begin{align*}
    & \leq \frac{n-r+2}{n-r+1}\frac{\mu}{2} (\wikbounds )\\
        & + \frac{n-r+2}{n-r+1}\|\frac{1}{n-r+2}\sum_{i\not\in R_{r-2}}\nabla F_i(\iw_t(r-2)) - \ag(\iw_t(r-2))\|
\end{align*}

By applying it recursively (Note that $\nabla F(\iw_t(0)) = \ag(\iw_t(0))$). In the end, we get the following inequality:
\begin{align*}
    \begin{split}
        & \leq \sum_{k=1}^{r-1}\frac{n-k}{n-r}\frac{\mu}{2} (\wikbounds)\\
        & \leq \wikbounds\frac{\mu}{2} \sum_{k=1}^{r-1}\frac{n-k}{n-r}
        % ((1+\frac{r}{n-r})\frac{\mu}{2} + (1+\frac{r-1}{n-r})\xi_{j_1,j_m}(1) + \dots +(1+\frac{1}{n-r})\xi_{j_1,j_m}(r-1)) \\
        % &\cdot (\frac{2n}{n-7k-1}M_1\frac{1}{n} )
    \end{split}
\end{align*}

Also for $r \ll n$, $\frac{n-k}{n-r} \leq 2$. So the formula above can be bounded as:
\begin{align*}
    \begin{split}
        & \leq r\wikbounds \mu 
    \end{split}
\end{align*}

% Then based on Lemma \ref{lemma: bound_d_j_multi}, $$\xi_{j_1,j_m}(k) = A d_{j_1,j_m + T_0 - 1}(k)
% + A (\frac{2n}{n-7k-1}M_1\frac{1}{n} )$$
% % $$Ad_{j_a,j_b + T_0 - 1}(0)
% % + A\frac{2Ck}{\frac{1}{2}-\frac{1}{n}}M_1\frac{1}{n}$$
% $$\leq A d_{j_1,j_m + T_0 - 1}(0)
% + A \sum_{l=1}^k (C_{l-1}M_1\frac{1}{n} + D_{l-1})$$, the formula above can be further bounded as:
% \begin{align}
%     \begin{split}
%         & \leq 
%         \sum_{k=1}^r (1+\frac{k}{n-r})[A d_{j_1,j_m + T_0 - 1}(0) + (A \sum_{l=1}^k (C_{l-1}M_1\frac{1}{n} + D_{l-1}))]\\
%         & \cdot (\frac{2n}{n-7k-1}M_1\frac{1}{n} ):= \Delta_r\\
%         % & = [(\frac{nr}{n-r}-\frac{r(r-1)}{2(n-r)})Ad_{j_1,j_m +T_0 - 1}(0)\\
%         % & + (\frac{r(r+1)(2r+1)}{3(n-r)} + r^2 - \frac{r(r+1)}{2(n-r)})A\frac{M_1}{\frac{1}{2}-\frac{1}{n}}\frac{C}{n}]\frac{M_1}{\frac{1}{2}-\frac{1}{n}}\frac{C}{n} 
%     \end{split}
% \end{align}

\end{proof}

Note that for $\|\frac{1}{n-r+1}\sum_{i\not\in R_{r-1}}\nabla F_i(\iw_t(r-1))-\ag(\iw_t(r-1))\|$, we get a tighter bound when $t\rightarrow \infty$ by using Formula \eqref{eq: real_approx_gradient_gap_deriv1}, Lemma \ref{lemma: bound_d_j_multi} (i.e. $d_{j_a,j_b}(r) \leq d_{j_a,j_b}(0) + 2r\cdot \wikbounds$) and Lemma \ref{Lemma: bound_d_j} without using $\xi_{j_1,j_m}(r-1) \leq \frac{\mu}{2}$, which starts by bounding $\xi_{j_1,j_m}(k-1)$ where $k <= r$, $j_1 = j_0 + xT_0$ and $j_m = j_0 + (x+m-1)T_0$:

\begin{align}\label{eq: xi_bound_multi}
    \begin{split}
    & \xi_{j_1,j_m}(k-1) = A d_{j_1,j_m + T_0 - 1}(k-1)
+ A \wikbounds \\
& \leq A d_{j_1,j_m + T_0 - 1}(0) + 2(k-1)A \cdot \wikbounds\\
& 
+ A \wikbounds\\
& \leq A (1-\mu\eta)^{j_0 + xT_0}d_{0,mT_0-1}(0) + A(2k-1)\wikbounds
    \end{split}
\end{align}

Which can be plugged into Formula \eqref{eq: real_approx_gradient_gap_deriv1}:
\begin{align}\label{eq: real_approx_gradient_gap_tight}
    \begin{split}
        & \|\frac{1}{n-r+1}\sum_{i\not\in R_{r-1}}\nabla F_i(\iw_t(r-1))-\ag(\iw_t(r-1))\| \\
        & \leq \frac{n-r+2}{n-r+1}\xi_{j_1,j_m}(r-2) \wikbounds\\
        & + \frac{n-r+2}{n-r+1}\|\frac{1}{n-r+2}\sum_{i\not\in R_{r-2}}\nabla F_i(\iw_t(r-2)) - \ag(\iw_t(r-2))\|\\
        & \leq \sum_{k=1}^{r-1} \xi_{j_1,j_m}(k-1)\wikbounds\\
        & \leq \sum_{k=1}^{r-1}(A (1-\mu\eta)^{j_0 + xT_0}d_{0,mT_0-1}(0) + A(2k-1)\wikbounds)\\
        & \cdot\wikbounds\\
        & \leq A (1-\mu\eta)^{j_0 + xT_0}d_{0,mT_0-1}(0)r\wikbounds\\
        & + A(r\wikbounds)^2
    \end{split}
\end{align}

The last step uses  that $\wikbounds \leq \wikbounds$ and $\sum_{k=1}^{r-1} (2k-1) < \sum_{k=1}^r (2k-1) = r^2$. So when $t\rightarrow \infty$ and thus $x \rightarrow \infty$, $\|\frac{1}{n-r}\sum_{i\not\in R_r}\nabla F_i(\iw_t(r))-\ag(\iw_t(r))\| = o(\frac{r}{n})$

Then based on Lemma \ref{lemma: gradient_multi_bound} and \ref{lemma: approximate_vs_real_gradient_bound}, the bound on $\|\ag(\iw_t(r))\|$ becomes:
\begin{align}\label{eq: approximate_gradient_bound}
\begin{split}
    & \|\ag(\iw_t(r-1))\|\\
    & = \|\ag(\iw_t(r-1)) - \frac{1}{n-r+1}\sum_{i\not\in R_{r-1}}\nabla F_i(\iw_t(r-1))\\
    & + \frac{1}{n-r+1}\sum_{i\not\in R_{r-1}}\nabla F_i(\iw_t(r-1))\|\\
    & \leq \|\ag(\iw_t(r-1)) - \frac{1}{n-r+1}\sum_{i\not\in R_{r-1}}\nabla F_i(\iw_t(r-1))\|\\
    & + \|\frac{1}{n-r+1}\sum_{i\not\in R_{r-1}}\nabla F_i(\iw_t(r-1))\|\\
    % & \leq\Delta_r + \sum_{k=0}^{r-1} (\frac{2n}{n-7k-8}M_1\frac{1}{n} ) L + c_2\\
    & = r\wikbounds \mu + \wikbounds Lr + c_2
\end{split}
\end{align}

\textbf{Main results}

\begin{theorem}[Bound between iterates on full data and incrementally updated ones (online deletions)]\label{bfi_multi}
% Suppose that for some given $t$ we have the bounds $\|\bH_{t'} - \B_{j_m}\| \leq \xi_{j_1,j_m}$, and $\xi_{j_1,j_m} \leq (1-r/n)\mu - \beta$  for all possible values of $t'\le t$ and the  $j_1,\ldots,j_m$ corresponding to $t'$ (i.e., not just for the current values at $t$), for some positive $\beta>0$
% Then 
% $$\|\iw_{t+1} - \w_{t+1} \| \leq M_2 \frac{r}{n}$$ 
% where $M_2=\max(2c_2/\beta,M_1)$ is some positive constant, and recall that $M_1$ is defined in Theorem \ref{wu}. Neither depends on $t$.
Suppose that for any $k < r$, $\|\iw_{t}(k) - \iw_{t}(k-1)\| \leq \wikbounds$. At the $r_{th}$ deletion request, consider an iteration $t$ indexed with $j_m$ for which $j_m \leq t < j_m +T_0 -1$, and suppose that we are at the $x$-th iteration of full gradient updates, so  $j_1 = j_0 + xT_0$, $j_m = j_0 + (m - 1 + x) T_0$. Suppose that we have the bounds $\|\bH_{t}^{r-1} - \B_{j_m}^{r-1}\| \leq \xi_{j_1,j_m}(r-1) = Ad_{j_1,j_m + T_0 - 1}(r-1) + A(\wikbounds)$ (where we recalled the definition of $\xi$)  and $$\xi_{j_1,j_m}(r-1) = A d_{j_1,j_m + T_0 - 1}(r-1)
+ A (\wikbounds) \leq \frac{\mu}{2}$$ for all iterations $x$.
% and the  $j_1,\ldots,j_m$ corresponding to $t'$ (i.e., not just for the current values at $t$). % \ed{Need to double check that this is the right condition}. 
Then %for all $t$  $j_m \leq t \leq j_m + T_0$, 
$$\|\iw_{t+1}(r) - \iw_{t+1}(r-1) \| \leq
% \frac{2 c_2/n}{(1-1/n)\mu - \xi_{j_0,j_0+(m-1)T_0}(k-1)} \leq 
\wikbounds.$$ 
% $$\|\iw_{t+1} - \w_{t+1} \| \leq \frac{2r c_2/n}{(1-r/n)\mu - \xi_{j_1,j_m}}$$
% where $M_2=M_1 +  $ is some positive constant, and
Recall that $c_0$ is the Lipshitz constant of the Hessian, $M_1$ and $A$ are defined in Theorem \ref{wu_multi} and Corollary \ref{corollary: approx_hessian_real_hessian_bound_multi} respectively, and do not depend on $t$, 
\end{theorem}


Then by using the same derivation as the proof of Theorem \ref{bfi2}, we get the following results at the $r_{th}$ deletion request.

\begin{theorem}[Bound between iterates on full data and incrementally updated ones (all iterations, online deletion)]\label{bfi2_multi}
At deletion request $r$, if for all $k<r$, $\|\iw_t(k)-\iw_t(k-1)\| \leq \wikbounds$ holds, then for any $j_m < t < j_m +T_0 - 1$,  $$\|\iw_t(r)-\iw_t(r-1)\| \leq \wikbounds$$ and $$\|\bH_{t}^{r-1} - \B_{j_m}^{r-1}\| \leq \xi_{j_1,j_m}(r-1):= A d_{j_1,j_m + T_0 - 1}(r-1)
+ A \wikbounds$$ 
and $$\|\frac{1}{n-r+1}\sum_{i\not\in R_{r-1}}\nabla F_i(\iw_t(r-1))-\ag(\iw_t(r-1))\|\leq r\wikbounds \mu $$
hold
% the result $\iw_t$ of Algorithm \ref{alg: update_algorithm} approximates the correct iteration values $\uw_t$ at the rate 
% $\|\iw_t - \w_t\| \leq \frac{1}{\frac{1}{2}-\frac{r}{n}}M_1\frac{r}{n}$ and $\|\bH_{t} - \B_{j_m}\| \leq \xi_{j_1,j_m}$. 
% Recall that $j_1,\ldots,j_m$ depend on $t$,  $\xi_{j_1,j_m}$ is defined in \eqref{xi} and $M_3$ is the constant from Theorem \ref{main10}.
\end{theorem}


Then by induction (the base case is similar to Theorem \ref{bfi2}), we know that the following theorem holds for all iterations $t$:
\begin{theorem}[Bound between iterates on full data and incrementally updated ones (all iterations, all deletion requests, online deletion)]\label{bfi2_multi_all}
At the $r_{th}$ deletion request, for any $j_m < t < j_m +T_0 - 1$,  $$\|\iw_t(r)-\iw_t(r-1)\| \leq \wikbounds$$ and $$\|\bH_{t}^{r-1} - \B_{j_m}^{r-1}\| \leq \xi_{j_1,j_m}(r-1):= A d_{j_1,j_m + T_0 - 1}(r-1)
+ A \wikbounds$$ and 
$$\|\frac{1}{n-r+1}\sum_{i\not\in R_{r-1}}\nabla F_i(\iw_t(r-1))-\ag(\iw_t(r-1))\| \leq r\wikbounds \mu $$
hold
% the result $\iw_t$ of Algorithm \ref{alg: update_algorithm} approximates the correct iteration values $\uw_t$ at the rate 
% $\|\iw_t - \w_t\| \leq \frac{1}{\frac{1}{2}-\frac{r}{n}}M_1\frac{r}{n}$ and $\|\bH_{t} - \B_{j_m}\| \leq \xi_{j_1,j_m}$. 
% Recall that $j_1,\ldots,j_m$ depend on $t$,  $\xi_{j_1,j_m}$ is defined in \eqref{xi} and $M_3$ is the constant from Theorem \ref{main10}.
\end{theorem}

Then by induction (from the $r_{th}$ deletion request to the $1_{st}$ deletion request), the following inequality holds:
\begin{align}
    \|\iw_t(r)-\iw_t(0)\| = \|\iw_t(r)-\w_t\| \leq r \cdot \wikbounds
\end{align}

Then by using Formula \eqref{eq: w_u_w_gap}, the following inequality holds:
\begin{align}\label{eq: w_u_w_i_prev_bound}
    \begin{split}
    &\|\uw_t(r) - \iw_t(r-1)\| = \|\uw_t(r) - \w_t + \w_t - \iw_t(r-1)\|\\
    & \leq \|\uw_t(r) - \w_t\| + \|\w_t - \iw_t(r-1)\| \\
    & \leq M_1 \frac{r}{n} + (r-1)\cdot \wikbounds := M_2 \frac{r}{n}        
    \end{split}
\end{align}

where $M_2$ is a constant which does not depend on $t$ or $k$.

In the end, we get a similar results for the bound on $\|\iw_t(r) - \uw_t(r)\|$:
\begin{theorem}
[Convergence rate of \Increm\ (online deletion)]\label{main10_multi}
% Suppose 
% $\xi_{j_0,j_0+(m-1)T_0} \leq \min\{\frac{\mu}{2}, (1-\frac{r}{n})\mu - \frac{c_0M_1 r(n-r)}{2n^2}\}$ (recall $\xi$ was defined in \eqref{xi}) for all $t$ 
At the $r_{th}$ deletion request, for all iterations $t$, the result $\iw_t(r)$ of \Increm, Algorithm \ref{alg: update_algorithm_online}, approximates the correct iteration values $\uw_t(r)$ at the rate
$$\|\uw_t(r) - \iw_t(r)\| = o(\frac{r}{n}).$$
So $\|\uw_t(r) - \iw_t(r)\|$ is of a lower order than $\frac{r}{n}$.
% Here $M_3$ is a problem dependent constant that does not depend on $t$.
\end{theorem}



\textbf{The proof of Theorem \ref{bfi_multi}}
\begin{proof}

Note that the approximated update rules for $\iw_{t}$ at the $r_{th}$ and the $(r-1)_{st}$ deletion request are:
\begin{align}\label{eq: update_rule_w_it_curr}
\begin{split}
    & \iw_{t+1}(r) = \iw_t(r) - \frac{\eta}{n-r}[(n-r+1)(\B_{j_m}^{r-1}(\iw_t(r) - \iw_t(r-1))\\
    & + \ag(\iw_{t}(r-1))) - \nabla F_{i_r}(\iw_t(r))]
\end{split}
\end{align}

and 
\begin{align}\label{eq: update_rule_w_it_prev0}
\begin{split}
    & \iw_{t+1}(r-1) = \iw_{t}(r-1) \\
    & - \frac{\eta}{n-r+1}[(n-r+2)(\B_{j_m}^{r-2}(\iw_t(r-1) - \iw_t(r-2))\\
    & + \ag(\iw_{t}(r-2))) - \nabla F_{i_{r-1}}(\iw_t(r-1))]
\end{split}
\end{align}

Note that since $$\ag(\iw_t(r-1)) = \frac{1}{n-r+1}[(n-r+2)(\B_{j_m}^{r-2}(\iw_t(r-1) - \iw_t(r-2))$$
$$+ \ag(\iw_t(r-2))) - \nabla F_{i_{r-1}}(\iw_t(r-1))]$$
Then Formula \eqref{eq: update_rule_w_it_prev0} can be rewritten as:
\begin{align}\label{eq: update_rule_w_it_prev}
    \begin{split}
    & \iw_{t+1}(r-1) = \iw_{t}(r-1) \\
    & - \frac{\eta}{n-r+1}[(n-r+2)(\B_{j_m}^{r-2}(\iw_t(r-1) - \iw_t(r-2))\\
    & + \ag(\iw_{t}(r-2))) - \nabla F_{i_{r-1}}(\iw_t(r-1))]\\
    & = \iw_{t}(r-1) - \eta \ag(\iw_t(r-1))
\end{split}
\end{align}

Then by subtracting Formula \eqref{eq: update_rule_w_it_prev0} from Formula \eqref{eq: update_rule_w_it_prev}, the result becomes:

\begin{align}
\begin{split}
    & \iw_{t+1}(r) - \iw_{t+1}(r-1) \\
    & = (\iw_{t}(r) - \iw_{t}(r-1)) - \frac{\eta}{n-r}[(n-r+1)(\B_{j_m}^{r-1}(\iw_t(r) - \iw_t(r-1))\\
    & + \ag(\iw_{t}(r-1))) - \nabla F_{i_r}(\iw_t(r))] + \eta \ag(\iw_t(r-1))
\end{split}
\end{align}

Then by adding and subtracting $\bH_t^{r-1}$ and $\frac{1}{n-r+1}\sum_{i\not\in R_{r-1}}\nabla F(\iw_t(r-1))$ in the formula above and rearranging the result properly, it becomes:
\begin{align}\label{eq: w_i_t_prev_curr_gap_1}
\begin{split}
    & \iw_{t+1}(r) - \iw_{t+1}(r-1) \\
    & = (\textbf{I} - \eta\frac{n-r+1}{n-r}(\B_{j_m}^{r-1} - \bH_t^{r-1}))(\iw_{t}(r) - \iw_{t}(r-1))\\
    & - \frac{\eta}{n-r}[(n-r+1)(\bH_t^{r-1}(\iw_t(r) - \iw_t(r-1))\\
    & + \frac{1}{n-r+1}\sum_{i\not\in R_{r-1}}\nabla F(\iw_t(r-1)) - \frac{1}{n-r+1}\sum_{i\not\in R_{r-1}}\nabla F(\iw_t(r-1)) \\
    & + \ag(\iw_{t}(r-1))) - \nabla F_{i_r}(\iw_t(r))] + \eta \ag(\iw_t(r-1))\\
\end{split}
\end{align}


Then by using  that 
\begin{align*}
    & \bH_t^{r-1}(\iw_t(r) - \iw_t(r-1)) + \frac{1}{n-r+1}\sum_{i\not\in R_{r-1}}\nabla F(\iw_t(r-1))\\
    & = \frac{1}{n-r+1}\sum_{i\not\in R_{r-1}}\nabla F(\iw_t(r))
\end{align*}

and $$(\sum_{i\not\in R_{r-1}}\nabla F(\iw_t(r))) - \nabla F_{i_r}(\iw_t(r)) = \sum_{i\not\in R_{r}}\nabla F(\iw_t(r))$$

Formula \eqref{eq: w_i_t_prev_curr_gap_1} becomes:
\begin{align}\label{eq: w_i_t_prev_curr_gap_2}
\begin{split}
    & \iw_{t+1}(r) - \iw_{t+1}(r-1) \\
    & = (\textbf{I} - \eta\frac{n-r+1}{n-r}(\B_{j_m}^{r-1} - \bH_t^{r-1}))(\iw_{t}(r) - \iw_{t}(r-1))\\
    & - \frac{\eta}{n-r}[\sum_{i\not\in R_{r}}\nabla F(\iw_t(r)) - \sum_{i\not\in R_{r-1}}\nabla F(\iw_t(r-1)) \\
    & + (n-r+1)\ag(\iw_{t}(r-1))] + \eta \ag(\iw_t(r-1))\\
\end{split}
\end{align}

Also note that by using the Cauchy mean-value theorem, the following equation holds:
\begin{align*}
    \begin{split}
        & \sum_{i\not\in R_{r}}\nabla F_i(\iw_t(r)) - \sum_{i\not\in R_{r-1}}\nabla F_i(\iw_t(r-1)) \\
        & = \sum_{i\not\in R_{r}}\nabla F_i(\iw_t(r)) - \sum_{i\not\in R_{r}}\nabla F_i(\iw_t(r-1)) - \nabla F_{i_r}(\iw_t(r-1)) \\
        & = [\sum_{i \not\in R_r} \int_0^1 \bH_i(\iw_{t}(r-1) + x (\iw_{t}(r) - \iw_{t}(r-1)))dx](\iw_t(r)-\iw_t(r-1))\\
        & - \nabla F_{i_r}(\iw_t(r-1))
    \end{split}
\end{align*}

which can be plugged into Formula \eqref{eq: w_i_t_prev_curr_gap_2}, i.e.:
\begin{align}\label{eq: w_i_t_prev_curr_gap_3}
\begin{split}
    & \iw_{t+1}(r) - \iw_{t+1}(r-1) \\
    & = (\textbf{I} - \eta\frac{n-r+1}{n-r}(\B_{j_m}^{r-1} - \bH_t^{r-1}))(\iw_{t}(r) - \iw_{t}(r-1))\\
    & - \frac{\eta}{n-r}\{[\sum_{i \not\in R_r} \int_0^1 \bH_i(\iw_{t}(r-1) + x (\iw_{t}(r) - \iw_{t}(r-1)))dx]\\
    & \cdot(\iw_{t}(r) - \iw_{t}(r-1)) - \nabla F_{i_r}(\iw_t(r-1))\\
    & + (n-r+1)\ag(\iw_{t}(r-1))\} + \eta \ag(\iw_t(r-1))\\
\end{split}
\end{align}

which can be rearranged as:
\begin{align}\label{eq: w_i_t_prev_curr_gap_4}
\begin{split}
    & \iw_{t+1}(r) - \iw_{t+1}(r-1) \\
    & = (\textbf{I} - \eta\frac{n-r+1}{n-r}(\B_{j_m}^{r-1} - \bH_t^{r-1}))(\iw_{t}(r) - \iw_{t}(r-1))\\
    & - \frac{\eta}{n-r}\{[\sum_{i \not\in R_r} \int_0^1 \bH_i(\iw_{t}(r-1) + x (\iw_{t}(r) - \iw_{t}(r-1)))dx]\\
    & \cdot(\iw_{t}(r) - \iw_{t}(r-1)) - \nabla F_{i_r}(\iw_t(r-1))\} - \frac{\eta}{n-r}\ag(\iw_t(r-1))\\
\end{split}
\end{align}

Then by taking the matrix norm on both sides of Formula \eqref{eq: w_i_t_prev_curr_gap_4} and using  that $\|\bH_i(\iw_{t}(r-1) + x (\iw_{t}(r) - \iw_{t}(r-1)))\| \geq \mu$ and $\|\B_{j_m}^{r-1} - \bH_t^{r-1}\| \leq \xi_{j_1,j_m}(r-1)$, Formula \eqref{eq: w_i_t_prev_curr_gap_4} can be bounded as:
\begin{align}
    \begin{split}
        & \|\iw_{t+1}(r) - \iw_{t+1}(r-1)\|\\
        & \leq (1-\eta\mu)\|\iw_{t}(r) - \iw_{t}(r-1)\| \\
        & + \frac{(n-r+1)\eta}{n-r}\xi_{j_1,j_m}(r-1)\|\iw_{t}(r) - \iw_{t}(r-1)\|\\
        & + \frac{\eta}{n-r}\|\nabla F_{i_r}(\iw_t(r-1))\|\\
        & + \|\frac{\eta}{n-r}\ag(\iw_t(r-1))\|\\
    \end{split}
\end{align}

Then by using Lemma \ref{lemma: gradient_multi_bound} and Formula \eqref{eq: approximate_gradient_bound}, the formula above becomes:
\begin{align*}
    & \leq (1-\eta\mu + \frac{(n-r+1)\eta}{n-r}\xi_{j_1,j_m}(r))\|\iw_{t}(r) - \iw_{t}(r-1)\|\\
        & + \frac{\eta}{n-r}(\wikbounds L(r-1) + c_2)\\
        & + \frac{\eta}{n-r}(\wikbounds(r-1)\mu + \wikbounds L(r-1) + c_2)
\end{align*}

By using the bound on $\xi_{j_1,j_m}(r)$ and applying the above formula recursively across all iterations, the formula above becomes:
\begin{align}
    \begin{split}
    & \leq \frac{1}{\eta\mu - \frac{\eta(n-r+1)}{n-r}\frac{\mu}{2}}(\frac{\eta}{n-r}(\wikbounds L(r-1) + c_2)\\
    & + \frac{\eta}{n-r}(\wikbounds L(r-1) + \wikbounds \mu (r-1) + c_2)\\
    & = \frac{2}{(n-r-1)\mu}((\wikbounds (2L(r-1) + (r-1)\mu) + 2c_2)\\
    \end{split}
\end{align}

Then by using  that $M_1 = \frac{2c_2}{\mu}$ and $\wikbounds = \wikbound{r}$, the formula above can be rewritten as:
\begin{align*}
    & = \frac{2}{(n-r-1)\mu}\frac{\frac{2M_1(r-1)}{n}(2L+\mu) + \mu M_1 (1-\frac{r+1}{n} - \frac{2(r-1)}{n}(\frac{2L+\mu}{\mu})) }{1-\frac{r+1}{n} - \frac{2(r-1)}{n}(\frac{2L+\mu}{\mu})}\\
    & = \frac{2 \frac{M_1}{n}}{1-\frac{r+1}{n} - \frac{2(r-1)}{n}(\frac{2L+\mu}{\mu})} = \wikbounds
\end{align*}

This finishes the proof.

% Then by using  that $\frac{2n}{n-7k-8} \leq \frac{2n}{n-7r-1}$ and $\frac{n-k}{n-r} \leq \frac{n}{n-r} \leq 2$ for $r \ll n$, then the formula above can be bounded as:
% \begin{align*}
%     & \leq \frac{2}{(n-r-1)\mu}(((\frac{2r}{n-7r-1}M_1 ) L + c_2)\\
%     & + \mu (\frac{2n}{n-7r-1}M_1\frac{r}{n} ) + (\frac{2r}{n-7r-1}M_1) L + c_2)
% \end{align*}

% Also by using  that $M_1 = \frac{2c_2}{\mu}$ and $\mu < L$, the formula above can be further bounded as:
% \begin{align*}
%     & \leq 
% \end{align*}

% First of all, in the update rule for $\w_{t}(r-1)$, we add and subtract $\bH_t^{r-1}$ and $\B_t^{r-1}$, i.e.:
% \begin{align*}
%     \begin{split}
%         &\iw_{t+1}(r-1) = \iw_t(r-1)- \frac{\eta}{n-r+1}[(n-r+2)(\B_{j_m}^{r-1}(\iw_t(r-1) - \iw_t(r-2))\\
%         &+ \ag(\iw_{t}(r-2))) - \nabla F_{i_{r-1}}(\iw_t(r-1))]\\
%         & = \iw_t(r-1)- \frac{\eta}{n-r+1}[(n-r+2)(\bH_t^{r-1}(\iw_t(r-1) - \iw_t(r-2))\\
%         & + (\B_{j_m}^{r-1} - \bH_t^{r-1})(\iw_t(r-1) - \iw_t(r-2))\\
%         &+ \frac{1}{n-r+2}\sum_{i\not\in R_{r-2}} \nabla F_i(\iw_t(r-2)) + \ag(\iw_{t}(r-2))\\
%         & - \frac{1}{n-r+2}\sum_{i\not\in R_{r-2}} \nabla F_i(\iw_t(r-2))) - \nabla F_{i_{r-1}}(\iw_t(r-1))]\\
%     \end{split}
% \end{align*}

% Then by using  that
% \begin{align*}
%     \begin{split}
%     & \bH_t^{r-1}(\iw_t(r-1)-\iw_t(r-2)) + \frac{1}{n-r+2}\sum_{i\not\in R_{r-2}} \nabla F_i(\iw_t(r-2))\\
%     & = \frac{1}{n-r+2}\sum_{i\not\in R_{r-2}} \nabla F_i(\iw_t(r-1)) - \frac{1}{n-r+2}\sum_{i\not\in R_{r-2}} \nabla F_i(\iw_t(r-2))\\
%     & + \frac{1}{n-r+2}\sum_{i\not\in R_{r-2}} \nabla F_i(\iw_t(r-2)) = \frac{1}{n-r+2}\sum_{i\not\in R_{r-2}} \nabla F_i(\iw_t(r-1))
%     \end{split}
% \end{align*}

% The formula above can be rearranged as:
% \begin{align}\label{eq: rearrange_w_t_r}
% \begin{split}
% &\w_{t+1}(r-1) = \w_t(r-1)-\frac{\eta}{n-r+1}\sum_{i\not\in R_{r-1}}\nabla F_i(\w_t(r-1))\\
%     & -\frac{\eta(n-r+2)}{n-r+1}(\B_{j_m}^{r-1}-\bH_{t}^{r-1})(\iw_t(r-1)-\iw_t(r-2))\\
%     & - \frac{\eta(n-r+2)}{n-r+1}[\ag(\iw_t(r-2)) - \frac{\eta}{n-r+1}\sum_{i \not\in R_{r-2}}\nabla F_i(\iw_t(r-2))]    
% \end{split}
% \end{align}



% The updates for the iterations $j_m \leq t \leq j_m + T_0 - 1$ follow the quasi-Hessian update. We proceed in a similar way as before but by using equation \eqref{eq: rearrange_w_t_r} as the update rule for $\iw_t(r-1)$ instead. Plus, we use the condition $\|\iw_t(r-1) - \iw_t(r-2)\| \leq \frac{CM_1}{\frac{1}{2}-\frac{1}{n}}\frac{1}{n}$ and  that $\|\frac{1}{n-r}\sum_{i\not\in R_r}\nabla F_i(\iw_t(r))-\ag(\iw_t(r))\| \leq \Delta_r$ (See Lemma \ref{lemma: approximate_vs_real_gradient_bound}) and $\|\bH_{t}^{k-1} - \B_{j_m}^{k-1}\| \leq \xi_{j_1,j_m}(k-1)$ (see Corollary \ref{corollary: approx_Hessian_real_Hessian_bound_multi}), it can be bounded as: 

% \begin{align}\label{eq: iw_bound_multi_00}
%     \begin{split}
%         & \|\iw_{t+1}(r) - \uw_{t+1}(r-1) \|\\
%         & \leq \|\iw_{t}(r) - (\uw_{t}(r-1) - \frac{\eta}{n-r+1}\sum_{i\not\in R_{r-1}} \nabla F_i(\uw_t(r-1))) \\
%         & - \frac{\eta}{n-r}[(n-r+1)(\B_{j_m}(\iw_t(r) - \iw_t(r-1)) + \ag(\iw_{t}(r-1)))\\
%         & - \nabla F_{i_r}(\iw_t(r))]\|
%         % &+ \frac{\eta(n-r+2)}{n-r+1}\xi_{j_1,j_m}(r-1)\frac{CM_1}{\frac{1}{2}-\frac{1}{n}}\frac{1}{n}\\
%         % & + \frac{\eta(n-r+2)}{n-r+1}\Delta_{r-2}
%         % & = \|(\textbf{I} - \eta \frac{n}{n-r} \B_{j_m})(\iw_t(k) - \iw_t(k-1))\\
%         % & - \frac{r\eta}{n-r}\nabla F(\iw_t(k)) + \frac{\eta}{n-r} \sum_{i\in R} \nabla F_i(\iw_{t})  \|\\
%     \end{split}
% \end{align}

% Then by adding and subtracting $\frac{\eta}{n-r+1}\sum_{i\not\in R_{r-1}} \nabla F_i(\iw_t(r-1))$ and use the Lemma \ref{lemma: bound_d_j_multi} and triangle inequality, the above formula leads to:
% \begin{align}
%     \begin{split}
%         & = \|\iw_{t}(r) - (\uw_{t}(r-1) - \frac{\eta}{n-r+1}\sum_{i\not\in R_{r-1}} \nabla F_i(\uw_t(r-1))) \\
%         & - \frac{\eta}{n-r}((n-r+1)[\B_{j_m}\left(\iw_{t}(r) - \iw_{t}(r-1)\right) + \frac{\eta}{n-r+1}\sum_{i\not\in R_{r-1}} \nabla F_i(\iw_t(r-1)) \\
%         & + \ag(\iw_{t}(r-1)) - \frac{\eta}{n-r+1}\sum_{i\not\in R_{r-1}} \nabla F_i(\iw_t(r-1))]- \nabla F_{i_r}\left(\iw_{t}(r)\right))\|\\
%         % &  + \frac{\eta(n-r+2)}{n-r+1}\xi_{j_1,j_m}(r-1)\frac{CM_1}{\frac{1}{2}-\frac{1}{n}}\frac{1}{n} + \frac{\eta(n-r+2)}{n-r+1}\Delta_{r-2}\\
%         & \leq \|\iw_{t}(r) - (\uw_{t}(r-1) - \frac{\eta}{n-r+1}\sum_{i\not\in R_{r-1}} \nabla F_i(\uw_t(r-1))) \\
%         & - \frac{\eta}{n-r}((n-r+1)[\B_{j_m}\left(\iw_{t}(r) - \iw_{t}(r-1)\right) + \frac{\eta}{n-r+1}\sum_{i\not\in R_{r-1}} \nabla F_i(\iw_t(r-1))] \\
%         &- \nabla F_{i_r}\left(\iw_{t}(r)\right))\| + \frac{n\eta}{n-r}\Delta_{r-1}\\
%         & \leq \|\iw_{t}(r) - (\uw_{t}(r-1) - \frac{\eta}{n-r+1}\sum_{i\not\in R_{r-1}} \nabla F_i(\uw_t(r-1))) \\
%         & - \frac{\eta}{n-r}((n-r+1)[\bH_t\left(\iw_{t}(r) - \iw_{t}(r-1)\right) + \frac{\eta}{n-r+1}\sum_{i\not\in R_{r-1}} \nabla F_i(\iw_t(r-1))] \\
%         &- \nabla F_{i_r}\left(\iw_{t}(r)\right))\| + \frac{n\eta}{n-r}\Delta_{r-1} + \frac{(n-r+1)\eta}{n-r}\|(\bH_t - \B_{j_m})(\iw_t(r)-\iw_t(r-1))\|\\
%         % &+ \frac{\eta n}{n-r}\|\B_{j_m}(\iw_{r-1} - \uw_{r-1})\|
%         % & + \frac{\eta(n-r+2)}{n-r+1}\xi_{j_1,j_m}(r-1)\frac{CM_1}{\frac{1}{2}-\frac{1}{n}}\frac{1}{n} + \frac{\eta(n-r+2)}{n-r+1}\Delta_{r-2}\\
%     \end{split}
% \end{align}

% % Then by defining $$\Psi_r = \frac{n\eta}{n-r}\Delta_{r-1} + \frac{\eta(n-r+2)}{n-r+1}\xi_{j_1,j_m}(r-1)\frac{CM_1}{\frac{1}{2}-\frac{1}{n}}\frac{1}{n} + \frac{\eta(n-r+2)}{n-r+1}\Delta_{r-2}$$, 
% By rearranging the formula and using the triangle inequality.
% \begin{align}
%     \begin{split}
%         & 
%     \end{split}
% \end{align}


% \begin{align}
%     \begin{split}
%         & = \|(\textbf{I} - \eta \frac{n}{n-r} \B_{j_m})(\iw_t(r) - \iw_t(r-1)) - \frac{r\eta}{n-r}\nabla F(\iw_t(r-1))\\
%         & + \frac{\eta}{n-r} \sum_{i\in R} (\bH_{t,i}\mmop(\iw_t(r) - \iw_t(r-1)) + \nabla F_i(\w_{t}))\| + \Psi_r\\
%         & \leq \|(\textbf{I} - \eta \frac{n}{n-r} \B_{j_m})(\iw_t(r) - \iw_t(r-1))\| + \|\frac{r\eta}{n-r}\nabla F(\iw_t(r-1))\|\\
%         & + \|\frac{\eta}{n-r} \sum_{i\in R} \bH_{t,i}\mmop(\iw_t(r) - \iw_t(r-1))\| + \|\frac{\eta}{n-r} \nabla F_{i_r}(\w_{t})\|+ \Psi_r\\
%     \end{split}
% \end{align}
% The terms in the first absolute value can be rewritten as
% \begin{align}
%     \begin{split}
%         & [\textbf{I} - \eta \frac{n}{n-r} (\B_{j_m} - \bH_{t} + \bH_{t})](\iw_t(r) - \iw_t(r-1)) + \frac{\eta}{n-r} \sum_{i\in R} \bH_{t}\mmop(\iw_t(r) - \iw_t(r-1))\\
%         & = [\textbf{I} - \eta \frac{n}{n-r} (\B_{j_m} - \bH_{t})](\iw_t(r) - \iw_t(r-1)) - \frac{\eta}{n-r} \sum_{i \not\in R} \bH_{t}\mmop(\iw_t(r) - \iw_t(r-1))
%             \end{split}
% \end{align}
% we again bound
% \begin{align}\label{eq: iw_bound_last0}
%     \begin{split}
%         & \leq \|[\textbf{I} - \frac{\eta}{n-r}\sum_{i \not\in R} \bH_{t}](\iw_t(r) - \iw_t(r-1))\| + \frac{n\eta}{n-r}\|(\B_{j_m} - \bH_{t})(\iw_t(r) - \iw_t(r-1))\|\\
%         & + \|\frac{r\eta}{n-r}\nabla F(\iw_t(r-1))\| + \|\frac{\eta}{n-r} \nabla F_{i_r}(\w_{t})\| +\Psi_r\\
%         % & \leq (\|\textbf{I} - \eta \frac{n}{n-r}\bH_{j_m}\| + \eta \frac{n}{n-r}\|\B_{j_m} - \bH_{j_m}\|)(\iw_t(r) - \iw_t(r-1))\| + \frac{r\eta c_2}{n-r}\\
%         % & + \frac{\eta r L}{n-r} \|(\iw_t(r) - \iw_t(r-1))\| + \frac{\etar c_2}{n-r}\\
%         & \leq (1 - \eta \mu + \eta \frac{n}{n-r}\xi_{j_1,j_m})\|\iw_t(r) - \iw_t(r-1)\| + \frac{(r+1)\eta c_2}{n-r} + \Psi_r\\
%         % & = (1 - \eta \frac{n}{n-r}\mu + \eta \frac{n}{n-r}\ep_{j_1,j_m} + \frac{\etar L}{n-r})\|\iw_t(r) - \iw_t(r-1)\| + \frac{2r\eta c_2}{n-r}
%         % & = \|\iw_{t} - \frac{\eta}{n-r}(n \left[\bH_{t}\left(\iw_{t} - \w_{t}\right)\\
%         % & + (\bH_{t} - \B_{j_m})\left(\iw_{t} - \w_{t}\right) + \nabla F\left(\w_{t}\right)\right])- \sum_{\substack{i \in R}} \left(\nabla F_i\left(\w_{t}\right) + \bH_{t,i} (\iw_{t} - \iw_t(r-1)) \right)\|\\
%     \end{split}
% \end{align}

% Then according to Lemma \ref{Lemma: bound_d_j}, $d_{j_1,j_m + T_0 - 1} = d_{j_0+xT_0,j_0 + (x+m)T_0 - 1}$ decreases with increasing $x$, and thus $\xi_{j_1,j_m} = Ad_{j_1,j_m + T_0 - 1} + \frac{1}{\frac{1}{2}-\frac{r}{n}}AM_1 \frac{r}{n}$ is also decreasing with increasing $x$. So the formula above can be further bounded as:
% \begin{align}
%     \begin{split}
%         \leq (1-\eta\mu + \eta\frac{n}{n-r}\xi_{j_0,j_0+(m-1)T_0})\|\iw_t(r)-\iw_t(r-1)\| + \frac{2r\eta c_2}{n-r}+\Psi_r
%     \end{split}
% \end{align}

% This shows a recurrent inequality for $\|\iw_t(r) - \iw_t(r-1)\|$. Note that by assumption, $\xi_{j_1,j_m} \leq \frac{\mu}{2}$. Next, notice that the conditions for deriving the above inequality hold for all $j_m \le t \leq j_m + T_0 - 1$. 

% Then, when we reach $t=j_m$, we have an iteration where the gradient is computed exactly.   For these iterations we have
% $$\iw_{t+1}(r) = \iw_{t}(r) - \frac{\eta}{n-r} \sum_{i\not\in R_r}\nabla F(\iw_t(r))$$
% as well as $\iw_{t+1}(r) = \iw_{t}(r) - \eta \nabla F\left(\iw_t(r)\right)$. Using the same argument as in the bound for $\iw_{t+1}(r) - \iw_{t}(r)$ we find
% \begin{align*}
%     & \|\iw_{t+1}(r) - \iw_{t+1}(r-1)\|
%     \leq \left[1-\eta \mu \right]\|\iw_{t}(r) - \iw_{t}(r-1)\| + \frac{2c_2r \eta}{n-r}
% \end{align*}
% Therefore, we effectively have $\xi=0$ for these iterations. we then continue with $t\gets t-1$, and use the appropriate bound among the two derived above. This recursive process works until we reach $t=1$.

% Iterating, and assuming $- \eta \mu + \eta \frac{n}{n-r}\xi_{j_1,j_m}<0$ for each $t$, we find %\ed{actually, we only go back until $j_m$, where we need a bound on $\|\iw_{j_m} - \w_{j_m}\|$}
% \begin{align*}
% \|\iw_{t}(r) - \iw_t(r-1) \| &\le \frac{2\frac{\eta r c_2}{n-r}+ \Psi_r}{\eta \mu - \eta \frac{n}{n-r}\xi_{j_0,j_0+(m-1)T_0}}\\
% &= \frac{2r c_2/n + (1-\frac{r}{n})\Psi_r }{(1-r/n)\mu - \xi_{j_0,j_0+(m-1)T_0}}
% \end{align*}

% Note that by using the definition of $\Psi_r$,  that $\frac{25}{16}r \leq (2Cr - C)$ for $r >= 2$ and the condition $A d_{j_a,j_b + T_0 - 1}(0) + A(C )^2\frac{M_1}{\frac{1}{2}-\frac{1}{n}}\frac{r}{n} \leq \frac{\mu}{2}$
% \begin{align*}
%         \begin{split}
%     & \Delta_r = \sum_{k=1}^r (1+\frac{k}{n-r})[A d_{j_1,j_m + T_0 - 1}(0) + A \frac{2k -  1}{\frac{1}{2}-\frac{1}{n}}M_1\frac{C}{n}]\frac{M_1}{\frac{1}{2}-\frac{1}{n}}\frac{C}{n} \\
%     & \leq \sum_{k=1}^r (1+\frac{k}{n-r})[A d_{j_1,j_m + T_0 - 1}(0)
% + A \frac{2r - 1}{\frac{1}{2}-\frac{1}{n}}M_1\frac{C}{n}]\frac{M_1}{\frac{1}{2}-\frac{1}{n}}\frac{C}{n}\\
% & \leq \sum_{k=1}^r (1+\frac{k}{n-r}) \frac{\mu}{2}\frac{M_1}{\frac{1}{2}-\frac{1}{n}}\frac{C}{n}\\
% & = (1 + \frac{r+1}{n-r})\frac{\mu}{2}\frac{M_1}{\frac{1}{2}-\frac{1}{n}}\frac{Cr}{n}\leq \frac{3}{4}\mu\frac{M_1}{\frac{1}{2}-\frac{1}{n}}\frac{Cr}{n}
%     % & = [A d_{j_a,j_b + T_0 - 1}(0) + A(C )^2\frac{M_1}{\frac{1}{2}-\frac{1}{n}}\frac{r}{n}] \frac{M_1}{\frac{1}{2}-\frac{1}{n}}\frac{r}{n}\\
%     % & \leq [A d_{j_a,j_b + T_0 - 1}(0) + A((2Cr-C)\frac{M_1}{\frac{1}{2}-\frac{1}{n}}\frac{r}{n}] \frac{M_1}{\frac{1}{2}-\frac{1}{n}}\frac{r}{n} \leq \frac{\mu}{2}\frac{M_1}{\frac{1}{2}-\frac{1}{n}}\frac{r}{n}
%     \end{split}
% \end{align*}

% The last step uses  that $\frac{r+1}{n-r} \leq \frac{1}{2}$ when $n \geq 3r +2$, which holds when $r \ll n$.

% Then by using  that $\xi_{j_0,j_0+(m-1)T_0} \leq \frac{\mu}{2}$
% \begin{align*}
% \|\iw_{t}(r) - \iw_t(r-1) \| &\le \frac{2\frac{\eta r c_2}{n-r}+ \frac{n}{n-r}\Delta_r}{\eta \mu - \eta \frac{n}{n-r}\xi_{j_0,j_0+(m-1)T_0}}\\
% &= \frac{2r c_2/n + \Delta_r }{(1-r/n)\mu - \xi_{j_0,j_0+(m-1)T_0}}\\
% & \leq \frac{2r c_2/n + \frac{3}{4}\mu\frac{M_1}{\frac{1}{2}-\frac{1}{n}}\frac{Cr}{n}}{\frac{1}{2}\mu - \frac{r}{n}\mu} = \frac{CM_1}{\frac{1}{2}-\frac{r}{n}}\frac{r}{n}
% \end{align*}


% % As long as $\xi_{j_0,j_0+(m-1)T_0} \leq \frac{\mu}{2}$, then 
% % $$\|\iw_{t} - \iw_t(r-1) \| \leq \frac{2r c_2/n}{(1-r/n)\mu - \xi_{j_0,j_0+(m-1)T_0}} \leq \frac{2r c_2/n}{(1-r/n)\mu - \frac{\mu}{2}} = \frac{1}{\frac{1}{2}-\frac{r}{n}}M_1 \frac{r}{n}$$
% % % $$ = \frac{2c_2(M_1 + \frac{n}{r}\delta_{j_1,j_m})r/n}{(1-\frac{r}{n})\mu\frac{n}{r}\delta_{j_1,j_m} + 2c_2} \leq M_1\frac{r}{n} + \delta_{j_1,j_m}$$
% % The last step uses  that $M_1 = \frac{2c_2}{\mu}$.

% % is bounded by $M_2\frac{r}{n}$ where $M_2 = 2c_2/\beta$ is some positive constant.

\end{proof}



\textbf{The proof of Theorem \ref{main10_multi}}
\begin{proof}
Recall that the update rule for $\uw_t(r)$ is:
$$\uw_{t+1}(r) = \uw_t(r) - \eta\frac{1}{n-r}\sum_{i\not\in R_r}\nabla F(\uw_t(r))$$ and the update rule for $\iw_t(r)$ is (where the gradients are explicitly evaluated):
$$\iw_{t+1}(r) = \iw_{t}(r) - \frac{\eta}{n-r}[(n-r+1)(\B_{j_m}^{r-1}(\iw_t(r) - \iw_t(r-1)) + \ag(\iw_{t}(r-1))) - \nabla F_{i_r}(\iw_t(r))]$$
Then by subtracting $\iw_{t+1}(r)$ from $\uw_{t+1}(r)$, we get:
\begin{align*}
    \begin{split}
        & \|\iw_{t+1}(r) - \uw_{t+1}(r)\|\\
        & = \|\iw_{t}(r) - \uw_{t}(r) - \frac{\eta}{n-r}[(n-r+1)(\B_{j_m}^{r-1}(\iw_t(r) - \iw_t(r-1)) \\
        & + \ag(\iw_{t}(r-1))) - \nabla F_{i_r}(\iw_t(r))] + \frac{\eta}{n-r}\sum_{i \not\in R_r}\nabla F(\uw_t(r))\|\\
    \end{split}
\end{align*}

Then by bringing in $\bH_t^{r-1}$ and $\frac{1}{n-r+1}\sum_{i\in R_{r-1}}\nabla F(\iw_t(r-1))$ into the formula above, we get:
\begin{align*}
    \begin{split}
        & = \|\iw_{t}(r) - \uw_{t}(r) - \frac{(n-r+1)\eta}{n-r}\left[\left(\B_{j_m}^{r-1} - \bH_{t}^{r-1}\right)(\iw_{t}(r) - \iw_{t}(r-1))\right.\\
        & + \bH_{t}^{r-1}\mmop(\iw_{t}(r) - \iw_{t}(r-1)) + \ag(\iw_{t}(r-1))\\
        &\left. - \frac{1}{n-r+1}\sum_{i\in R_{r-1}}\nabla F(\iw_t(r-1)) + \frac{1}{n-r+1}\sum_{i\in R_{r-1}}\nabla F(\iw_t(r-1))\right]\\
     & + \frac{\eta}{n-r}(\nabla F_{i_r}(\iw_{t}(r)) - \nabla F_{i_r}(\iw_{t}(r-1)) + \nabla F_{i_r}(\iw_{t}(r-1)))\\
     & + \frac{\eta}{n-r}\sum_{\substack{i \not\in R_r}} \nabla F_i(\uw_{t}(r))\|
    \end{split}
\end{align*}

Then by using triangle inequality and the result from Formula \eqref{eq: real_approx_gradient_gap_tight}, the formula above can be bounded as:
\begin{align*}
    \begin{split}
        & \leq \|\iw_{t}(r) - \uw_{t}(r) - \frac{(n-r+1)\eta}{n-r}\left[\left(\B_{j_m}^{r-1} - \bH_{t}^{r-1}\right)(\iw_{t}(r) - \iw_{t}(r-1))\right.\\
        & + \left.\bH_{t}^{r-1}\mmop(\iw_{t}(r) - \iw_{t}(r-1)) + \frac{1}{n-r+1}\sum_{i\in R_{r-1}}\nabla F_i(\iw_t(r-1))\right]\\
     & + \frac{\eta}{n-r}(\nabla F_{i_r}(\iw_{t}(r)) - \nabla F_{i_r}(\iw_{t}(r-1)) + \nabla F_{i_r}(\iw_{t}(r-1)))\\
     & + \frac{\eta}{n-r}\sum_{\substack{i \not\in R_r}} \nabla F_i(\uw_{t}(r))\| + A (1-\mu\eta)^{j_0 + xT_0}d_{0,(m-1)T_0}(0)r\wikbounds\\
        & + A(r\wikbounds)^2
    \end{split}
\end{align*}

Note that the first matrix norm in this formula is the same as Formula \eqref{eq: w_i_w_u_gap_deriv1} by replacing $n$, $r$, $\iw_t$, $\uw_t$, $\w_t$, $\B_{j_m}$, $\bH_t$ and $\nabla F(\w_t)$ with $n-r+1$, $1$, $\iw_t(r)$, $\uw_t(r)$, $\iw_t(r-1)$, $\B_{j_m}^{r-1}$, $\bH_t^{r-1}$ and $\frac{1}{n-r+1}\sum_{i\not\in R_{r-1}}\nabla F_i(\iw_t(r-1))$ reps.. So by following the same derivation, the formula above can be bounded as:
\begin{align}
\begin{split}
& \leq \|(\textbf{I} - \frac{\eta}{n-r}\sum_{\substack{i \not\in R_r}}\bH_{t,i}^{r-1})(\iw_{t}(r)-\uw_{t}(r))\|\\
& + \|\frac{(n-r+1)\eta}{n-r}\left[\left(\B_{j_m}^{r-1} - \bH_{t}^{r-1}\right)(\iw_{t}(r) - \uw_{t}(r))\right]\|\\
& + \|\frac{\eta}{n-r}[\sum_{i\not\in R_r}\int_0^1 \bH_i(\iw_t(r-1) + x(\uw_t(r)-\iw_t(r-1)))dx \\
& - \int_0^1 \bH_i(\iw_t(r-1) + x(\iw_t(r)-\iw_t(r-1)))dx](\uw_{t}(r)-\iw_t(r-1))\|\\
& + \|\frac{(n-r+1)\eta}{n-r}\left[\left(\B_{j_m}^{r-1} - \bH_{t}^{r-1}\right)(\uw_{t}(r) - \iw_{t}(r-1))\right]\|\\
& + A (1-\mu\eta)^{j_0 + xT_0}d_{0,(m-1)T_0}(0)r\wikbounds\\
        & + A(r\wikbounds)^2
\end{split}
\end{align}

Then we use the following facts 
\benum 
\item $\|\textbf{I} - \eta \bH_{t,i}^{r-1}\| \le 1 - \eta \mu$ 
\item from Theorem \ref{bfi2_multi_all} on the approximation accuracy of the quasi-Hessian to mean Hessian, we have the error bound $\|\bH_t^{r-1} - \B_{j_m}^{r-1}\|\le\xi_{j_1,j_m}(r-1)$,
\item we bound the difference of integrated Hessians using the strategy from equation \eqref{eq: hessian_diff_bound0}
\item from Formula \eqref{eq: w_u_w_i_prev_bound}, we have the error bound $\|\uw_{t}(r)-\iw_t(r-1)\|\le M_2 \frac{r}{n}$ (and this requires no additional assumptions)
\eenum
The expression can be bounded as follows. 

\begin{align}
    \begin{split}
        & \leq (1-\eta\mu + \frac{(n-r+1)\eta}{n-r}\xi_{j_0,j_0+(m-1)T_0}(r-1)+\frac{c_0M_2r\eta}{2n})\|\iw_t - \uw_t\|\\
        & + \frac{M_2(n-r+1)r\eta}{n(n-r)} \xi_{j_1,j_m}(r-1) + A (1-\mu\eta)^{j_0 + xT_0}d_{0,(m-1)T_0}(0)r\wikbounds\\
        & + A(r\wikbounds)^2
    \end{split}
\end{align}



% By using the result from Formula \eqref{eq: xi_bound_multi}, the formula above can be bounded as:
% \begin{align}
%     \begin{split}
%         & \leq (1-\eta\mu + \frac{n\eta}{n-r}\xi_{j_0,j_0+(m-1)T_0}(r-1)+\frac{c_0M_2r\eta}{2n})\|\iw_t - \uw_t\|\\
%         & + \frac{M_2r\eta}{n-r} (A (1-\mu\eta)^{j_0 + xT_0}d_{0,mT_0-1}(0) + A(2r-1)\wikbounds)\\
%         & + A (1-\mu\eta)^{j_0 + xT_0}d_{0,mT_0-1}(0)r\wikbounds\\
%         & + A(r\wikbounds)^2
%     \end{split}
% \end{align}

which is very similar to Formula \eqref{eq: w_u_w_i_gap_deriv_2} (except the difference in the coefficient). So by following the derivation after Formula \eqref{eq: w_u_w_i_gap_deriv_2}, we know that:
\begin{align}
    \|\iw_t(r)-\uw_t(r)\| = o(\frac{r}{n})
\end{align}

when $t\rightarrow \infty$.

\end{proof}


% \begin{theorem}[Bound between iterates on full data and incrementally updated ones (all iterations, online)]\label{bfi2_multi}
% For any $j_m < t < j_m +T_0 - 1$, 
% % the result $\iw_t$ of Algorithm \ref{alg: update_algorithm} approximates the correct iteration values $\uw_t$ at the rate 
% $\|\iw_t - \w_t\| \leq \frac{1}{\frac{1}{2}-\frac{r}{n}}M_1\frac{r}{n}$ and $\|\bH_{t} - \B_{j_m}\| \leq \xi_{j_1,j_m}$. 
% % Recall that $j_1,\ldots,j_m$ depend on $t$,  $\xi_{j_1,j_m}$ is defined in \eqref{xi} and $M_3$ is the constant from Theorem \ref{main1}.
% \end{theorem}


% $\B - \bH \leq \xi_{j_1, j_m} = Ad_{j_1,j_m +T_0 -1}(k) + C$

% $d_{j_1,j_m+T_0-1}(k) \leq d_{j_1,j_m+T_0-1}(k-1) + \frac{2}{n} \frac{1}{\frac{1}{2} - \frac{1}{n}}$







\input{online_SGD_analysis.tex}



\subsection{Extension of \Increm\ for non-strongly convex, non-smooth objective functions}

For the original version of the L-BFGS algorithm, strong convexity is essential to make the secant condition hold. In this subsection, we present our extension of \Increm\ to non-strongly convex, non-smooth objectives. 

To deal with non-strongly convex objectives, we assume that convexity holds in some local regions. When constructing the arrays $\Delta G$ and $\Delta W$, only the model parameters and their gradients where local convexity holds are used. 

For local non-smoothness, we found that even a small distance between $\w_t$ and $\iw_t$ can make the estimated gradient $\nabla F(\iw_t)$ drift far away from $\nabla F(\w_t)$.
To deal with this, we explicitly check if the norm of $\B_{j_m}(\w_t - \iw_t)$ (which equals to $\nabla F(\iw_t) - \nabla F(\w_t)$) is larger than the norm of $L(\w_t - \iw_t)$ for a constant $L$. In our experiments, $L$ is configured as 1.
% when the gradients are approximately computed, the estimated gradients  can be very far away from 
The details of the modifications above are highlighted in Algorithm \ref{alg: update_algorithm_general}.


\begin{algorithm}[!htbp] 
\small
% \footnotesize
\SetKw{Continue}{continue}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{The full training set $\left(\textbf{X}, \textbf{Y}\right)$, model parameters cached during the training phase for the full training samples $\{\w_{0}, \w_{1}, \dots, \w_{t}\}$ and corresponding gradients $\{\nabla F\left(\w_{0}\right), \nabla F\left(\w_{1}\right), \dots, \nabla F\left(\w_{t}\right)\}$, the removed training sample or the added training sample $R$, period $T_0$, total iteration number $T$, history size $m$, warmup iteration number $j_0$, learning rate $\eta$}
\Output{Updated model parameter $\iw_{t}$}
Initialize $\iw_{0} \leftarrow \w_{0}$

Initialize an array $\Delta G = \left[\right]$

Initialize an array $\Delta W = \left[\right]$

Initialize $last\_t = j_0$

$is\_explicit=False$

\For{$t=0;t<T; t++$}{

\eIf{\hl{$(t - last_t)  \mod T_0 == 0$ or $t \leq j_0$}}
{
    \hl{$is\_explicit=True$}
}


\eIf{$is\_explicit == True$ or $t \leq j_0$}
{
    $last\_t = t$ \label{line: explicit_start}
        
    compute $\nabla F\left(\iw_{t}\right)$ exactly
    
    compute $\nabla F\left(\iw_{t}\right) - \nabla F\left(\w_{t}\right)$ based on the cached gradient $\nabla F\left(\w_{t}\right)$
    
    \tcc{check local convexity}
    \If{\hl{$<\nabla F\left(\iw_{t}\right) - \nabla F\left(\w_{t}\right), \iw_{t} - \w_{t}> \leq 0$}}
    {
        \hl{compute $\iw_{t+1}$ by using exact GD update
        (equation \eqref{eq: update_rule_naive})    }
        
        \Continue
    }
    
    set $\Delta G\left[k\right] = \nabla F\left(\iw_{t}\right) - \nabla F\left(\w_{t}\right)$
    
    set $\Delta W\left[k\right] = \iw_{t} - \w_{t}$, based on the cached parameters $\w_{t}$
    
    $k\leftarrow k+1$
    
    compute $\iw_{t+1}$ by using exact GD update
    (equation \eqref{eq: update_rule_naive})
}
{
    Pass $\Delta W\left[-m:\right]$, $\Delta G\left[-m:\right]$, the last $m$ elements in $\Delta W$ and $\Delta G$, which are from the $j_1^{th}, j_2^{th},\dots, j_m^{th}$ iterations where $j_1 < j_2< \dots < j_m$ depend on $t$, $\textbf{v} = \iw_{t} - \w_{t}$, and the history size $m$, to the L-BFGFS Algorithm (See Supplement) to get the approximation of $\bH(\w_{t})\textbf{v}$, i.e., $\B_{j_m}\textbf{v}$
    
    \tcc{check local smoothness}
    \If{\hl{$\|\B_{j_m}\textbf{v}\| \geq \|\textbf{v}\|$}}
    {
        \hl{\textbf{go to} line \ref{line: explicit_start}}
    }
    
    Approximate $\nabla F\left(\iw_{t}\right) = \nabla F\left(\w_{t}\right) + \B_{j_m}\left(\iw_{t} - \w_{t}\right)$
    
    Compute $\iw_{t+1}$ by using the "leave-$r$-out" gradient formula, based on the approximated $\nabla F(\iw_{t})$ 
}
}

\Return $\iw_{t}$
\caption{DeltaGrad (general models)}
\label{alg: update_algorithm_general}
\end{algorithm}
